Flux: Liquid Types for Rust

We introduce Flux, which shows how logical refinements can work hand in glove with Rust's ownership mechanisms to yield ergonomic type-based verification of low-level pointer manipulating programs. First, we design a novel refined type system for Rust that indexes mutable locations, with pure (immutable) values that can appear in refinements, and then exploits Rust's ownership mechanisms to abstract sub-structural reasoning about locations within Rust's polymorphic type constructors, while supporting strong updates. We formalize the crucial dependency upon Rust's strong aliasing guarantees by exploiting the stacked borrows aliasing model to prove that ``well-borrowed evaluations of well-typed programs do not get stuck''. Second, we implement our type system in Flux, a plug-in to the Rust compiler that exploits the factoring of complex invariants into types and refinements to efficiently synthesize loop annotations -- including complex quantified invariants describing the contents of containers -- via liquid inference. Third, we evaluate Flux with a benchmark suite of vector manipulating programs and parts of a previously verified secure sandboxing library to demonstrate the advantages of refinement types over program logics as implemented in the state-of-the-art Prusti verifier. While Prusti's more expressive program logic can, in general, verify deep functional correctness specifications, for the lightweight but ubiquitous and important verification use-cases covered by our benchmarks, liquid typing makes verification ergonomic by slashing specification lines by a factor of two, verification time by an order of magnitude, and annotation overhead from up to 24% of code size (average 9%) to nothing at all.

==> Makefile <==
all: pdf

pdf:
	latexmk -pdf main.tex

cont: continuous
continuous:
	latexmk -pvc -pdf -interaction=nonstopmode main.tex

chop:
	rm -f anon-supplemental.pdf anon-submission.pdf
	cp main.pdf anon-supplemental.pdf
	if which cpdf; \
         then cpdf  anon-supplemental.pdf "1-28" -o anon-submission.pdf; \
         else pdftk anon-supplemental.pdf cat 1-28 output anon-submission.pdf; fi

plain:
	touch no-editing-marks
	$(MAKE) clean
	$(MAKE) 

ed:
	rm -f no-editing-marks
	$(MAKE) clean
	$(MAKE)

clean:
	latexmk -c main.tex

cleanall:
	latexmk -C -bibtex main.tex

.PHONY: all pdf clean cleanall cont continuous plain ed


==> decr-typing.tex <==
{
$$
\begin{array}{l}
\lineno{ 1}  \ctxts{
               \decr :
               \polysig{}
               {}
               {}
               {}
               {\tbor{\lft}{\mut}{\nat}}
               {\uninit{n}}
               {}
            } \\

\lineno{ 2} \kw{let}\ \decr = \kw{rec}\ \ff \rparam{}(x)\ :=\ \\
\lineno{ 3}  \ind \ctxts{ \varcx_1 = \emptyset ;
                          \env_1   = \greater\bind..., \minus\bind..., \ff\bind..., x\bind\tbor{\lft}{\mut}{\nat};
                          \loccx_1 = \emptyset
                        }  \\
\lineno{ 4}  \ind \kw{let}\ \yy = *\xx\ \kw{in}\\
\lineno{ 5}  \ind \ctxts{ \varcx_2 = \emptyset ;
                          \env_2   = \env_1, y\bind \nat;
                          \loccx_2 = \loccx_1
                        }\\
\lineno{ 6}  \ind \kw{unpack}\ (\yy, \aa_\yy)\ \kw{in}\\
\lineno{ 7}  \ind \ctxts{ \varcx_3 = \aa_\yy\bind\sint, \aa_\yy \geq 0;
                          \env_3 = \env_1,\yy\bind \tint<\aa>;
                          \loccx_3 = \loccx_1
                        } \\
\lineno{ 8}  \ind \kw{if}\ \kw{call}\ \greater{}\rparam{\aa_\yy, 0}(\yy, 0)\ \{ \\
\lineno{ 9}  \ind\ind \ctxts{ \varcx_4 = \varcx_3, \aa_\yy > 0;
                              \env_4   = \env_3;
                              \loccx_4 = \loccx_1
                            } \\
\lineno{10}  \ind\ind \xx := \kw{call}\ \minus\rparam{\aa_\yy, 1}(\yy, 1)  \quad \ctxts{\tassign: \subtyping[\varcx_4]{\tint<\aa_\yy - 1>}{\nat}}
            \\
\lineno{11}  \ind \}\ \kw{else}\ \{ \poison \} \\
            % \ident \ctxts{ \varcx_5 = \varcx_3; \env_5   = \env_3; \loccx_5 = \loccx_1}
\end{array}
$$
}%
\begin{comment}
$$
\begin{array}{l}
\less : \polysig{\overline{\tvar}}
{\aa_1,\aa_2:\sint}
{{\ctrue}}
{\emptyset}
{\rtyp{\tint}{\aa_1},\rtyp{\tint}{\aa_2}}
{\rtyp{\tbool}{\aa_1 <  \aa_2}}
{\emptyset}\\
\minus : \polysig{\overline{\tvar}}
{\aa_1,\aa_2:\sint}
{{\ctrue}}
{\emptyset}
{\rtyp{\tint}{\aa_1},\rtyp{\tint}{\aa_2}}
{\rtyp{\tint}{\aa_1 - \aa_2}}
{\emptyset}\\
\decr : \polysig{\overline{\tvar}}
{}
{{\ctrue}}
{\emptyset}
{\tbor{\lft}{\mut}{\texists{\aa}{\rtyp{\tint}{\aa}}{0 \leq \aa}}}
{\uninit{n}}
{\emptyset}\\
\kw{let}\ \decr = \kw{rec}\ \ff \langle \rangle(x)\ :=\ \\
\quad\ \ {\color{gray} \tfun: \varcx:= \emptyset
              , \env:= \less:\_, \minus:\_, \ff:\_, x:\tbor{\lft}{\mut}{\texists{\aa}{\rtyp{\tint}{\aa}}{0 \leq \aa}}
              , \loccx := \emptyset}  \\
\quad\ \ \kw{let}\ \yy = *\xx\ \kw{in}\\
\quad\ \ {\color{gray} \tlet:
                 \env \addenv \yy:\texists{\aa}{\rtyp{\tint}{\aa}}{0 \leq \aa}
}\\
\quad\ \ \kw{unpack}\ (\yy, \aa_\yy)\ \kw{in}\\
\quad\ \ {\color{gray} \tunpack:
    \varcx \addenv  \aa_\yy:\sint, 0 \leq \aa_\yy,
    \env \updenv \yy: \rtyp{\tint}{\aa_\yy}} \\
\quad\ \ \kw{if}\ \kw{call}\ \less\ \langle 0, \aa_\yy \rangle\   (0,\yy)\ \{
{\color{gray}  :: \rtyp{\tbool}{0 < \aa_\yy} \text{ by rule } \tcall}
\\
\quad\ \ {\color{gray} \tif_1: \varcx \addenv 0 < \aa_\yy}  \\
\quad\quad\ \ \xx := \kw{call}\ \minus\ \langle \aa_\yy, 1 \rangle\ (\yy,1)  \quad
{\color{gray} :: \rtyp{\tint}{\aa_\yy - 1}
\text{ by rule } \tcall}
\\
\quad\ \ {\color{gray} \tassign, \text{since }
\subtyping[\aa_\yy:\sint, 0 \leq \aa_\yy, 0 < \aa_\yy]{\rtyp{\tint}{\aa_\yy - 1}}{\texists{\aa}{\rtyp{\tint}{\aa}}{0 \leq \aa}}
 }  \\

\quad\ \ \}\ \kw{else}\ \{ \poison \} \\
\quad\ \ {\color{gray} \tif:
\loccx = \emptyset, \typ = \uninit{n} }
\end{array}
$$
\end{comment}
%


==> formal/syntax-fig-long.tex <==
\begin{figure}
    {
    \small
    $$
    \begin{array}{rrcl}
        \syntaxcat{Expressions} &
        e & ::= &
                     \blet{\xx}{\highlight{\new{\lvar}}}{e}
                \mid \highlight{\eunpack{\xx}{\aa}{e}}
                \\
          && \mid &
                     \fcall*{e}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}
                \mid \sassign{\place}{\ee}
                \mid \blet{\xx}{e}{e}
                \mid \bif{\ee}{e}{e}
                \\
          && \mid &
                     \rvstrgref{\place}
                \mid \rvmutref{\place}
                \mid \rvshrref{\place}
                \mid \deref{\place}
                \mid \xx
                \mid \val                                              \\
        \syntaxcat{Values} &
        \val & ::=
                        & \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}
                 \mid \ctrue \mid \cfalse
                   \mid  0, \pm 1, \dots                   \\
                && \mid & \poison \mid \vptr{\cloc}{\ptrtag}
                                                 \\


        \syntaxcat{A-values} &
            \aval & ::=  & \val \mid \xx  \\

        \syntaxcat{Places} &
            \place & ::= & \xx \mid \vptr{\cloc}{\ptrtag} \\

        \syntaxcat{Refinements} &
          \expr & ::= & \aa \mid \cloc \mid  \ctrue \mid \cfalse \mid 0, \pm 1, \dots
          \mid \expr = \expr \mid \lnot \expr \mid \expr [\land,\lor] \expr \mid \expr [+, - , *] \expr  \\
          % && \mid & \

        \syntaxcat{Types} &
            \typ & :=   &
                             \highlight{\rtyp{\tcon}{\expr}}
                        \mid \highlight{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}
                        \mid \highlight{\tptr{\loc}}
                        \mid \tbor{\lft}{\bormode}{\typ}
                        \mid \uninit{n}
                        \\
                && \mid & \polysig{\overline{\tvar}}
                                  {\highlight{\overline{\aa: \sort}}}
                                  {\highlight{\expr}}
                                  {\loccx}
                                  {\overline{\typ}}
                                  {\typ}
                                  {\loccx} \\
        \syntaxcat{Base Types} &
            \tcon & ::= & \tint  \mid \tbool      \\

        \syntaxcat{Modifier} &
            \bormode & ::=   & \mut \mid \shr   \\

        \syntaxcat{Locations} &
            \loc & := & \cloc \mid \lvar    \\

        \syntaxcat{Sorts} &
            \sort  & := &  \sint \mid \sbool \mid \sloc \lftonly{\mid  \slft}\\

            \syntaxcat{Contexts} & && \\
            \syntaxcat{Value} &
            \env & :=   & \emptyset \mid \env, \mapstoenv{\xx}{\typ} \\
            \syntaxcat{Refinement} &
            \varcx & :=   & \emptyset
                        \mid \varcx, \aa: \sort
                        \mid \varcx, \expr \\
        \syntaxcat{Location} &
            \loccx & :=   & \emptyset \mid \loccx, \mapstoowned{\loc}{\typ} \\
    \end{array}
    $$
    }
\caption{Syntax of \corelan.}
\label{fig:syntax}
\end{figure}


==> formal/syntax-fig-old.tex <==
\begin{figure}
    {
    \small
    $$
    \begin{array}{rrcll}
        \syntaxcat{Expressions} &
        e & ::= & \blet{\xx}{\highlight{\new{\lvar}}}{e} % \mid           & \textit{allocation and let-bind}       \\
        \mid  \highlight{\eunpack{\xx}{\aa}{e}}                         & \textit{allocation and unpack} \\
          && \mid & \fcall*{e}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}  % & \textit{function call} \\
             \mid  \sassign{\place}{\ee}                                     & \textit{call and assignment} \\
          && \mid & \rvstrgref{\place} \mid \rvmutref{\place} \mid \rvshrref{\place} & \textit{(re)borrows} \\
          && \mid & \blet{\xx}{e}{e} \mid \bif{\ee}{e}{e} & \textit{let-bind and if}       \\
          && \mid & \deref{\place}                                            % & \textit{potinter dereference} \\
          \mid \xx \mid  \val                                             & \textit{deref, variables, and values} \\
        % \syntaxcat{Statements} &
        % \stmt & ::=  & \sassign{\place}{\rval}                                & \textit{assignment} \\
        %      && \mid & \sskip                                                 & \textit{} \\
        \syntaxcat{Values} &
        \val & ::=
                        & \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}   % & \textit{functions} \\
                 \mid \ctrue \mid \cfalse
                   \mid  0, \pm 1, \dots                   & \textit{functions and constants}  \\
                && \mid & \poison \mid \vptr{\cloc}{\ptrtag}             % & \textit{pointers (intermediate)} \\
                                                 & \textit{uninitialized memory and pointers} \\

          \syntaxcat{Logic} &
          \expr & ::= & \aa \mid \cloc \mid  \ctrue \mid \cfalse \mid 0, \pm 1, \dots & \textit{variables and constants} \\
          && \mid & \expr = \expr \mid \lnot \expr \mid \expr \land \expr \mid \expr [+, - , *] \expr  & \textit{equality, bools, and  arithmetic} \\
          % && \mid & \                                                             & \textit{locations} \\


        \syntaxcat{A-values} &
            \aval & ::=  & \val \mid \xx  \\

        \syntaxcat{Places} &
            \place & ::= & \xx \mid \vptr{\cloc}{\ptrtag} & \textit{variables and tagged locations}\\

        \syntaxcat{Locations} &
            \loc & := & \cloc \mid \lvar    \\

        \syntaxcat{Types} &
            \typ & :=   & \highlight{\rtyp{\tcon}{\expr}}
                \mid \highlight{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}  & \textit{indexed and existential types} \\
                && \mid & \highlight{\tptr{\loc}}                          %    & \textit{pointer to location $\loc$}\\
                 \mid  \tbor{\lft}{\bormode}{\typ}              %& \textit{borrowed reference (mutable or shared)}  \\
                 \mid  \uninit{n}                               & \textit{pointer, reference, and uninitialized} \\
                && \mid & \polysig{\overline{\tvar}}
                                  {\highlight{\overline{\aa: \sort}}}
                                  {\highlight{\expr}}
                                  {\loccx}
                                  {\overline{\typ}}
                                  {\typ}
                                  {\loccx} \\
        \syntaxcat{Base Types} &
            \tcon & ::= & \tint  \mid \tbool      & \textit{integers, booleans} \\
        \syntaxcat{Modifier} &
            \bormode & ::=   & \mut \mid \shr  & \textit{mutable or shared} \\
        \syntaxcat{Sorts} &
            \sort  & := &  \sint \mid \sbool \mid \sloc \lftonly{\mid  \slft}\\

            \syntaxcat{ Environments} & &&& \\
            \syntaxcat{Variable} &
            \env & :=   & \emptyset \mid \env, \mapstoenv{\xx}{\typ} \\
            \syntaxcat{Logical} &
            \varcx & :=   & \emptyset
                        \mid \varcx, \aa: \sort
                        \mid \varcx, \expr \\
        \syntaxcat{Location} &
            \loccx & :=   & \emptyset \mid \loccx, \mapstoowned{\loc}{\typ} \\
    \end{array}
    $$
    }
\caption{Syntax of \corelan.}
\label{fig:syntax}
\end{figure}


==> impl-old.tex <==
\lstMakeShortInline[language=lr,basicstyle=\ttfamily]`

\section{Algorithmic Verification}
\label{sec:implementation}

\sys implements the type checking rules of~\Cref{sec:formalism}
as a \rust compiler plugin, adding an  extra analysis step to the
compiler pipeline (similar to the Clippy\footnote{
    \url{https://github.com/rust-lang/rust-clippy}} linter).
%
As a compiler plugin, \sys operates on compiled \rust programs,
which has two major benefits.
%
First, the programs satisfy \rust's safety requirements, which
are assumed by our analysis. For example,
\sys assumes that
every access through a reference
satisfies \rust's \emph{borrow-checker} rules.
Second, the \rust compiler generates the typed intermediate
representation of compiled programs, which is passed to \sys.
%
Concretely, \sys performs the analysis on
\rust Mid-level Intermediate Representation (MIR) which is extracted
from the compiler combined with (non refined) type information.
%
MIR is a control-flow graph (CFG) representation,
unlike our core calculus \corelan
that is in continuation passing style (CPS),
but this is not a challenge, since both
representations are easy to relate
via the correspondence defined by \citet{CFGCPS}.

Yet, there were three main challenges in implementing
\sys as the core system presented in~\S~\ref{sec:formalism}.
First (\S~\ref{subsec:impl:parameters}),
the syntax of \corelan
has explicit refinement annotations
(the highlighted % $\highlight{\text{highlighted}}$
parts of~\cref{fig:formalism:syntax}).
that do not appear in \rust's MIR.
Second (\S~\ref{subsec:impl:continuations}),
the \corelan judgements have rules that require  inference,
\eg the rule \tletcont of~\cref{fig:ty:instr} guesses the continuation's
context.
Finally (\S~\ref{subsec:impl:poly}),
\sys supports polymorphic types
% (encoded as the type indexed vectors in~\S~\ref{sec:formalism})
which is crucial for ergonomic specification and
verification, but require the instantiation of
refinement types which is, in general, challenging to
implement.
%
We explain how we addressed these three challenges via the
liquid types inference framework~\citep{LiquidTypes, LocalRefinement}.



\subsection{Refinement Annotations}
\label{subsec:impl:parameters}
\label{subsec:implementation:inference}

\sys, following the essence of refinement typing,
does not modify the syntax of \rust programs,
but permits refined type signatures.
So, the users should explicitly declare the refined
type signatures of \corelan (using the user-friendly
syntax of~\S~\ref{sec:overview}),
but the \kw{unpack} instructions
and the refinement parameters of function calls and continuation
jumps are automatically inferred by the system.

The inference of \kw{unpack} instructions happens on-the-fly.
The MIR code analyzed by \tool{} does not have explicit
\kw{unpack} instructions.
% \ag{``MIR code analyzed...'' flows a little better to me than ``The MIR that is analyzed'', or just ``MIR analyzed''.}
Instead, \tool introduces a fresh refinement variable
as soon as an existential type goes into the context.
In this way it can keep the context normalized,
which is required for the instantiation of
refinement parameters.

The refinement parameter instantiation
is performed by a syntax-directed heuristic.
Intuitively, \tool uses the `@n` syntax
to connect each refinement parameter with a concrete
function argument.
%
%To simplify refinement parameter instantiation, we apply some syntactic restrictions to the surface syntax.
%In particular, instead of having a separate list of parameters that can be used
%freely in the function signature, we require a parameter `n` to be declared alongside its use
%as an index with the `@n` syntax.
%This restriction is used to pick a definite position to unify the parameter with a refinement
%expression at the call site.
%We guide unification by matching the type of arguments.
For instance, consider the function `is_pos` from~\S~\ref{fig:functional}
which refines its argument using `i32<@n>`.
%
In the call `is_pos($\n1$)`, we can match the type `i32<$\n1$>` with `i32<@n>`
and instantiate `n` to `$\n1$`.


This strategy
performs well in practice,
and it is sufficient to instantiate the parameters
in all the benchmarks in our evaluation (\S~\ref{sec:eval}), but it
is not complete, for example it cannot infer a parameter declared
inside a polymorphic argument.
%
In case of instantiation failure \sys exits with an error and
the user can, as a fallback option,
provide additional arguments to simplify the instantiation.
%
For example, the function `normalize_centers` in \cref{fig:kmeans} has to
take an additional parameter to declare `@n` because \sys would not be able to instantiate it
inside the inner `RVec`.

\subsection{Refinement Inference}
\label{subsec:impl:continuations}
The rule \tletcont requires guessing (\aka inferring) a
signature for the continuation that, combined with the (also non-algorithmic)
context inclusion judgement, is used to check loop invariants.
% The \corelan typing rule that requires guessing
% (\aka inference) is the rule \tletcont
% that, combined with the (also non algorithmic)
% context inclusion checking, is used to check loop invariants.
%
In \sys such loop invariants are encoded as logical invariants
in the continuation contexts and are inferred in a \textit{two phase} analysis.
As an example, consider the function
`init_zeros` in~\cref{fig:kmeans} of \S~\ref{sec:overview}.
%
In this function, the header of the loop
corresponds to continuation,
let's call it \kk, and it is associated to
a context $\loccx_\kk$.
%
The goal is to infer this context.

\bpara{In the first phase} of the analysis, \tool collects all the join points
of the continuation, \ie all the contexts that jump to \kk.
In the `init_zeros` example, the loop
is entered under two different contexts,
the initial context $\loccx_0$ and the loop body $\loccx_i$:
$$
\begin{array}{rcl}
    \loccx_0
    &\defeq&
    \{\vartt{n} \mapsto \rtyptt{usize}<v>, \vartt{i} \mapsto \rtyptt{i32}<\n0>, \vartt{vec} \mapsto \rtyptt{RVec}<\rtyptt{f32}, \n0>\}
    \\
    \loccx_i
    &\defeq&
    \{\vartt{n} \mapsto \rtyptt{usize}<v>, \vartt{i} \mapsto \rtyptt{i32}<j+\n1>, \vartt{vec} \mapsto \rtyptt{RVec}<\rtyptt{f32}, j+\n1>\}
\end{array}
$$
Where `n`, `i`, and `vec` are the locations in scope.
% contexts while $\dots$ denotes other non-shared locations.
The variable $v$ indexing the type of `n` is in scope for
the entire function and since `n` is not mutated through the loop its
type is the same in both contexts.
%
The refinement variable $j$ signifies the value of `i` in
the previous iteration, and it is out of scope outside the body of loop.
%
The goal of inference is to construct
a continuation context that includes both
$\loccx_0$ and $\loccx_1$ and it is strong
enough to prove that the length of `vec` equals `n`.
By syntactic unification,
the first phase of the analysis will construct the following
continuation context.
%
$$
\begin{array}{l}
    \kk :  \forall b, c.\, \kw{cont}(\kappa(b, c);\loccx_\kk), \text{ where }
    \loccx_\kk
    \defeq
    \{\vartt{n} \mapsto \rtyptt{usize}<v>, \vartt{i} \mapsto \rtyptt{i32}<b>, \vartt{vec} \mapsto \rtyptt{RVec}<\rtyptt{f32}, c>\}
\end{array}
$$
That is, the derived context preserves the matching
parts (here the index of `n`),
while for the rest (here the indices of `i` and `vec`)
fresh logical names are generated (here $b$ and $c$).
%
% \ag{The previous sentence is a little confusing. ``While for the rest fresh logical names are generated (here ...)'' maybe?}
Importantly, the fresh names can be related
by the \textit{refinement variable}
$\kappa$, \ie an unknown predicate capturing dependencies
between logical values whose value will be decided using
liquid types inference in the next phase.


\bpara{In the second phase}
the type checking rules of~\S~\ref{sec:formalism}
are applied. These rules check context inclusion at each join point
(rule \tjump) which, in turn, reduces to semantic subtyping (rule \loccxincsub)
that essentially performs validity checking of logical conditions.
In our example, the two continuation calls lead to the following
context inclusion checks.
$$
\begin{array}{lcl}
    \loccxinc{\varcx_0}{\elftcx}{\llftcx}{\loccx_0}{\loccx_\kk[0/b][0/c]}
    &\Rightarrow&
    \kappa(0, 0)
    \\
    \loccxinc{\varcx_i}{\elftcx}{\llftcx}{\loccx_i}{\loccx_\kk[j+1/b][j+1/c]}
    &\Rightarrow&
    \kappa(j+1, j+1)
\end{array}
$$
For typechecking to succeed,
the context inclusion judgements on the left should hold,
which (using the typing rules) reduce to the
logical conditions on the right.
%
These conditions allow liquid inference to find the solution
$\kappa(b,c) := b = c$ for the unknown variable $\kappa$,
which is strong enough to
verify the top level specification of `init_zeros`,
\ie that at the exit of the loop (when $v = b$),
the length of `vec` is equal to `n`.


\subsection{Polymorphic Instantiation}
\label{subsec:impl:poly}

\sys further infers invariants over elements of
type constructors by instantiating
the polymorphic types of the constructors by
existential types with unknown predicates
and solving them using liquid inference.
%
For example, consider the following function that creates
and returns a vector with one element.

\begin{minipage}{\textwidth}
\begin{lr}
#[lr::sig(fn() -> RVec<i32{v : v > `\n0`}>)]
fn make_vec() -> RVec<i32> {
    let vec = RVec::new();   // $\color{comment} \vartt*{vec} \mapsto \rtyptt*{RVec}<\rtyptt*{i32}[\nu: \kappa_1(\nu)], \n0>$
    RVec::push(&mut vec, `\n{42}`); // $\color{comment} \vartt*{vec} \mapsto \rtyptt*{RVec}<\rtyptt*{i32}[\nu: \kappa_2(\nu)], \n1>$
    vec
}
\end{lr}
\end{minipage}
The comments show the type of `vec` after each statement.
The call to `new` needs to instantiate the parameter `T` in the return
type \rtyptt{RVec}<\tvartt, \n0>.
\sys extracts from the \rust compiler that
`T` is instatiated by an `i32` but the refinement is unknown.
Thus, `T` gets instantiated
by the template \rtyptt{i32}[\nu: \kappa_1(\nu)] where $\kappa_1$ is a fresh
refinement variable denoting an unknown predicate.
Similarly, the call to `push` also requires instantiating its polymorphic parameter,
so the template \rtyptt{i32}[\nu: \kappa_2(\nu)] gets created.
%
Type checking the function with these templates
generates three logical constraints:
\begin{align*}
1)\quad \kappa_1(\nu) \Rightarrow \kappa_2(\nu)
&&
2)\quad \nu = 42      \Rightarrow \kappa_2(\nu)
&&
3)\quad \kappa_2(\nu) \Rightarrow \nu > 0
\end{align*}
The first two constraints correspond to subtyping for the first and second arguments to `push`; the third
relates the type of `vec` to the output type.
Using liquid inference, \sys solves both unknows to $\nu > 0$
(\ie
$
\kappa_1(\nu) := \kappa_2(\nu) := \nu > 0
$) which is a predicate strong enough to verify the specification
of `make_vec`.




\lstDeleteShortInline`


==> metatheory/canonical.tex <==
\begin{lemma}[Canonical Forms Booleans]\label{lemma:canonical:bool}
  If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\val}{\typ}{\loccx_o}{} and $\typ = \tbool<\expr>$
  or $\typ = \texists{\aa}{\tbool<\aa>}{\expr'}$
  then $\val = \ctrue$ or $\val = \cfalse$.
\end{lemma}
\begin{proof}
  By induction on the typing derivation.
  The following cases apply:
  \begin{itemize}
    \item \textbf{\ttrue:} Direct since the rules only applies if $\val=\ctrue$.
    \item \textbf{\tfalse:} Direct since the rules only applies if $\val=\cfalse$.
    \item \textbf{\tsub:} By inversion of the subtyping judgment on the premise of the rule either
    \subrtyp, \subunpack or \subexists applies.
    In all cases we conclude by using the inductive hypothesis choosing either the indexed or existential case.
  \end{itemize}
\end{proof}

\begin{lemma}[Canonical Forms Ints]\label{lemma:canonical:int}
  If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\val}{\typ}{\loccx_o}{} and
  $\typ = \tint<n>$ or $\typ = \texists{\aa}{\tint<\aa>}{\expr}$
  then $\val = z$ for some $z\in\mathbb{Z}$.
\end{lemma}
\begin{proof}
  By induction on the typing derivation.
  The following cases apply:
  \begin{itemize}
    \item \textbf{\tconstint:} Direct since the rules only applies if $\val=z$.
    \item \textbf{\tsub:} By inversion of the subtyping judgment on the premise of the rule either
    \subrtyp, \subunpack or \subexists applies.
    In all cases we conclude by using the inductive hypothesis choosing either the indexed or existential case.
  \end{itemize}
\end{proof}

\begin{lemma}[Canonical Forms Pointers]\label{lemma:canonical:ptr}
\quad
\begin{enumerate}
    \item If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\val}{\tptr{\loc}}{\loccx_o}{} then $\val=\vptr{\cloc}{\ptrtag}$.
    \item If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\val}{\tref{\bormode}{\typ}}{\loccx_o}{} then $\val=\vptr{\cloc}{\ptrtag}$.
\end{enumerate}
\end{lemma}
\begin{proof}
    Both by induction on the typing derivation.
    The following cases apply
    \begin{itemize}
        \item \textbf{Case \ttptr:} Direct by the form of the rule.
        \item \textbf{Case \tsub:} By inversion of the subtyping premise in the rule \tsub either
        \subptr, \subborshr or \subbormut apply.
        In all cases we conclude by applying the inductive hypothesis.
    \end{itemize}
\end{proof}

\begin{lemma}[Canonical Forms Vectors]\label{lemma:canonical:vec}
  If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\val}{\typ}{\loccx_o}{} and if $\typ = \tvec<m>$ or $\typ = \texists{\aa}{\tvec<\aa>}{\expr}$
  then $\val = \vvec{n}{\val'}$.
\end{lemma}
\begin{proof}
  By induction on the typing derivation
  The following cases apply:
  \begin{itemize}
    \item \textbf{Case \tvecvec:} Direct since the rule only applies if $\val=\vvec{m}{\val'}$.
    \item \textbf{Case \tsub:} By inversion of the subtyping judgment on the premise of \tsub
    either \subrtyp, \subunpack or \subexists apply.
    In all cases we conclude by using the inductive hypothesis choosing either the indexed or existential case.
  \end{itemize}
\end{proof}

\begin{lemma}[Canonical Forms Functions]\label{lemma:canonical:fun}
  If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\val}
                {\polysig{}
                        {\overline{\aa: \sort}}
                        {\expr}
                        {\loccx}
                        {\overline{\xx : \typ}}{\typ}{\loccx_{fi}}
                }
                {\loccx_o}{},
   then either
  \begin{enumerate}
    \item $\val = \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}$,
    \item $\val = \vecnew$,
    \item $\val = \vecpush$, or
    \item $\val = \vecindexmut$.
  \end{enumerate}
\end{lemma}
\begin{proof}
  By induction on the typing derivation.
  The following cases apply:
  \begin{itemize}
    \item \textbf{Case \tfun:} In this case (1) holds.
    \item \textbf{Case \tvecnew} In this case (2) holds.
    \item \textbf{Case \tvecpush} In this case (3) holds.
    \item \textbf{Case \tvecindexmut} In this case (4) holds.
    \item \textbf{Case \tsub:} By inversion of the subtyping judgment in the premise of the rule
    \tsub we have that only \subfun applies.
    We conclude by applying the inductive hypothesis.
  \end{itemize}
\end{proof}


==> metatheory/commands.tex <==
%% NOTES

\newcommand\nv[1]{{\color{magenta}{NV:#1}}}
% \newcommand\ag[1]{{\color{green}{AG: #1}}}
\newcommand\nl[1]{{\color{cyan}{NL:#1}}}
% \newcommand\rj[1]{{\color{red}{RJ:#1}}}
% \newcommand\nv[1]{}
\newcommand\ag[1]{}
%\newcommand\nl[1]{}
\newcommand\rj[1]{}
\newcommand\tool{\sys\xspace}
\newcommand\ie{\textit{i.e.,}\xspace}
\newcommand\aka{\textit{a.k.a.,}\xspace}
\newcommand\eg{\textit{e.g.,}\xspace}
\newcommand\etc{\textit{etc.}\xspace}
% \newcommand\todoref[1]{{\color{red}{REF[#1]}}}
\newcommand\todo[1]{{\color{red}{#1}}}
\newcommand\nnew[1]{{\color{blue}{#1}}}
\newcommand\bpara[1]{\smallskip\noindent\textbf{\emph{#1}\xspace}}

%%%%%%%%%%%%%
%% Toggles %%
%%%%%%%%%%%%%

%% to hide lifetimes first unset SHOWLFT:
%% export SHOWLFT=false; pdflatex main.tex

\newcommand{\getenv}[2][]{%
  \CatchFileEdef{\temp}{"|kpsewhich --var-value #2"}{\endlinechar=-1}%
  \if\relax\detokenize{#1}\relax\temp\else\let#1\temp\fi}

\getenv[\showlft]{SHOWLFT}
\newtoggle{lft}

\ifdefstring{\showlft}{}{
  \toggletrue{lft}
}{
  \ifdefstring{\showlft}{false}{
    \togglefalse{lft}
  }{
    \toggletrue{lft}
  }
}

\newcommand\lftonly[1]{\iftoggle{lft}{#1}{}}
%\newcommand\lftonly[1]{}

\getenv[\showthrd]{SHOWTHRD}
\newtoggle{thrd}

\ifdefstring{\showthrd}{}{
  \toggletrue{thrd}
  % \togglefalse{thrd}
}{
  \ifdefstring{\showthrd}{false}{
    \togglefalse{thrd}
  }{
    \toggletrue{thrd}
  }
}
\newcommand\thrdonly[1]{\iftoggle{thrd}{#1}{}}
\newcommand\kw[1]{\texttt{\bf{#1}}}

%% Better overset
\makeatletter
\newcommand{\oset}[3][0ex]{%
  \mathrel{\mathop{#3}\limits^{\vbox to #1{\kern-\tw@\ex@
   \hbox{\tiny #2}\vss}}}}
\makeatother

%%%%%%%%%%%%
%% Syntax %%
%%%%%%%%%%%%

% Lambda rust
\newcommand{\ite}[3]{\kw{if}~#1~\kw{then}~#2~\kw{else}~#3}
\newcommand{\case}[3]{\kw{case}~#1~\kw{of}~[#2, #3]~}
\newcommand{\alloc}[1]{\kw{alloc}(#1)}
\newcommand{\free}[2]{\kw{free}(#1, #2)}
\newcommand{\poison}{\text{\Biohazard}\xspace}
\newcommand{\rbot}{\ensuremath{\bot}\xspace}
\newcommand{\naderef}[1]{{}^{\ast\texttt{na}}#1}
\newcommand{\naassign}[2]{#1 :=_{\texttt{na}}#2}


% Operational

\newcommand\hp{\ensuremath{h}\xspace}
\newcommand\hpapp{\ensuremath{\texttt{+}}\xspace}
\newcommand\rexpr{\ensuremath{e}\xspace}
\newcommand\cnt{\ensuremath{c}\xspace}
\newcommand\fenv{\ensuremath{G}\xspace}
% \newcommand\interpctx[3]{\ensuremath{#1 \in [\!|#2;#3|\!]}\xspace}
\newcommand\interp[1]{\ensuremath{[\!|#1|\!]}\xspace}
\newcommand\trans[1]{\ensuremath{#1}\xspace}
\newcommand\goesto[6]{\ensuremath{\langle#1,#2,#3\rangle \rightsquigarrow^{\star} \langle#4,#5,#6\rangle }\xspace}
\newcommand\eval[6]{\ensuremath{\langle#1,#2,#3\rangle \rightsquigarrow \langle#4,#5,#6\rangle }\xspace}
\newcommand\evalerr[3]{\ensuremath{\langle#1,#2,#3\rangle \rightsquigarrow \memerr}\xspace}
\newcommand\evalstm[5]{\ensuremath{\langle#1,#2, #3\rangle \rightsquigarrow \langle#4, #5\rangle }\xspace}
\newcommand\evalstmerr[3]{\ensuremath{\langle#1,#2, #3\rangle \rightsquigarrow \memerr }\xspace}
\newcommand\memerr{\ensuremath{\texttt{ERR}}\xspace}
\newcommand\syntaxcat[1]{\textit{\textbf{#1}}} % syntax category

% Programs
\newcommand\rval{\ensuremath{\mathit{rv}}\xspace}
\newcommand\aval{\ensuremath{\mathit{av}}\xspace}
\newcommand\lval{\ensuremath{\mathit{lv}}\xspace}
\newcommand\cst{\ensuremath{c}\xspace}
\newcommand\place{\ensuremath{p}\xspace}
%\newcommand\place{\ensuremath{\xx}\xspace}
\newcommand\stmt{\ensuremath{S}\xspace}
\newcommand\fbody{\ensuremath{F}\xspace}
\newcommand\ffbody{\ensuremath{F}\xspace}
\newcommand\ddef{\ensuremath{\mathit{D}}\xspace}
\newcommand\pdef{\ensuremath{\mathit{P}}\xspace}
\newcommand\fdef[4]{\ensuremath{\kw{fn}\ {#1}({#2})~\kw{ret}~#3~\{#4\} }\xspace}
\newcommand\rvcopy[1]{\ensuremath{\kw{copy}~ #1 }\xspace}
\newcommand\rvmove[1]{\ensuremath{\kw{move}~ #1 }\xspace}
\newcommand\rvshrref[1]{\ensuremath{\&\textbf{shr}~#1}\xspace}
\newcommand\rvmutref[1]{\ensuremath{\&\textbf{mut}~#1}\xspace}
\newcommand\rvstrgref[1]{\ensuremath{\&\textbf{strg}~#1}\xspace}
\newcommand\deref[1]{\ensuremath{\ast #1}\xspace}
\newcommand\cloc{\ensuremath{\ell}\xspace}

% Constants
\newcommand\ctrue{\ensuremath{\kw{true}}\xspace}
\newcommand\cfalse{\ensuremath{\kw{false}}\xspace}

% Statements
\newcommand\sskip{\ensuremath{\kw{skip}}\xspace}
\newcommand\sassign[2]{\ensuremath{#1 := #2}\xspace}
%\newcommand\smemcp[3][n]{\ensuremath{#2 :=_{#1} \kw{copy}~#3}}
\newcommand\smemcp[3][n]{\ensuremath{#2 :=_{#1} #3}}
\newcommand\smemmv[3][n]{\ensuremath{#2 :=_{#1} \kw{move}~#3}}
\newcommand\sdel[2]{\ensuremath{\kw{delete}(#1, #2)}}
\newcommand\sunpack[2]{\ensuremath{\kw{unpack}(#1, #2)}\xspace}

% Function Body
\newcommand\bseq[2]{\ensuremath{{#1}; {#2}}}
\newcommand\bjump[3]{\ensuremath{\kw{jump}~#1\langle#2\rangle(#3)}\xspace}
\newcommand\bjumphl[3]{\ensuremath{\kw{jump}~#1\highlight{\langle#2\rangle}(#3)}\xspace}
\newcommand\bif[3]{\ensuremath{\kw{if}\ {#1}\ \{ #2\}\ \kw{else}\ \{ #3\}}\xspace}
\newcommand\blet[3]{\ensuremath{\kw{let}~#1 = #2~\kw{in}~#3}\xspace}
\newcommand\bunpack[3]{\ensuremath{\kw{unpack}(#1, #2)~\kw{in}~#3}}
\newcommand\bcall[5]{\ensuremath{\kw{call}~#1\langle#3\rangle(#4)~\kw{ret}~#5}\xspace}
\newcommand\bcallhl[5]{\ensuremath{\kw{call}~#1\highlight{\langle#3\rangle}(#4)~\kw{ret}~#5}\xspace}
\newcommand\bletcont[4]{\ensuremath{\kw{letcont}~#1(#2)~=~#3~\kw{in}~#4}\xspace}
\newcommand\bnewlft[1]{\ensuremath{\kw{newlft}; #1}}
\newcommand\bendlft[1]{\ensuremath{\kw{endlft}; #1}}
\newcommand\new[1]{\ensuremath{\kw{new}(#1)}}

% Types
\newcommand\typ{\ensuremath{\tau}\xspace}
% \newcommand\uninit[1]{\ensuremath{\lightning_{\hspace{-0.2ex}#1}}\xspace}
\newcommand\uninit[1]{\ensuremath{\lightning}\xspace}
\newcommand\rtyp[2]{\ensuremath{{#1}\langle {#2}\rangle}\xspace}
\newcommand\texists[3]{\ensuremath{\{#1.\; #2 \mid #3\}}\xspace}
\newcommand\tvar{\ensuremath{T}\xspace}
\newcommand\tucon{\ensuremath{c}\xspace}
\newcommand\tcon{\ensuremath{B}\xspace}
\NewDocumentCommand\bty{o}{
  \ensuremath{
    \IfValueTF{#1}{\rtyp{B}{#1}}{B\xspace}
  }
}
\newcommand\flft{{\digammaup}}
\newcommand\tpolycont[5]{\ensuremath{\forall #1.~\tcont{#2}{#3}{#4}{#5}}}
\newcommand\tcont[4]{\ensuremath{\kw{cont}(#1; \lftonly{#2;} #3.\,#4)}\xspace}
\newcommand\constr{\ensuremath{C}\xspace}
\newcommand\sig{\ensuremath{\mathit{s}}\xspace}
% \newcommand\polysig[9]{\ensuremath{\forall \lftonly{#1,}#2,#3.~\kw{fn}(#4; \lftonly{\flft : #5;~}#6.~#7) \rightarrow #8.~#9}\xspace}
% \newcommand\polysig[9]{\ensuremath{\forall #2.~\kw{fn}(#3; \lftonly{\flft : #4;~}#5; #6.~#7) \rightarrow #8.~#9}\xspace}
\newcommand\polysig[7]{
  \ensuremath{\forall #2.~ \kw{fn}(#3; #4; #5) \rightarrow #6 / #7}\xspace
}
\newcommand\layout{\ensuremath{\eta}\xspace}

% layouts
\newcommand\lblock[1]{\ensuremath{#1}}

% references
\newcommand\tptr[1]{\ensuremath{\kw{ptr}(#1)}\xspace}
\newcommand\tbor[3]{\ensuremath{\&\lftonly{^{#1}}_{#2}~{#3}}}        % borrowed reference
\newcommand\shr{\ensuremath{\kw{shr}}\xspace}
\newcommand\mut{\ensuremath{\kw{mut}}\xspace}
\newcommand\strg{\ensuremath{\kw{strg}}\xspace}
\newcommand\lft{\ensuremath{\kappa}\xspace}
\newcommand\fleft{\ensuremath{\kappa}\xspace}
\newcommand\static{\ensuremath{\kw{static}}\xspace}
\newcommand\bormode{\ensuremath{\mu}\xspace}                         % borrowing mode

% type constructors
\NewDocumentCommand\tint{d<>}{
  \ensuremath{
    \IfValueTF{#1}
      {\rtyp{\kw{int}}{#1}}
      {\kw{int}\xspace}
  }
}
\NewDocumentCommand\tbool{d<>}{
  \ensuremath{
    \IfValueTF{#1}
    {\rtyp{\kw{bool}}{#1}}
    {\kw{bool}}
  }
\xspace}
% \newcommand\tvec[1]{\ensuremath{\kw{vec}\langle{#1}\rangle}\xspace}
\newcommand\conrvec{\ensuremath{\kw{vec}_{\typ}}\xspace}
\newcommand\rvec[1]{\ensuremath{\conrvec\langle{#1}\rangle}\xspace}

% Expressions
\newcommand{\val}{\ensuremath{v}\xspace}
\newcommand\ee{\ensuremath{e}\xspace}
\newcommand\CC{\ensuremath{C}\xspace}
\newcommand\expr{\ensuremath{r}\xspace}
\newcommand\sort{\ensuremath{\sigma}\xspace}
\newcommand\etrue{\ensuremath{\textlog{true}}\xspace}
\newcommand\efalse{\ensuremath{\textlog{false}}\xspace}

% Sorts
\newcommand\sint{\ensuremath{\mathbf{int}}\xspace}
\newcommand\sbool{\ensuremath{\mathbf{bool}}\xspace}
\newcommand\styp{\ensuremath{\mathbf{type}}\xspace}
\newcommand\sloc{\ensuremath{\mathbf{loc}}\xspace}
\newcommand\slft{\ensuremath{\mathbf{lft}}\xspace}

% Function variable
\newcommand\ff{\ensuremath{f}\xspace}
\newcommand\fmain{\ensuremath{main}\xspace}

% Continuation variable
\newcommand\kk{\ensuremath{k}\xspace}

% Program variables
\newcommand\xx{\ensuremath{x}\xspace}
\newcommand\yy{\ensuremath{y}\xspace}
\newcommand\zz{\ensuremath{z}\xspace}

% Ghost variables
%\renewcommand\aa{\ensuremath{v}\xspace}
% \newcommand\ii{\ensuremath{\iota}\xspace}
\renewcommand\aa{\ensuremath{a}\xspace}
\newcommand\bb{\ensuremath{b}\xspace}
\newcommand\lvar{\ensuremath{\rho}\xspace}
\newcommand\lret{\ensuremath{\rho_\text{o}}\xspace}

% Lifetime variables
\newcommand\lftvar{\ensuremath{\alpha}\xspace}


%%%%%%%%%%%%%%%%%%
%% Environments %%
%%%%%%%%%%%%%%%%%%
\newcommand\varcx{\ensuremath{\mathbf{\Delta}}\xspace}                         % variable context
\newcommand\loccx{\ensuremath{\mathbf{T}}\xspace}                     % location context
\newcommand\kenv{\ensuremath{\mathbf{K}}\xspace}                      % continuation context
\newcommand\genv{\ensuremath{\mathbf{\Sigma}}\xspace}                          % global environment
\newcommand\elftcx{\ensuremath{\mathbf{E}}\xspace}                    % external lifetime context
\newcommand\llftcx{\ensuremath{\mathbf{L}}\xspace}                    % local lifetime context
\newcommand\elftinc[2]{\ensuremath{#1 \sqsubseteq_{\text{e}} #2}}     % external lifetime inclusion
\newcommand\llftinc[2]{\ensuremath{#1 \sqsubseteq_{\text{l}} #2}}     % local lifetime inclusion
\newcommand{\mapstoenv}[2]{\ensuremath{{#1}\text{:} {#2}}}           % owned maps to
\newcommand{\mapstoowned}[2]{\ensuremath{{#1}\mapsto {#2}}}           % owned maps to
\newcommand{\mapstoblocked}[3][\lft]{                                 % blocked maps to
  % \ensuremath{#2 \oset[0.2ex]{\ensuremath{\dagger{#1}}}{\mapsto} #3}}
  \ensuremath{#2 \fmapsto[\ensuremath{\dagger{#1}}] #3}}

%%%%%%%%%%%%%%%%
%% judgments %%
%%%%%%%%%%%%%%%%

\newenvironment{judgment}[2]{\begin{mathpar}\judgmentheader{#1}{#2}\\}{\end{mathpar}}
\newcommand\judgmentheader[2]{\textbf{#1}\hfill{\fbox{#2}}}

% Well-formedness
\newcommand\wfvdash{\ensuremath{\vdash_{\texttt{wf}}}}
\NewDocumentCommand\wf{O{\varcx}m}{\ensuremath{#1 \wfvdash #2}}
\NewDocumentCommand\wfvarcx{m}{\ensuremath{\wfvdash #1}}
\NewDocumentCommand\sortck{O{\varcx}mm}{\ensuremath{#1 \vdash #2 : #3 }}                          % sort checking

\newcommand\fresh[2]{\ensuremath{\text{fresh}_{#2}\ {#1} }}

\newcommand\isloc[1]{\ensuremath{\text{\isMemLocName(#1)}}\xspace}
\newcommand\isMemLocName{\ensuremath{\text{isMemLoc}}\xspace}
\newcommand\ownVecName{\ensuremath{\text{OwnVec}}\xspace}
\newcommand\ownVec[4]{\ensuremath{\text{\ownVecName(#1, #2, #3, #4)}}\xspace}

% Checking judgments
\newcommand\defck[2]{\ensuremath{#1 \vdash #2}}                                                   % function definition checking
\NewDocumentCommand\bodyck{ommmmmm}{                                                              % function body checking
  \ensuremath{\IfValueTF{#1}{#1;}{} #2\mid \lftonly{#3; #4 \mid} #5; #6 \vdash \ensuremath{#7}}}
\NewDocumentCommand\stmtck{O{\varcx}O{\elftcx}O{\llftcx}mmm}{                                    % statement checking
  \ensuremath{#1 \mid \lftonly{#2; #3 \mid} #4 \vdash #5 \dashv #6}}
\NewDocumentCommand\rvalck{O{\varcx}O{\elftcx}O{\llftcx}mmmm}{                                    % r-value checking
  \ensuremath{#1 \mid \lftonly{#2; #3 \mid} #4 \vdash #5 \rightsquigarrow #6 \dashv #7}}

\NewDocumentCommand\subtyping{O{\varcx}O{\elftcx}O{\llftcx}mm}{                                   % subtyping
  \ensuremath{#1 \lftonly{\mid #2; #3} \vdash #4 \preccurlyeq #5}}
% \newcommand\entailment[2]{\ensuremath{\llbracket #1 \vdash #2 \rrbracket}}
\newcommand\entailment[2]{\lmodel{#1}{#2}}

% Type copying, moving, writing and borrowing
\NewDocumentCommand\typcopying{O{\elftcx}O{\llftcx}mmm}{                                           % type coyping
  \ensuremath{\lftonly{#1; #2 \mid} #3 \vdash #4 \oset{cp}{\rightsquigarrow} #5}}
\NewDocumentCommand\typmoving{mmmm}{                                                               % type moving
  \ensuremath{#1 \vdash #2 \oset{mv}{\rightsquigarrow} #3 \dashv #4}}
\NewDocumentCommand{\typborrowing}{O{\elftcx}O{\llftcx}mmmmm}{                                     % type borrowing
  \ensuremath{\lftonly{#1; #2 \mid} #4 \vdash #5 \oset[0.3ex]{\&#3}\rightsquigarrow #6 \dashv #7}}
\NewDocumentCommand\typwriting{O{\varcx}O{\elftcx}O{\llftcx}mmmm}{                                 % type writing
  \ensuremath{#1 \mid \lftonly{#2; #3 \mid} #4 \vdash #5 \leftsquigarrow #6 \dashv #7}}

% Lifetime judgments
\NewDocumentCommand\alive{O{\elftcx}O{\llftcx}m}{                          % lifetime liveness
  \ensuremath{#1; #2 \vdash #3~\text{alive}}}
\newcommand\elftcxsat[4]{\ensuremath{#1 \mid #2; #3 \vdash #4}}            % external lifetime context satisfaction
\NewDocumentCommand\lftinc{O{\elftcx}O{\llftcx}mm}{                        % lifetime inclusion
  \ensuremath{#1; #2 \vdash #3 \sqsubseteq #4}}
\newcommand\loccxunblocking[3]{\ensuremath{#1 \Rightarrow^{\dagger#2} #3}} % location context unblocking
\newcommand\loccxinc[5]{                                                   % location context inclusion
  \ensuremath{#1 \lftonly{\mid #2; #3} \vdash #4 \Rightarrow #5}}
\newcommand\llftcxinc[3][\Delta]{                                          % local lifetime context inclusion
  \ensuremath{#1 \vdash #2 \Rightarrow #3}}
\newcommand\kenvinc[4][\Delta]{                                            % continuation context inclusion
  \ensuremath{#1 \mid #2 \vdash #3 \Rightarrow #4}}

%%%%%%%%%%%%%%%%
%% Rule Names %%
%%%%%%%%%%%%%%%%

% Statements
\newcommand\rulename[1]{\ensuremath{\textsc{#1}}\xspace}

\newcommand\tpgs{\rulename{T-Pgs}}
\newcommand\tpg{\rulename{T-Pg}}
\newcommand\tdef{\rulename{T-Def}}
\newcommand\tskip{\rulename{T-skip}}
\newcommand\tassign{\rulename{T-assign}}
\newcommand\tassignstrg{\rulename{T-assign-strg}}
\newcommand\tunpack{\rulename{T-unpack}}
\newcommand\tcall{\rulename{T-call}}
\newcommand\pvar{\rulename{P-var}}
\newcommand\pptr{\rulename{P-Ptr}}
\newcommand\ttvar{\rulename{T-var}}
\newcommand\tfun{\rulename{T-fun}}
\newcommand\tsub{\rulename{T-sub}}
\newcommand\ttptr{\rulename{T-ptr}}
\newcommand\tumem{\rulename{T-mem}}
\newcommand\tvecnew{\rulename{T-vec-new}}
\newcommand\tvecpush{\rulename{T-vec-push}}
\newcommand\tvecindexmut{\rulename{T-vec-index-mut}}
\newcommand\tvecvec{\rulename{T-vec}}
\newcommand\twfidx{\rulename{WF-Idx}}
\newcommand\twfex{\rulename{WF-Ex}}
\newcommand\twfptr{\rulename{WF-Ptr}}
\newcommand\twfref{\rulename{WF-Ref}}
\newcommand\twfmem{\rulename{WF-Mem}}
\newcommand\twffun{\rulename{WF-Fun}}
\newcommand\twfemp{\rulename{WF-Emp}}
\newcommand\twfbind{\rulename{WF-Bind}}

% Rvalues
\newcommand\tconstint{\rulename{T-int}}
\newcommand\ttrue{\rulename{T-true}}
\newcommand\tfalse{\rulename{T-false}}
\newcommand\tcopy{\rulename{T-copy}}
\newcommand\tmove{\rulename{T-move}}
\newcommand\tdel{\rulename{T-del}}
\newcommand\tborshr{\rulename{T-bor-shr}}
\newcommand\tbormut{\rulename{T-bor-mut}}

% Function body checking
\newcommand\tconsequence{\rulename{T-consequence}}
\newcommand\tseq{\rulename{T-Seq}}
\newcommand\tif{\rulename{T-If}}
\newcommand\tlet{\rulename{T-Let}}
\newcommand\tnew{\rulename{T-New}}
\newcommand\tjump{\rulename{T-Jump}}
\newcommand\tletcont{\rulename{T-Cont}}
\newcommand\tnewlft{\rulename{T-Newlft}}
\newcommand\tendlft{\rulename{T-Endlft}}

% Type coyping, moving and borrowing
\newcommand\tcopyown{\rulename{T-copy-own}}
\newcommand\tcopybor{\rulename{T-copy-bor}}
\newcommand\tcopyptr{\rulename{T-copy-ptr}}
\newcommand\tmoveown{\rulename{T-move-own}}
\newcommand\tmoveptr{\rulename{T-move-ptr}}
\newcommand\tborown{\rulename{T-bor-own}}
\newcommand\tborptr{\rulename{T-bor-ptr}}
\newcommand\tborrebor{\rulename{T-rebor}}
\newcommand\twriteown{\rulename{T-write-own}}
\newcommand\twriteptr{\rulename{T-write-ptr}}
\newcommand\twritebor{\rulename{T-write-bor}}

% Subtyping
\newcommand\subptr{\rulename{S-Ptr}}
\newcommand\subrref{\rulename{S-Ref}}
\newcommand\submem{\rulename{S-Mem}}
\newcommand\subfun{\rulename{S-Fun}}
\newcommand\subrtyp{\rulename{S-RType}}
\newcommand\subunpack{\rulename{S-Unpack}}
\newcommand\subexists{\rulename{S-Exists}}
\newcommand\subborlft{\rulename{S-Bor-Lft}}
\newcommand\subborshr{\rulename{S-Bor-Shr}}
\newcommand\subbormut{\rulename{S-Bor-Mut}}
\newcommand\subreflcon{\rulename{S-Con-Refl}}
\newcommand\subvec{\rulename{S-Vec}}
\newcommand\loccxinctrans{\rulename{C-Trans}}
\newcommand\loccxincperm{\rulename{C-Perm}}
\newcommand\loccxincweaken{\rulename{C-Weaken}}
\newcommand\loccxincframe{\rulename{C-Frame}}
\newcommand\loccxincsub{\rulename{C-Sub}}
\newcommand\loccxincbor{\rulename{C-Bor}}
\newcommand\loccxincblock{\rulename{C-Block}}

% Heaplet typing
\newcommand\hptracked{\rulename{Hp-tracked}}
\newcommand\hpuntracked{\rulename{Hp-untracked}}

% Stack typing
\newcommand\hpshr{\rulename{S-Shr}}
\newcommand\hpshrmut{\rulename{S-Shr-Mut}}
\newcommand\hpmut{\rulename{S-Mut}}
\newcommand\hpmutstrg{\rulename{S-Mut-Strg}}
\newcommand\hpstrg{\rulename{S-Strg}}
\newcommand\hpempty{\rulename{S-Empty}}
\newcommand\hpdisabled{\rulename{S-Disabled}}

% Stcked borrows
\newcommand\osalloc{\rulename{OS-alloc}}
\newcommand\osdealloc{\rulename{OS-dealloc}}
\newcommand\osaccess{\rulename{OS-access}}
\newcommand\osretag{\rulename{OS-retag}}

%%%%%%%%%%
%% Misc %%
%%%%%%%%%%
\newcommand\iscopy[1]{\ensuremath{#1~\texttt{copy}}}
\newcommand\getsort[1]{\ensuremath{\texttt{sort}(#1)}}
\newcommand\substvar{\ensuremath{\theta}\xspace}
\newcommand\subst[2]{\ensuremath{[#2 / #1]}\xspace}
\newcommand\applysubst[2]{\ensuremath{#1\cdot #2}}
\newcommand\embed[1]{\ensuremath{\llbracket #1 \rrbracket}}
\newcommand\sizeof[1]{\ensuremath{\texttt{size}(#1)}}
\newcommand\layoutof[1]{\ensuremath{\texttt{layout}(#1)}}
\newcommand\emptylist{\ensuremath{[]}}
\newcommand\modeord[2]{\ensuremath{#1 \preceq #2}}

\newcommand\lambdarust{\ensuremath{\lambda_{\text{Rust}}}\xspace}
\newcommand\corelan{\ensuremath{\lambda_{\text{LR}}}\xspace}
\newcommand\coretarget{\ensuremath{\lambda_{\text{T}}}\xspace}

% Operational judgments

\newcommand\intEmp{\rulename{I-Emp}}
\newcommand\intIdx{\rulename{I-Idx}}
\newcommand\intEx{\rulename{I-Ex}}
\newcommand\intPtr{\rulename{I-Ptr}}
\newcommand\intMut{\rulename{I-Mut}}
\newcommand\intShr{\rulename{I-Shr}}
\newcommand\intUnin{\rulename{I-Unin}}
\newcommand\opnew{\rulename{O-New}}
\newcommand\opnewerr{\rulename{O-New-Err}}
\newcommand\opprop{\rulename{O-Prop}}
\newcommand\opproperr{\rulename{O-Prop-Err}}
\newcommand\oplet{\rulename{O-Let}}
\newcommand\opcnt{\rulename{O-Cont}}
\newcommand\opseq{\rulename{O-Seq}}
\newcommand\opskip{\rulename{O-Skip}}
\newcommand\opseqerr{\rulename{O-Seq-Err}}
\newcommand\opifprop{\rulename{O-If-Prop}}
\newcommand\opifTrue{\rulename{O-If-True}}
\newcommand\opifFalse{\rulename{O-If-False}}
\newcommand\opjump{\rulename{O-Jump}}
\newcommand\opcall{\rulename{O-Call}}
\newcommand\opcallprop{\rulename{O-Call-Prop}}
\newcommand\opunpack{\rulename{O-UnPack}}
\newcommand\opass{\rulename{O-Assign}}
\newcommand\opasserr{\rulename{O-Assign-Err}}
\newcommand\opassrval{\rulename{O-Assign-rval}}
\newcommand\opassptr{\rulename{O-Assign-Ptr}}
\newcommand\opstrgrebor{\rulename{O-Strg-Rebor}}
\newcommand\opmutrebor{\rulename{O-Mut-Rebor}}
\newcommand\opshrrebor{\rulename{O-Shr-Rebor}}
\newcommand\opderef{\rulename{O-Deref}}
\newcommand\opdass{\rulename{O-DAssign}}
\newcommand\opcopy{\rulename{O-Copy}}
\newcommand\opmove{\rulename{O-Move}}
\newcommand\opvecpush{\rulename{O-Vec-push}}
\newcommand\opvecpushempty{\rulename{O-Vec-push-empty}}
\newcommand\opvecnew{\rulename{O-Vec-new}}
\newcommand\opvecindexmut{\rulename{O-Vec-index-mut}}
\newcommand\htsub{\rulename{HT-Sub}}
\newcommand\hbind[2]{\ensuremath{[#1 \mapsto #2]}}
\newcommand\hval{\ensuremath{v}}
\newcommand\hsingle[2]{\ensuremath{[#1 \mapsto #2]}}
\newcommand\hbindn[3]{\ensuremath{[#2 \mapsto_{#1} #3]}}
\newcommand\cntbind[2]{\ensuremath{[#1 \mapsto #2]}}
\newcommand\evals[2]{\ensuremath{ #1 \rightsquigarrow^{\ast} #2 }}
\newcommand\tstrgrebor{\rulename{T-Strg-Rebor}}
\newcommand\tstrgmutrebor{\rulename{T-Strg-Mut-Rebor}}
\newcommand\tmutmutrebor{\rulename{T-Mut-Rebor}}
\newcommand\tderef{\rulename{T-Deref}}
\newcommand\tderefstrg{\rulename{T-Deref-Strg}}
\newcommand\trvalval{\rulename{T-Rval-val}}
\newcommand\tshrrebor{\rulename{T-Shr-Rebor}}


\newcommand\hastype[3]{\ensuremath{#1 \vdash #2 : #3}\xspace}

% Denotational judgments
\newcommand\defden[2]{\ensuremath{#1 \models #2}}                                                   % function definition checking
\newcommand\lmodel[2]{\ensuremath{#1 \models #2}}                                                   % function definition checking

\NewDocumentCommand\bodyden{ommmmmm}{                                                              % function body checking
  \ensuremath{\IfValueTF{#1}{#1;}{} #2\mid \lftonly{#3; #4 \mid} #5; #6 \models \ensuremath{#7}}}

%%%%%%%%%%%%%%%%%%%%
%% Semantic model %%
%%%%%%%%%%%%%%%%%%%%
\newcommand\TId{\textdom{TId}\xspace}
\newcommand\Lft{\textdom{Lft}\xspace}
\newcommand\listtycon[1]{\ensuremath{\mathit{list}(#1)}\xspace}
\newcommand\thread{\ensuremath{t}\xspace}
\newcommand{\fullborrow}[2]{\ensuremath{\&^{#1}_{\textbf{full}} #2}}
\newcommand{\fracborrow}[2]{\ensuremath{\&^{#1}_{\textbf{frac}} #2}}
\newcommand\lftnamesp{\ensuremath{\namesp_{\text{lft}}}}
\newcommand\shrnamesp{\ensuremath{\namesp_{\text{shr}}}}
\newcommand\lftvs{\ensuremath{\vs[\namesp_{\text{lft}}]}}
\NewDocumentCommand{\lfttk}{om}{  % lifetime token
  \IfValueTF{#1}{[#2]_{#1}}{[#2]}
}
\NewDocumentCommand{\deadtk}{m}{[\dagger#1]}
\newcommand{\semsubtyping}[2]{\ensuremath{#1 \sqsubseteq^{\text{ty}} #2}} % semantic subtyping
\newcommand{\semsize}[1]{\ensuremath{#1.\texttt{size}}}
\newcommand\isize{\ensuremath{\texttt{size}}\xspace}
\newcommand\iown{\ensuremath{\texttt{own}}\xspace}
\NewDocumentCommand\ownlambda{O{\thread}O{\overline{\val}}m}{\ensuremath{\lambda \thrdonly{#1,} #2.\,#3}}
\NewDocumentCommand\baseownlambda{O{\val}O{\thread}O{\overline{\val}}m}{\ensuremath{\lambda #1, \thrdonly{#2,} #3.\,#4}}
\NewDocumentCommand\shrlambda{O{\lft}O{\thread}O{\loc}m}{\ensuremath{\lambda #1, \thrdonly{#2,} #3.\,#4}}
\NewDocumentCommand\baseshrlambda{O{\val}O{\lft}O{\thread}O{\loc}m}{\ensuremath{\lambda #1, \thrdonly{#2,} #3, #4.\,#5}}

\NewDocumentCommand{\semown}{smoo}{
  \ensuremath{
    \IfBooleanTF{#1}{\semtyp{#2}}{#2}.\texttt{own}
    \IfValueT{#3}{
      \IfValueTF{#4}
        {(\thrdonly{#3,} #4)}
        {\thrdonly{(#3)}}
    }
  }
}
\NewDocumentCommand{\semtconown}{mooo}{
  \ensuremath{
    #1.\texttt{own}
    \IfValueT{#2}{
      \IfValueTF{#3}{
        \IfValueTF{#4} {
          (#2 \thrdonly{, #3}, #4)
        }{
          \texttt{own}(#2 \trhdonly{, #3})
        }
      }{
        \texttt{own}(#2)
      }
    }
  }
}

\NewDocumentCommand{\semshr}{smooo}{
  \ensuremath{
    \IfBooleanTF{#1}{\semtyp{#2}}{#2}.\texttt{shr}
    \IfValueT{#3}{
      \IfValueTF{#4}{
        \IfValueTF{#5}
          {(#3\thrdonly{, #4}, #5)}
          {(3\thrdonly{, #4})}
      }{
        \texttt{shr}(#3)
      }
    }
  }
}
\NewDocumentCommand{\semtconshr}{moooo}{
  \IfValueTF{#2}{
    \IfValueTF{#3}{
      \IfValueTF{#4}{
        \IfValueTF{#5}{
           \ensuremath{#1.\texttt{shr}(#2\thrdonly{, #3}, #4, #5)}
        }{
           \ensuremath{#1.\texttt{shr}(#2\thrdonly{, #3}, #4)}
        }
      }{
        \ensuremath{#1.\texttt{shr}(#2\thrdonly{, #3})}
      }
    }{
      \ensuremath{#1.\texttt{shr}(#2)}
    }
  }{
    \ensuremath{#1.\texttt{shr}}
  }
}
\newcommand\simpletype[1]{\ensuremath{\text{SimpleType}(#1)}}
\newcommand\singleton[1]{\ensuremath{\text{Singleton}(#1)}}
\newcommand\selfty[2]{\ensuremath{#1}}
% \newcommand\selfty[2]{\ensuremath{\text{Self}(#1,#2)}}
\newcommand\seminterp[1]{\ensuremath{\llbracket #1\rrbracket}}
\newcommand\locinterp[2][\gamma]{\ensuremath{\llbracket #2\rrbracket_{#1}}}


\NewDocumentCommand\semtyp{O{\gamma}m}{\ensuremath{\seminterp{#2}_{#1}}}
\NewDocumentCommand\semsig{O{\gamma}mO{\loc}}{\ensuremath{\seminterp{#2}_{#1}(#3)}}
\NewDocumentCommand\semgenv{O{\gamma}m}{\ensuremath{\seminterp{#2}_{#1}}}
\NewDocumentCommand\semexpr{O{\gamma}m}{\ensuremath{\seminterp{#2}_{#1}}}
\NewDocumentCommand\semloccx{O{\gamma}mO{\thread}}{\ensuremath{\seminterp{#2}_{#1}\thrdonly{(#3)}}}
\NewDocumentCommand\semkenv{mO{\thread}}{\ensuremath{\seminterp{#1}\thrdonly{(#2)}}}
\NewDocumentCommand\semllftcx{O{\gamma}mO{q}}{\ensuremath{\seminterp{#2}_{#1}(#3)}}
\NewDocumentCommand\semloc{mO{\gamma}}{\ensuremath{\seminterp{#1}_{#2}}}
\NewDocumentCommand\semlft{O{\gamma}m}{\ensuremath{\seminterp{#2}_{#1}}}
\NewDocumentCommand\semcont{O{\gamma}m}{\ensuremath{\seminterp{#2}_{#1}}}
\NewDocumentCommand\sembodyck{O{\gamma}mmmmm}{
  \ensuremath{\seminterp{#2; #3 \mid #4; #5 \vdash \ensuremath{#6}}}_{#1}}
\NewDocumentCommand\semelftcx{O{\gamma}m}{\ensuremath{\seminterp{#2}_{#1}}}
\NewDocumentCommand\semft{O{\gamma}m}{\ensuremath{\seminterp{#2}_{#1}}}
\NewDocumentCommand\semelftcxsat{O{\gamma}mmm}{\ensuremath{\seminterp{#2;#3 \vdash #4}_{#1}}}
\NewDocumentCommand\semlftinc{O{\gamma}mmmm}{\ensuremath{\seminterp{#2;#3 \vdash #4 \sqsubseteq #5}_{#1}}}
\NewDocumentCommand\semalive{O{\gamma}mmm}{\ensuremath{\seminterp{#2;#3 \vdash #4~\text{alive}}_{#1}}}

\newcommand\Type[3]{
  {
  \arraycolsep=1pt
  \begin{array}[t]{llll}
    \text{Type}&\{ & \text{size} & := {#1} \\
               & ; & \text{own}  & := {#2} \\
               & ; & \text{shr}  & := {#3} \\
               & \}
  \end{array}
  }
}
\newcommand\TypeCon[4]{
  {
  \arraycolsep=1pt
  \begin{array}[t]{lllll}
    \text{TypeCon} &\{ & \text{sort} & := {#1} \\
                   & ; & \text{size} & := {#2} \\
                   & ; & \text{own}  & := {#3} \\
                   & ; & \text{shr}  & := {#4}  \\
                   & \}
  \end{array}
  }
}



\newcommand\defeq{\ensuremath{\doteq}}



\newcommand{\highlight}[2][lightgray]{\mathchoice%
  {\colorbox{#1}{$\displaystyle#2$}}%
  {\colorbox{#1}{$\textstyle#2$}}%
  {\colorbox{#1}{$\scriptstyle#2$}}%
  {\colorbox{#1}{$\scriptscriptstyle#2$}}}%

%%%%%%%%%%
%% Text %%
%%%%%%%%%%
\Crefname{section}{\S}{\SS}
\Crefname{subsection}{\S}{\SS}
\Crefname{subsubsection}{\S}{\SS}
\newcommand{\ANNOT}{14\%\xspace}
\newcommand{\kmeans}{k-means\xspace}
\newcommand{\benchmark}[1]{#1\xspace}
\newcommand{\lang}[1]{\textsc{#1}}
\newcommand{\rust}{\lang{Rust}\xspace}
% \newcommand{\sys}{\textsc{LiquidRust}\xspace}
\newcommand{\sys}{\textsc{Flux}\xspace}
\newcommand{\csolve}{\textsc{Csolve}\xspace}
\newcommand{\dsolve}{\textsc{Dsolve}\xspace}
\newcommand{\prusti}{\textsc{Prusti}\xspace}
\newcommand{\ocaml}{Ocaml\xspace}
\newcommand{\viper}{\textsc{Viper}\xspace}
\newcommand{\rusthorn}{\textsc{RustHorn}\xspace}
\newcommand{\whyml}{\textsc{WhyML}\xspace}
\newcommand{\rustbelt}{\textsc{RustBelt}\xspace}
\newcommand{\refinedc}{\textsc{RefinedC}\xspace}
\newcommand{\iris}{\textsc{Iris}\xspace}
\newcommand{\oxide}{\textsc{Oxide}\xspace}
\newcommand{\creusot}{\textsc{Creusot}\xspace}

\newcommand{\fstar}{F$^*$\xspace}
\NewDocumentCommand{\rtyptt}{smd<>o}{
  \texttt{\IfBooleanTF{#1}{#2}{\color{entity.name.type}#2}}\IfValueT{#3}{\ensuremath{\texttt{<}#3\texttt{>}}}\IfValueT{#4}{\ensuremath{\texttt{\{}#4\texttt{\}}}}
}
\NewDocumentCommand{\tvartt}{s}{\texttt{\IfBooleanTF{#1}{T}{\color{entity.name.type}T}}\xspace}
\NewDocumentCommand{\vartt}{sm}{\texttt{\IfBooleanTF{#1}{#2}{\color{variable}#2}}}

\newcommand\coderule{\rule{\textwidth}{0.6pt}\xspace}

\NewDocumentCommand\fcall{smmmm}{
\ensuremath{
  \kw{call}~#2
  \ifthenelse{\equal{#4}{}}{}{\IfBooleanTF{#1}{\highlight{\langle#4\rangle}}{\langle#4\rangle}}
  (#5)
}\xspace
}
\newcommand\eunpack[3]{\ensuremath{\kw{unpack}(#1, #2)~\kw{in}~#3}}
\newcommand\vrec[4]{\ensuremath{\kw{rec}~#1\langle #2\rangle(#3)~:=~#4}}
\newcommand\evalue{v\xspace}
\newcommand\enew[1]{\ensuremath{\kw{new}(#1)}}
\newcommand\loc{\ensuremath{\eta}\xspace}
\newcommand\sbstate{\ensuremath{\varsigma}\xspace}


%% STACKED BORROWS
\newcommand\evalloc[3]{\ensuremath{\text{EAlloc}(\text{Pointer}(#1, #2), #3})}
\newcommand\evretag[6]{\ensuremath{\text{ERetag}(\text{Pointer}(#1, #2), #3, #4, #5, #6)}}
\newcommand\evaccess[4]{\ensuremath{\text{EAccess}(\text{#1, Pointer(#2, #3), #4})}}
\newcommand\evdealloc[3]{\ensuremath{\text{EDealloc}(\text{Pointer}(#1, #2), #3)}}
\newcommand\aread{\ensuremath{\text{AccessRead}}\xspace}
\newcommand\awrite{\ensuremath{\text{AccessWrite}}\xspace}
\newcommand\sbtrans[3]{\ensuremath{#1 \xrightarrow{#2} #3}}
\newcommand\ptrtag{\ensuremath{t}\xspace}
\newcommand\vptr[2]{\ensuremath{\text{ptr}(#1, #2)}}
\newcommand\fixedsize[1][n]{\ensuremath{\text{FixedSize}(#1)}\xspace}
\newcommand\retag[1]{\ensuremath{\kw{retag}(#1)}}

\newcommand{\typing}[8]{\ensuremath{#1 \mid #2; #3 \mid #4 \vdash_e #5: #6 \dashv #7}}
\newcommand{\pltyping}[7]{\ensuremath{\typing{#1}{#2}{#3}{#4}{#5}{#6}{#7}{}}}
\newcommand{\sttyping}[5]{\ensuremath{#1; #2; #3 \vdash #4 \dashv #5}}
\newcommand{\stmtyping}[7]{\ensuremath{#1 \mid #2; #3 \mid #4 \vdash_s #5 \dashv #6 }}
\newcommand{\rvaltyping}[7]{\ensuremath{#1 \mid #2; #3 \mid #4 \vdash_r #5: #6 \dashv #7}}
\newcommand{\valtyping}[6]{\ensuremath{#1 \mid #2 \mid #4 \vdash #5: #6}}
\newcommand{\env}{\ensuremath{\Gamma}\xspace}
\newcommand{\dynenv}{\ensuremath{\Sigma}\xspace}
\newcommand\tref[2]{\ensuremath{\&_{#1}~{#2}}}        % borrowed reference

\newcommand\transalloc[5]{\sbtrans{#1}{\evalloc{#2}{#3}{\fixedsize[#4]}}{#5}}
\newcommand\transnew[3][\cloc]{\sbtrans{#2}{\evalloc{#1}{\ptrtag}{\fixedsize[1]}}{#3}}
\newcommand\transreborrow[6]{\sbtrans{#1}{\evretag{#2}{#3}{#4}{\fixedsize[1]}{#5}{\Raw}}{#6}}
\newcommand\transread[4]{\sbtrans{#1}{\evaccess{\aread}{#2}{#3}{\fixedsize[1]}}{#4}}
\newcommand\transwrite[4]{
\sbtrans{#1}{\evaccess{\awrite}{#2}{#3}{\fixedsize[1]}}{#4}
}
\newcommand\transdealloc[5]{
\sbtrans{#1}{\evdealloc{#2}{#3}{\fixedsize[#4]}}{#5}
}
\newcommand\SbRef[1]{\ensuremath{\text{Ref}(#1)}}
\newcommand\Raw{\ensuremath{\text{Raw}}\xspace}

\newcommand\fv[1]{\text{FV}(#1)}
\newcommand\dom[1]{\text{dom}(#1)}

\NewDocumentCommand\stacktyping{O{\varcx}O{\dynenv}mmmm}
{\ensuremath{#1 \mid #4 \mapsto #6 \mid #2 \vdash_{#3} #5}}
\NewDocumentCommand\statetyping{O{\varcx}O{\loccx}O{\dynenv}mm}
{\ensuremath{#1 \mid #2 \mid #3 \vdash \langle#4,#5\rangle}}
\NewDocumentCommand\stackstyping{O{\varcx}O{\loccx}O{\dynenv}m}
{\ensuremath{#1 \mid #2 \mid #3 \vdash #4}}
\NewDocumentCommand\heaptyping{O{\varcx}O{\loccx}O{\dynenv}m}
{\ensuremath{#1 \mid #2 \mid #3 \vdash #4}}
\NewDocumentCommand\heaplettyping{O{\varcx}O{\loccx}O{\dynenv}mmm}
{\ensuremath{#1 \mid #2 \mid #3 \vdash \langle [#4 \mapsto #5], #6\rangle}}
\NewDocumentCommand\reftyping{O{\varcx}O{\loccx}mmm}
{\ensuremath{#1 \mid #2 \vdash [#3 \mapsto #4]: #5}}

\newcommand\stack{S}
\newcommand\stacks{\xi}

\newcommand\sharedro{\text{SharedRO}\xspace}
\newcommand\unique{\text{Unique}\xspace}
\newcommand\disabled{\text{Disabled}\xspace}
\newcommand\dotstacks{.\textsc{stacks}\xspace}


%% Vectors
\NewDocumentCommand{\vvec}{O{\typ}mm}
{\ensuremath{\kw{vec}_{#1}(#2, #3)}}
\NewDocumentCommand\tvec{O{\typ}d<>}
{\ensuremath{
   \IfValueTF{#2}
   {\rtyp{\kw{Vec}_{#1}}{#2}}
   {\kw{Vec}_{#1}}
}}
\NewDocumentCommand\vecpush{O{\typ}}
{\ensuremath{\tvec[#1]\kw{::push}}\xspace}
\NewDocumentCommand\vecnew{O{\typ}}
{\ensuremath{\tvec[#1]\kw{::new}}\xspace}
\NewDocumentCommand\vecindexmut{O{\typ}}
{\ensuremath{\tvec[#1]\kw{::index\_mut}}\xspace}

\makeatletter%
\@ifundefined{append}{%
\newcommand\append{\mathbin{+\kern-1.0ex+}}
}{}
\makeatother%

%% Sets
\newcommand{\Val}{\ensuremath{\mathit{Val}}\xspace}


==> metatheory/definitions.tex <==
\section{Auxiliary Definitions}

\subsection{Free Refinement Variables}
\[
\begin{array}{lcl}
    \text{\textbf{Expressions}} & & \\
     \fv{\blet{\xx}{e_1}{e_2}} & = & \fv{e_1} \cup \fv{e_2} \\
     \fv{\blet{\xx}{\new{\lvar}}{e}} & = & \fv{e} \setminus \{\lvar \}                                 \\
     \fv{\bif{\ee_1}{e_2}{e_3}} & = & \fv{e_1} \cup \fv{e_2} \cup \fv{e_3} \\
     \fv{\eunpack{\xx}{\aa}{e}} & = & \fv{e} \setminus \{\aa\} \\
     \fv{\fcall{e}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}} & = & \fv{e} \cup \bigcup_i \fv{\expr_i}\\
     \fv{\sassign{\place}{\ee}} & = & \fv{\ee} \\
     \fv{[\rvstrgref{\place}, \rvmutref{\place}, \rvshrref{\place}]} & = & \{\} \\
     \fv{\deref{\place}}  & = & \{\}\\
     \fv{\xx} & = & \{\} \\
     \fv{\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}}  & =& \fv{e} \setminus \{\overline{\aa}\}\\
     \fv{[\ctrue, \cfalse]} & = & \{\} \\
     \fv{0, \pm 1, \dots}  & = & \{\} \\
     \fv{\poison} & = & \{\}\\
     \fv{\vptr{\cloc}{\ptrtag}} & = & \{\} \\
     \fv{\vvec{n}{\val}} & = & \fv{\val} \\[0.5em]

    \text{\textbf{Types}} & & \\
    \fv{\rtyp{\tcon}{\expr}} & = & \fv{\expr}\\
    \fv{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}} & = & \fv{\expr} \setminus \{\aa\} \\
    \fv{\tptr{\loc}} & = & \fv{\loc}\\
    \fv{\tbor{\lft}{\bormode}{\typ}} & = & \fv{\typ}\\
    \fv{\uninit{n}} & = & \{\}\\
    \fv{\polysig{\overline{\tvar}}
    {{\overline{\aa: \sort}}}
    {{\expr}}
    {\loccx_i}
    {\overline{\typ}}
    {\typ_o}
    {\loccx_o}} & = & (\fv{\expr} \cup \fv{\loccx_i} \bigcup_i \fv{\typ_i} \cup \fv{\typ_o} \cup \fv{\loccx_o}) \setminus \{\overline{\aa}\}\\[0.5em]

    \text{\textbf{Refinements}} & & \\
    \fv{\aa}& = & \{\aa\} \\
    \fv{\expr_1 [=, \land, +, - , *] \expr_2}& = & \fv{\expr_1}\cup \fv{\expr_2} \\
    \fv{\lnot \expr}& = & \fv{\expr} \\
    \fv{[\ctrue,\cfalse,\cloc]}  &=& \{\} \\
    \fv{n}       &=& \{\} \quad n \in \mathbb{Z}\\[0.5em]

    \text{\textbf{Location Contexts}} & & \\
    \fv{\emptyset} & = & \emptyset \\
    \fv{\loccx, \mapstoowned{\loc}{\typ}} & = & \fv{\loccx} \cup \fv{\typ} \cup \fv{\loc} \\[0.5em]

    \text{\textbf{Value Contexts}} & & \\
    \fv{\emptyset} & = & \emptyset \\
    \fv{\env, \mapstoenv{\xx}{\typ}} & = & \fv{\env} \cup \fv{\typ} \\[0.5em]

    \text{\textbf{Dynamic Location Contexts}} & & \\
    \fv{\emptyset} & = & \emptyset \\
    \fv{\dynenv, \mapstoowned{(\cloc,\ptrtag)}{\typ}} & = & \fv{\dynenv} \cup \fv{\typ} \\
\end{array}
\]
\clearpage

\subsection{Type Substitution}
$$
\begin{array}{lcl}
    \text{\textbf{Types}} & & \\
    {\rtyp{\tcon}{\expr}}\subst{\aa}{\expr_\aa} & = & \rtyp{\tcon}{\expr\subst{\aa}{\expr_\aa}}\\
    {\texists{\bb}{\rtyp{\tcon}{\bb}}{\expr}}\subst{\aa}{\expr_\aa} & = & \left\{\begin{array}{ll}
        \texists{\bb}{\rtyp{\tcon}{\bb}}{\expr}, & \text{if } \bb = \aa\\
        \texists{\bb}{\rtyp{\tcon}{\bb}}{\expr\subst{\aa}{\expr_\aa}}, & \text{otherwise }
        \end{array}\right.\\
    {\tptr{\loc}}\subst{\aa}{\expr_\aa} & =  & \left\{\begin{array}{ll}
        \tptr{\expr_\aa}, & \text{if } \aa = \loc\\
        \tptr{\loc}, & \text{otherwise }
        \end{array}\right.\\
    ({\tbor{\lft}{\bormode}{\typ}})\subst{\aa}{\expr_\aa} & = & {\tbor{\lft}{\bormode}{\typ\subst{\aa}{\expr_\aa}}}\\
    {\uninit{n}}\subst{\aa}{\expr_\aa} & = & \uninit{n}\\
    ({\polysig{\overline{\tvar}}
    {{\overline{\aa: \sort}}}
    {{\expr}}
    {\loccx_i}
    {\overline{\typ}}
    {\typ_o}
    {\loccx_o}})\subst{\aa}{\expr_\aa} & = & \left\{\begin{array}{ll}
                \polysig{\overline{\tvar}}
            {{\overline{\aa: \sort}}}
            {{\expr}}
            {\loccx_i}
            {\overline{\typ}}
            {\typ_o}
            {\loccx_o} & \text{if } \aa \in \{\overline{\aa}\}\\

            \polysig{\overline{\tvar}}
            {{\overline{\aa: \sort}}}
            {{\expr\subst{\aa}{\expr_\aa}}}
            {\loccx_i\subst{\aa}{\expr_\aa}}
            {\overline{\typ\subst{\aa}{\expr_\aa}}}
            {\\ \quad\quad\quad\typ_o\subst{\aa}{\expr_\aa}}
            {\loccx_o\subst{\aa}{\expr_\aa}}, & \text{otherwise }
        \end{array}\right.\\[0.5em]

    \text{\textbf{Logical Expressions}} & & \\
    {\bb}\subst{\aa}{\expr_\aa}& = & \left\{\begin{array}{ll}
        \expr_\aa, & \text{if } \aa = \bb\\
        \bb, & \text{otherwise }
        \end{array}\right. \\
    {(\expr_1 [=, \land, +, - , *] \expr_2)}\subst{\aa}{\expr_\aa}& = & \expr_1\subst{\aa}{\expr_\aa} [=, \land, +, - , *] \expr_2\subst{\aa}{\expr_\aa} \\
    {(\lnot \expr)}\subst{\aa}{\expr_\aa}& = & \lnot \expr\subst{\aa}{\expr_\aa} \\
    {n}\subst{\aa}{\expr_\aa}& = & n \quad n \in \mathbb{Z} \\
    {\cloc}\subst{\aa}{\expr_\aa}& = & \cloc \\
    {\ctrue}\subst{\aa}{\expr_\aa}& = & \ctrue \\
    {\cfalse}\subst{\aa}{\expr_\aa}& = & \cfalse \\[0.5em]

    \text{\textbf{Location Contexts}} & & \\
    {\emptyset}\subst{\aa}{\expr_\aa} & = & \emptyset \\
    {(\loccx, \mapstoowned{\loc}{\typ})}\subst{\aa}{\expr_\aa} & = &
    \loccx\subst{\aa}{\expr_\aa}, \mapstoowned{\loc\subst{\aa}{\expr_\aa}}{\typ\subst{\aa}{\expr_\aa}} \\[0.5em]

    \text{\textbf{Value Contexts}} & & \\
    {\emptyset}\subst{\aa}{\expr_\aa} & = & \emptyset \\
    {(\env, \mapstoenv{\xx}{\typ})}\subst{\aa}{\expr_\aa} & = &
    \env\subst{\aa}{\expr_\aa}, \mapstoenv{\xx}{\typ\subst{\aa}{\expr_\aa}} \\[1em]

    \text{\textbf{Dynamic Location Contexts}} & & \\
    {\emptyset}\subst{\aa}{\expr_\aa} & = & \emptyset \\
    {(\dynenv, \mapstoowned{(\cloc,\ptrtag)}{\typ})}\subst{\aa}{\expr_\aa} & = &
    \dynenv\subst{\aa}{\expr_\aa}, \mapstoowned{(\cloc,\ptrtag)}{\typ\subst{\aa}{\expr_\aa}} \\[0.5em]

    \text{\textbf{Refinement Contexts}} & & \\
    {\emptyset}\subst{\aa}{\expr_\aa} & = & \emptyset \\
    {(\varcx, \aa': \sort)}\subst{\aa}{\expr_\aa} & = &
        \varcx\subst{\aa}{\expr_\aa}, \aa': \sort \text{, if } \aa \not= \aa' \\
    {(\varcx, \expr)}\subst{\aa}{\expr_\aa} & = & \varcx\subst{\aa}{\expr_\aa}, \expr\subst{\aa}{\expr_\aa} \\
\end{array}
$$
\clearpage


\subsection{Expression Substitution (values)}
$$
\begin{array}{lcl}
    (\eunpack{\xx}{\aa}{\ee})\subst{\yy}{\val_\yy} & = & \left\{\begin{array}{ll}
        \ee\subst{\yy}{\val_\yy}\subst{\aa}{\interp{\val_\yy}}, & \text{if } \xx = \yy\\
        \eunpack{\xx}{\aa}{\ee}\subst{\yy}{\val_\yy}, & \text{otherwise }
        \end{array}\right.\\
    (\blet{\xx}{\ee_\xx}{\ee})\subst{\yy}{\val_\yy} & = & \left\{\begin{array}{ll}
        \blet{\xx}{\ee_\xx\subst{\yy}{\val_\yy}}{\ee}, & \text{if } \xx = \yy\\
        \blet{\xx}{\ee_\xx\subst{\yy}{\val_\yy}}{\ee\subst{\yy}{\val_\yy}}, & \text{otherwise }
        \end{array}\right.\\
    (\blet{\xx}{\new{\lvar}}{\ee})\subst{\yy}{\val_\yy} & = & \left\{\begin{array}{ll}
        \blet{\xx}{\new{\lvar}}{\ee}, & \text{if } \xx = \yy\\
        \blet{\xx}{\new{\lvar}}{\ee\subst{\yy}{\val_\yy}}, & \text{otherwise }
        \end{array}\right.\\
        \xx\subst{\yy}{\val_\yy} & = & \left\{\begin{array}{ll}
            \val_\yy, & \text{if } \xx = \yy\\
            \xx, & \text{otherwise }
            \end{array}\right.\\
        (\bif{\ee}{\ee_1}{\ee_2})\subst{\yy}{\val_\yy} & = &
    \bif{\ee\subst{\yy}{\val_\yy}}{\ee_1\subst{\yy}{\val_\yy}}{\ee_2\subst{\yy}{\val_\yy}} \\
    (\bseq{\stmt}{\ee})\subst{\yy}{\val_\yy} & = &
    \bseq{\stmt\subst{\yy}{\val_\yy}}{\ee\subst{\yy}{\val_\yy}}\\
    (\fcall{e}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}})\subst{\yy}{\val_\yy} & = &
    \fcall{e\subst{\yy}{\val_\yy}}{\overline{\typ}}{\overline{\expr}}{\overline{\aval\subst{\yy}{\val_\yy}}}\\

    % \text{\textbf{Value Substitution}} & & \\
    (\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}})\subst{\yy}{\val_\yy} & = & \left\{\begin{array}{ll}
        \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\ee\subst{\yy}{\val_\yy}}, & \text{if } \yy \not = \ff \text{ and } \yy \not = \xx_i\\
        \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\ee}, & \text{otherwise }
        \end{array}\right.
    \\
    \val\subst{\yy}{\val_\yy} & = & \val \\

    % \text{\textbf{Statement Substitution}} & & \\

    \sassign{\place}{\rval}\subst{\yy}{\val_\yy} & = &
    \sassign{\place\subst{\yy}{\val_\yy}}{\rval\subst{\yy}{\val_\yy}}
    \\
    % \sskip\subst{\yy}{\val_\yy} & = & \sskip \\

    % \text{\textbf{R-Value Substitution}} & & \\

    % \val\subst{\yy}{\val_\yy} & = & \val\subst{\yy}{\val_\yy}\\
    (\rvstrgref{\place}) \subst{\yy}{\val_\yy} & = & \rvstrgref{\place\subst{\yy}{\val_\yy}} \\

    (\rvmutref{\place}) \subst{\yy}{\val_\yy} & = & \rvmutref{\place\subst{\yy}{\val_\yy}} \\

    (\rvshrref{\place}) \subst{\yy}{\val_\yy} & = & \rvshrref{\place\subst{\yy}{\val_\yy}} \\

    (\deref{\place}) \subst{\yy}{\val_\yy} & = & \deref{\place\subst{\yy}{\val_\yy}} \\
\end{array}
$$

\subsection{Expressions Substitution (refinements)}
$$
\begin{array}{lcl}
    (\eunpack{\xx}{\bb}{\ee})\subst{\aa}{\expr_\aa} & = & \left\{\begin{array}{ll}
        \eunpack{\xx}{\bb}{\ee\subst{\aa}{\val_\aa}}, & \text{if } \aa \neq \bb \\
        \eunpack{\xx}{\bb}{\ee} & \text{otherwise }
        \end{array}\right.\\

    (\blet{\xx}{\ee_\xx}{\ee})\subst{\aa}{\expr_\aa} & = & \blet{\xx}{\ee_\xx\subst{\aa}{\expr_\aa}}{\ee\subst{\aa}{\expr_\aa}} \\

    (\blet{\xx}{\new{\lvar}}{\ee})\subst{\aa}{\expr_\aa} & = & \left\{\begin{array}{ll}
        \blet{\xx}{\new{\lvar}}{\ee\subst{\aa}{\expr_\aa}}, & \text{if } \aa \neq \lvar \\
        \blet{\xx}{\new{\lvar}}{\ee\subst{\aa}{\expr_\aa}}, & \text{otherwise} \\
        \end{array}\right.\\

    \xx\subst{\aa}{\expr_\aa} & = & \xx \\

    (\bif{\ee}{\ee_1}{\ee_2})\subst{\aa}{\expr_\aa} & = &
    \bif{\ee\subst{\aa}{\expr_\aa}}{\ee_1\subst{\aa}{\expr_\aa}}{\ee_2\subst{\aa}{\expr_\aa}} \\

    (\bseq{\stmt}{\ee})\subst{\aa}{\expr_\aa} & = &
    \bseq{\stmt\subst{\aa}{\expr_\aa}}{\ee\subst{\aa}{\expr_\aa}}\\

    (\fcall{e}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}})\subst{\aa}{\expr_\aa} & = &
    \fcall{e\subst{\aa}{\expr_\aa}}{\overline{\typ}}{\overline{\expr\subst{\aa}{\expr_\aa}}}{\overline{\aval\subst{\aa}{\expr_\aa}}} \\

    % \multicolumn{3}{l}{\text{\textbf{Substitution of refinements in values}}}  \\

    (\vrec{\ff}{\overline{\bb}}{\overline{\xx}}{{e}})\subst{\aa}{\expr_\aa} & = & \left\{\begin{array}{ll}
        \vrec{\ff}{\overline{\bb}}{\overline{\xx}}{\ee\subst{\aa}{\expr_\aa}}, & \text{if } \aa \neq \bb_i \\
        \vrec{\ff}{\overline{\bb}}{\overline{\xx}}{\ee}, & \text{otherwise }
        \end{array}\right.
    \\

    \val\subst{\aa}{\expr_\aa} & = & \val \\

    % \multicolumn{3}{l}{\text{\textbf{Substitution of refinements in statements}}}  \\

    \sassign{\place}{\rval}\subst{\aa}{\expr_\aa} & = &
    \sassign{\place\subst{\aa}{\expr_\aa}}{\rval\subst{\aa}{\expr_\aa}} \\

    % \sskip\subst{\aa}{\expr_\aa} & = & \sskip \\

    % \multicolumn{3}{l}{\text{\textbf{Substitution of refinements in r-values}}}  \\

    % \val\subst{\aa}{\expr_\aa} & = & \val\subst{\aa}{\expr_\aa}\\

    (\rvstrgref{\place}) \subst{\aa}{\expr_\aa} & = & \rvstrgref{\place\subst{\aa}{\expr_\aa}} \\

    (\rvmutref{\place}) \subst{\aa}{\expr_\aa} & = & \rvmutref{\place\subst{\aa}{\expr_\aa}} \\

    (\rvshrref{\place}) \subst{\aa}{\expr_\aa} & = & \rvshrref{\place\subst{\aa}{\expr_\aa}} \\

    (\deref{\place}) \subst{\aa}{\expr_\aa} & = & \deref{\place\subst{\aa}{\expr_\aa}} \\
\end{array}
$$
\clearpage

\subsection{Type Sorts and Value Indices}

The following definitions connect values and types with
the refinement logic.
%
The function \getsort{\bty} associates a \emph{refinement sort} to
a base type \bty.
%
Values of type \bty must be indexed with refinements of that sort.
%
The function \interp{\cdot} maps values to a \emph{refinement index}.
%
This function is partial as only values of a base type can be refined.
%
Integers and booleans are mapped to the exact value in the logic.
%
Vectors are mapped to an index representing its length.

$$
\begin{array}{lcl}
    \getsort{\tint} & = & \sint\\
    \getsort{\tbool} & = & \sbool\\
    \getsort{\tvec} & = & \sint \\
    \interp{\ctrue}         & = & \ctrue \\
    \interp{\cfalse}        & = & \cfalse\\
    \interp{n}              & = & n, \text{ for } n \in \mathbb{Z} \\
    \interp{\vvec{n}{\val}} & = & n, \text{ for } n \in \mathbb{Z} \\
\end{array}
$$
\clearpage


==> metatheory/formalism.tex <==
\section{Syntax of \corelan.}
\label{subsec:formalism:syntax}
\input{syntax}
\input{definitions}

\section{Declarative Judgements of \corelan.}
\label{subsec:formalism:typing}
\input{wellformed}
\input{typing}
\input{models}
%\begin{comment}

\section{Stacked Borrows}
\label{subsec:formalism:stacked-borrows}
\input{stacked-borrows}

\section{Operational Semantics of \corelan.}
\label{subsec:formalism:operational}
\input{operational}
\input{runtime-typing.tex}

\clearpage
\section{Soundness of \corelan.}
\label{subsec:formalism:soundness}

\subsection{Main theorems}

Our soundness claim states that
evaluation of a well typed expression will
1) return a value of the same type,
2) return a memory violation error (\memerr), or
3) diverge.

\input{theorems/soundness}
\input{theorems/progress}
\input{theorems/preservation}


\clearpage
\subsection{Proof of soudness}
\input{proofs/soundness}

\subsection{Proof of preservation}
\input{proofs/preservation}
% \input{proofs/stmt-preservation}
% \input{proofs/rvalue-preservation}

\subsection{Proof of progress}
\input{proofs/progress}

\subsection{Lemmata}
\input{lemmata}
\input{type-substitution}
\input{canonical}

\subsection{Lemmata about memory events}
\input{memory-events-lemmata}

% \clearpage
% \section{Vectors}
% \subsection{Syntax}
% \input{vectors/syntax}
% \subsection{Declarative judgments}
% \input{vectors/typing}
% \input{vectors}




==> metatheory/lemmata.tex <==
\begin{lemma}[Subtyping Transitive]\label{lemma:subtype:trans}
  If \wf{\typ_1}, then
  if \subtyping{\typ_1}{\typ_2} and \subtyping{\typ_2}{\typ_3},
  then \subtyping{\typ_1}{\typ_3}.
\end{lemma}
\begin{proof}
By induction on the structure of the three types.
We split cases on $\typ_1$
\begin{itemize}
  \item $\typ_1 \equiv \rtyp{\tcon}{\expr_1}$.
  Then, the left rule can be either \subrtyp or \subexists.
  \begin{itemize}
  \item \textbf{Left rule is \subrtyp.}
    Then $\typ_2 \equiv \rtyp{\tcon}{\expr_2}$ and we know
    (1) $\subtyping
    {\rtyp{\tcon}{\expr_1}}
    {\rtyp{\tcon}{\expr_2}}$.
   The right rule can be either \subrtyp or \subexists.
    \begin{itemize}
      \item \textbf{Right rule is \subrtyp.}
      Then $\typ_3 \equiv \rtyp{\tcon}{\expr_3}$ and we know
      (2) $\subtyping
      {\rtyp{\tcon}{\expr_2}}
      {\rtyp{\tcon}{\expr_3}}$.
      By inversion of (1) and (2) we get:
      (3) \entailment{\varcx}{\expr_1 = \expr_2} and
      (4) \entailment{\varcx}{\expr_2 = \expr_3}.
      By (3), (4), and assumption~\ref{assumption:model:transitive}, we have
      (5) \entailment{\varcx}{\expr_1 = \expr_3}.
      By rule~\subrtyp we conclude the proof.
      \item \textbf{Right rule is \subexists.}
      Then $\typ_3 \equiv \texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_3}$ and we know
      (2) \subtyping
      {\rtyp{\tcon}{\expr_2}}
      {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_3}}.
      By inversion of (1) and (2) we get
      (3) \entailment{\varcx}{\expr_1 = \expr_2} and
      (4) \entailment{\varcx}{\expr_3[\expr_2/\aa]}.
      By (3), (4), and assumption~\ref{assumption:model:congruence}, we get
      (5) \entailment{\varcx}{\expr_3[\expr_1/\aa]},
      which concludes the proof by rule~\subexists.
    \end{itemize}
  \item \textbf{Left rule is \subexists.}
  Then $\typ_2 \equiv \texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_2}$ and we know
  (1) $\subtyping
  {\rtyp{\tcon}{\expr_1}}
  {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_2}}$.
 The right rule can only be \subunpack:
 (2) \subtyping
 {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_2}}
 {\typ_3}.
 By inversion of (2):
 (3) \subtyping[\varcx, \aa: \getsort{\tcon}, \expr_2]
                {\rtyp{\tcon}{\aa}}
                {\typ_3}.
 Thus, $\typ_3$ can be either singleton or existential
 and, respectively, the applied rules are
 can be either \subrtyp or \subexists.
    \begin{itemize}
      \item \textbf{Right inverted rule is \subrtyp.}
      Then $\typ_3 \equiv \rtyp{\tcon}{\expr_3}$ and we know
      $$(4) \subtyping[\varcx, \aa: \getsort{\tcon}, \expr_2]
                {\rtyp{\tcon}{\aa}}
                {\rtyp{\tcon}{\expr_3}}$$
      Since by assumption, \wf{\typ_1}, \sortck[\varcx]{\expr_1}{\getsort{\tcon}}
      by which and lemma~\ref{lemma:type-substitution}, from (4) we get:
      $$(5) \subtyping[\varcx, \expr_2\subst{\aa}{\expr_1}]
                {\rtyp{\tcon}{\expr_1}}
                {\rtyp{\tcon}{\expr_3}}$$
      By inversion of (1) we know that \entailment{\varcx}{\expr_2[\expr_1/\aa]},
      by which and lemma~\ref{lemma:condition} we get
      $$(6) \subtyping[\varcx]
                {\rtyp{\tcon}{\expr_1}}
                {\rtyp{\tcon}{\expr_3}}$$
      Which concludes the proof.
      \item \textbf{Right inverted rule is \subexists.}
      Then $\typ_3 \equiv \texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_3}$ and we know
      $$(4) \subtyping[\varcx, \aa: \getsort{\tcon}, \expr_2]
                {\rtyp{\tcon}{\aa}}
                \texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_3}$$
      By inversion:
      $$ (5) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_2}{\expr_3}$$
      Since by assumption, \wf{\typ_1}, \sortck[\varcx]{\expr_1}{\getsort{\tcon}}
      by which and assumption~\ref{assumption:model:substitution}, we get:
      $$ (6) \entailment{\varcx, \expr_2[\expr_1/\aa]}{\expr_3[\expr_1/\aa]}$$
      By inversion of (1) we know that \entailment{\varcx}{\expr_2[\expr_1/\aa]},
      by which and assumption~\ref{assumption:model:cut} we get
      $$ (7) \entailment{\varcx}{\expr_3[\expr_1/\aa]}$$
      Which concludes the proof by rule \subexists.
    \end{itemize}
\end{itemize}

  \item $\typ_1 \equiv \texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_1}$.
  The left rule is \subunpack:
  (1) \subtyping
  {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_1}}
  {\typ_2}.
  By inversion:
  (2) \subtyping
  [\varcx, \aa: \getsort{\tcon}, \expr_1]
  {\rtyp{\tcon}{\aa}}
  {\typ_2}. So, the inverted right rule can be either \subrtyp or \subexists:
  \begin{itemize}
    \item \textbf{Left inverted rule is \subrtyp.}
    Then, $\typ_2 \equiv \rtyp{\tcon}{\expr_2}$ and we know:
    (3): \subtyping
    [\varcx, \aa: \getsort{\tcon}, \expr_1]
    {\rtyp{\tcon}{\aa}}
    {\rtyp{\tcon}{\expr_2}}.
    By inversion:
    (4): \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1}{\aa = \expr_2}.
    Since \subtyping{\rtyp{\tcon}{\expr_2}}{\typ_3}, the right rule can be
    either \subrtyp or \subexists:
    \begin{itemize}
      \item \textbf{Right rule is \subrtyp.}
      Then, $\typ_3 \equiv \rtyp{\tcon}{\expr_3}$ and we know:
      (5): \subtyping
      [\varcx]
      {\rtyp{\tcon}{\expr_2}}
      {\rtyp{\tcon}{\expr_3}}.
      By inversion: (6) \entailment{\varcx}{\expr_2 = \expr_3}.
      By assumption~\ref{assumption:model:equality} and (6), (4) becomes:
      (7) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1}{\aa = \expr_3}.
      By (7) and rule \subrtyp:
      \subtyping[\varcx, \aa: \getsort{\tcon}, \expr_1]
                {\rtyp{\tcon}{\aa}}
                {\rtyp{\tcon}{\expr_3}},
                which concludes the proof by rule \subunpack.
      \item \textbf{Right rule is \subexists.}
      Then $\typ_3 \equiv \texists{\aa_3}{\rtyp{\tcon}{\aa_3}}{\expr_3}$ and we know
      (5) \subtyping
                {\rtyp{\tcon}{\expr_2}}
                {\texists{\aa_3}{\rtyp{\tcon}{\aa_3}}{\expr_3}}.
      By inversion:
      (6) \entailment{\varcx}{\expr_3[\expr_2/\aa_3]}.
      By assumption~\ref{assumption:model:weakening} on (6):
      (7) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1}{\expr_3[\expr_2/\aa_3]}.
      By (4) and assumption~\ref{assumption:model:equality}
      (8) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1}{\expr_3[\aa/\aa_3]}.
      By rule \subexists
      \subtyping[\varcx, \aa: \getsort{\tcon}, \expr_1]{\rtyp{\tcon}{\aa}}{\texists{\aa_3}{\rtyp{\tcon}{\aa_3}}{\expr_3}}.
      The proof concludes by rule \subunpack.
    \end{itemize}
    \item \textbf{Left inverted rule is \subexists.}
    Then $\typ_2 \equiv \texists{\aa_2}{\rtyp{\tcon}{\aa_2}}{\expr_2}$ and we know
    (3) \subtyping
    [\varcx, \aa: \getsort{\tcon}, \expr_1]
    {\rtyp{\tcon}{\aa}}
    {\texists{\aa_2}{\rtyp{\tcon}{\aa_2}}{\expr_2}}.
    By inversion,
    (4) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1}{\expr_2[\aa/\aa_2]}.
    The right rule is \subunpack and by inversion we get:
    (5) \subtyping
    [\varcx, \aa_2: \getsort{\tcon}, \expr_2]
    {\rtyp{\tcon}{\aa_2}}
    {\typ_3}. Thus the right inverted rule can be either \subrtyp or \subexists.
    \begin{itemize}
      \item\textbf{Right inverted rule is \subrtyp.}
      Then $\typ_3 \equiv \rtyp{\tcon}{\expr_3}$ and we know
      \subtyping[\varcx, \aa_2: \getsort{\tcon}, \expr_2]{\rtyp{\tcon}{\aa_2}}{\rtyp{\tcon}{\expr_3}}.
      By inversion:
      (6) \entailment{\varcx, \aa_2: \getsort{\tcon}, \expr_2}{\aa_2 = \expr_3}.
      By (6) and assumption~\ref{assumption:model:weakening}:
      (7) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1, \aa_2: \getsort{\tcon}, \expr_2}{\aa_2 = \expr_3}.
      By assumption~\ref{assumption:model:substitution}:
      (8) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1, \expr_2[\aa/\aa_2]}{\aa = \expr_3}.
      By (4) and assumption~\ref{assumption:model:cut}:
      (9) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1}{\aa = \expr_3}.
      By rule ~\subrtyp:
      (10) \subtyping[\varcx, \aa: \getsort{\tcon}, \expr_1]
                {\rtyp{\tcon}{\aa}}
                {\rtyp{\tcon}{\expr_3}}.
      Then, rule~\subunpack concludes the proof.
      \item\textbf{Right inverted rule is \subexists.}
      Then $\typ_3 \equiv \texists{\aa_3}{\rtyp{\tcon}{\aa_3}}{\expr_3}$
      and we know \subtyping
      [\varcx, \aa_2: \getsort{\tcon}, \expr_2]
      {\rtyp{\tcon}{\aa_2}}
      {\texists{\aa_3}{\rtyp{\tcon}{\aa_3}}{\expr_3}}.
      By inversion:
      (6) \entailment{\varcx, \aa_2: \getsort{\tcon}, \expr_2}{\expr_3[\aa_2/\aa_3]}.
      By (6) and assumption~\ref{assumption:model:weakening}:
      (7) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1, \aa_2: \getsort{\tcon}, \expr_2}{\expr_3[\aa_2/\aa_3]}.
      By assumption~\ref{assumption:model:substitution}:
      (8) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1, \expr_2[\aa/\aa_2]}{\expr_3[\aa_2/\aa_3][\aa/\aa_2]}.
      By (4) and assumption~\ref{assumption:model:cut}:
      (9) \entailment{\varcx, \aa: \getsort{\tcon}, \expr_1}{\expr_3[\aa/\aa_3]}.
     The proof concludes by rules~\subexists and \subunpack.
    \end{itemize}
  \end{itemize}
  \item $\typ_1 \equiv \tptr{\loc}$.
  The left rule is \subptr and $\typ_2 \equiv \tptr{\loc}$.
  Similarly, the right rule is \subptr and $\typ_3 \equiv \tptr{\loc}$.
  The proof concludes by rule \subptr.
  \item $\typ_1 \equiv \uninit{n}$.
  As before, $\typ_2 \equiv \typ_3 \equiv \uninit{n}$
  and the proof concludes by rule \submem.
  \item $\typ_1 \equiv \tbor{\lft}{\shr}{\typ'_1}$.
  The left rule is \subborshr and $\typ_2 \equiv \tbor{\lft}{\shr}{\typ'_2}$.
  By inversion, (1) \subtyping{\typ'_1}{\typ'_2}.
  The right rule is \subborshr and $\typ_3 \equiv \tbor{\lft}{\shr}{\typ'_3}$.
  By inversion, (2) \subtyping{\typ'_2}{\typ'_3}.
  By inductive hypothesis on (1) and (2):  \subtyping{\typ'_1}{\typ'_3},
  which concludes the proof by rule \subborshr.

  \item $\typ_1 \equiv \tbor{\lft}{\mut}{\typ'_1}$.
  The left rule is \subbormut and $\typ_2 \equiv \tbor{\lft}{\mut}{\typ'_2}$.
  By inversion, (1) \subtyping{\typ'_1}{\typ'_2} and (2) \subtyping{\typ'_2}{\typ'_1}.
  The right rule is \subbormut and $\typ_3 \equiv \tbor{\lft}{\mut}{\typ'_3}$.
  By inversion, (3) \subtyping{\typ'_2}{\typ'_3} and (4) \subtyping{\typ'_3}{\typ'_2}.
  By inductive hypothesis on (1) and (3): (5) \subtyping{\typ'_1}{\typ'_3}.
  By inductive hypothesis on (4) and (2): (6) \subtyping{\typ'_3}{\typ'_1}.
  The proof concludes by (5), (6), and rule \subbormut.

  \item $\typ_1 \equiv \polysig{\overline{\tvar}}
  {\overline{\aa: \sort}}
  {\expr_1}
  {\loccx_{1i}}
  {\overline{\typ_1}}
  {\typ_{1o}}
  {\loccx_{1o}}$.
  Then,
  $\typ_2 \equiv \polysig{\overline{\tvar}}
  {\overline{\aa: \sort}}
  {\expr_2}
  {\loccx_{2i}}
  {\overline{\typ_2}}
  {\typ_{2o}}
  {\loccx_{2o}}$
  and $ \typ_3 \equiv
  \polysig{\overline{\tvar}}
            {\overline{\aa: \sort}}
            {\expr_3}
            {\loccx_{3i}}
            {\overline{\typ_3}}
            {\typ_{3o}}
            {\loccx_{3o}}$.
By inversion of the two rules:
(1) \entailment{\varcx, \overline{\aa: \sort}}{\expr_2 \Rightarrow \expr_1},
(2) \loccxinc
    {\varcx, \overline{\aa: \sort}}
    {\elftcx}{\llftcx}
    {\loccx_{2i}}
    {\loccx_{1i}},
(3) $\forall i. \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{2i}}{\typ_{1i}}$
(4) \loccxinc
{\varcx, \overline{\aa: \sort}}
{\elftcx}{\llftcx}
{\loccx_{1o}}
{\loccx_{2o}},
(5) \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{1o}}{\typ_{2o}},
(6) \entailment{\varcx, \overline{\aa: \sort}}{\expr_3 \Rightarrow \expr_2},
(7) \loccxinc
    {\varcx, \overline{\aa: \sort}}
    {\elftcx}{\llftcx}
    {\loccx_{3i}}
    {\loccx_{2i}},
(8) $\forall i. \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{3i}}{\typ_{2i}}$
(9) \loccxinc
{\varcx, \overline{\aa: \sort}}
{\elftcx}{\llftcx}
{\loccx_{2o}}
{\loccx_{3o}}, and
(10) \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{2o}}{\typ_{3o}}.

By (1), (5), and assumption~\ref{assumption:model:transitive:implication}:
(11) \entailment{\varcx, \overline{\aa: \sort}}{\expr_3 \Rightarrow \expr_1}.
By (2), (6), and rule \loccxinctrans:
(12) \loccxinc
    {\varcx, \overline{\aa: \sort}}
    {\elftcx}{\llftcx}
    {\loccx_{3i}}
    {\loccx_{1i}}.
By (3), (8), and inductive hypothesis:
(13) $\forall i. \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{3i}}{\typ_{1i}}$.
By (4), (9), and rule \loccxinctrans:
(14) \loccxinc
{\varcx, \overline{\aa: \sort}}
{\elftcx}{\llftcx}
{\loccx_{1o}}
{\loccx_{3o}}.
By (5), (10), and inductive hypothesis:
(15) \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{1o}}{\typ_{3o}}.
The proof concludes by (11)-(15) and rule \subfun.
\end{itemize}
\end{proof}



\begin{lemma}[Weakening]\label{lemma:weakening}
  If \typing{\varcx}
       {\env}
       {\loccx_i}
       {\dynenv}
       {\ee}
       {\typ}
       {\loccx_o}
       {}, \wf{\dynenv'}, and $\dynenv' \supseteq \dynenv$ then
\typing{\varcx}
       {\env}
       {\loccx_i}
       {\dynenv'}
       {\ee}
       {\typ}
       {\loccx_o}
       {}
\end{lemma}
\begin{proof}
 By induction on the expression typing derivation trees.
 \dynenv is only used in the rules \tcall to ensure well-formedness, which is established by assumption,
 and \ttptr, where the theorem holds because $\dynenv' \supseteq \dynenv$.
\end{proof}

\begin{lemma}[Context Inclusion]\label{lemma:conctext-inclusion}
If \loccxinc{\varcx}{}{}{\loccx_2}{\loccx_1} and \typing{\varcx}{\env}{\loccx_1}{\dynenv}{\ee}{\typ}{\loccx_{1o}}{\dynenv},
then \typing{\varcx}{\env}{\loccx_2}{\dynenv}{\ee}{\typ}{\loccx_{2o}}{\dynenv}
and \loccxinc{\varcx}{}{}{\loccx_{2o}}{\loccx_{1o}}.
\end{lemma}
\begin{proof}
  By induction on the derivation trees.
  \newline
  %%% EXPRESSIONS
    \begin{itemize}
        \item \textbf{Rule \tsub:}
        \typing{\varcx}{\env}{\loccx_1}{\dynenv}{\ee}
                {\typ}
                {\loccx_{1o}}
                {\dynenv}.
        By inversion:
        (1) \typing{\varcx}{\env}{\loccx_1}{\dynenv}{\ee}
        {\typ_1}
        {\loccx}
        {\dynenv},
        (2) \subtyping{\typ_1}{\typ}, and
        (3) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx}{\loccx_{1o}}.
        By inductive hypothesis on (1):
        (4) \typing{\varcx}{\env}{\loccx_2}{\dynenv}{\ee}
        {\typ_1}
        {\loccx_{2o}}
        {\dynenv} and
        (5) \loccxinc{\varcx}{}{}{\loccx_{2o}}{\loccx}.
        By (2), (4), and rule \tsub,
        \typing{\varcx}{\env}{\loccx_2}{\dynenv}{\ee}
        {\typ}
        {\loccx_{2o}}
        {\dynenv}.
        By (3), (5), and rule~\loccxinctrans,
        (5) \loccxinc{\varcx}{}{}{\loccx_{2o}}{\loccx_{1o}}.

        \item \textbf{Rule \tlet:}
        \typing{\varcx}{\env}{\loccx_{1i}}{\dynenv}{\blet{\xx}{\ee_{\xx}}{\ee}}{\typ}{\loccx_{1o}}{\dynenv_o}.
        By inversion:
        (1) \typing{\varcx}{\env}{\loccx_{1i}}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv},
        (2) \typing{\varcx}{\env,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee}{\typ}{\loccx_{1o}}{\dynenv_o}, and
        (3) $\xx \not \in \dom{\env}$.
        By inductive hypothesis on (1):
        (4) \typing{\varcx}{\env}{\loccx_{2i}}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx'_2}{\dynenv}
        and (5) \loccxinc{\varcx}{}{}{\loccx'_2}{\loccx}.
        By inductive hypothesis on (2), with (5):
        (6) \typing{\varcx}{\env,\mapstoenv{\xx}{\typ_\xx}}{\loccx'_2}{\dynenv}{\ee}{\typ}{\loccx_{2o}}{\dynenv_o}, and
         (5) \loccxinc{\varcx}{}{}{\loccx_{2o}}{\loccx_{1o}}.
         The proof concludes by (5) and rule \tlet on (4), (6), and (3).


        \item \textbf{Rule \tnew:}
        \typing{\varcx}
            {\env}{\loccx_{1i}}{\dynenv}{\blet{\xx}{\new{\lvar}}{e}}{\typ}{\loccx_{1o}}{\dynenv}.
        By inversion:
        (1) \typing{\varcx, \lvar:\sloc}
        {\env, \mapstoenv{\xx}{\tptr{\lvar}}}
        {\loccx_{1i}, \mapstoowned{\lvar}{\uninit{1}}}
        {\dynenv}{\ee}{\typ}{\loccx_{1o}}{\dynenv},
        (2) \wf{\typ},
        (3) \wf{\loccx_{1o}},
        (4) $\xx \notin \dom{\env}$,
        (5) $\lvar \notin \dom{\varcx}$.
        By lemma~\ref{lemma:contextinclusion:endend} and inductive hypothesis on (1):
        (6) \typing{\varcx, \lvar:\sloc}
        {\env, \mapstoenv{\xx}{\tptr{\lvar}}}
        {\loccx_{2i}, \mapstoowned{\lvar}{\uninit{1}}}
        {\dynenv}{\ee}{\typ}{\loccx_{2o}}{\dynenv} and
        (7) \loccxinc{\varcx}{}{}{\loccx_{2o}}{\loccx_{1o}}.
        The proof concludes by (7) and rule \tnew on
        (6), (3), (4), (5), and lemma~\ref{lemma:wf}.

        \item \textbf{Rule \tif:}
        The proofs go by induction and transitive of context inclusion (as in the \tlet case).

        \item \textbf{Rule \tunpack:}
        The proof goes by induction and lemma~\ref{lemma:wf}.

        \item \textbf{Rule \tcall:}
        \typing{\varcx}{\env}{\loccx}{\dynenv}
               {\fcall{\ee}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
               {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}}, \loccx_2}{}.
        By inversion:
        (1) $\forall i. \typing{\varcx}{\env}{\loccx}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx}{}$,
        (2) \typing{\varcx}{\env}{\loccx}{\dynenv}{e}
               {\polysig{\overline{\tvar}}
                        {\overline{\aa: \sort}}
                        {\expr}
                        {\loccx_{i}}
                        {\overline{\typ}}
                        {\typ_o}
                        {\loccx_{o}}}
              {\loccx_1, \loccx_2 }{\dynenv},
        (3) $ \substvar = \subst{\overline{\aa}}{\overline{\expr}}$,
        (4) \loccxinc{\varcx}{}{}{\loccx_1}{\applysubst{\substvar}{\loccx_{i}}},
        (5) $\forall i.\sortck{\expr_i}{\sort_i}$,
        (6) \lmodel{\varcx}{\applysubst{\substvar}{\expr}}, and
        (7) \wf{\dynenv}.
       Assume $\loccx'$, so that,
       (8) \loccxinc{\varcx}{}{}{\loccx'}{\loccx}.
       By inductive hypothesis on (1) ans (2):
       (9) $\forall i. \typing{\varcx}{\env}{\loccx'}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx'}{}$,
       (10) \typing{\varcx}{\env}{\loccx'}{\dynenv}{e}
              {\polysig{\overline{\tvar}}
                       {\overline{\aa: \sort}}
                       {\expr}
                       {\loccx_{i}}
                       {\overline{\typ}}
                       {\typ_o}
                       {\loccx_{o}}}
             {\loccx'_{12} }{\dynenv},
        (11) \loccxinc{\varcx}{}{}{\loccx'_{12}}{\loccx_1, \loccx_2}.
        Because of (11), $\dom{\loccx_1, \loccx_2}\subseteq \dom{\loccx'_{12}}$.
        We split $\loccx'_{12}$ to $\loccx'_{12} \equiv \loccx'_1, \loccx'_2$,
        so that $\dom{\loccx_2} = \dom{\loccx'_2}$.
        Then,
        (12) \loccxinc{\varcx}{}{}{\loccx'_1}{\loccx_1} and
        (13) \loccxinc{\varcx}{}{}{\loccx'_2}{\loccx_2}.
        By (9), (10), (3), (5), (6), (7), and rule \loccxinctrans on (4) and (12),
        from rule \tcall we get:
        \typing{\varcx}{\env}{\loccx'}{\dynenv}
        {\fcall{\ee}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
        {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}}, \loccx'_2}{}.
        The proof concludes by \loccxincframe and (13).




        \item \textbf{Rule \ttvar, \ttrue, \tfalse, \tconstint, \tfun, \ttptr, and \tumem:}
        In these cases the context is not used and not changed, thus
        $\loccx_{2o} = \loccx_2$,
        $\loccx_{1o} = \loccx_1$, and by assumption:   \loccxinc{\varcx}{}{}{\loccx_{2o}}{\loccx_{1o}}.

        \item \textbf{Rule \tassign:}
        By inversion, inductive hypothesis and application of the rule.

        \item \textbf{Rule \tassignstrg:}
        By inversion, inductive hypothesis, application of the rule and lemma~\ref{lemma:contextinclusion:endend}.

        \item \textbf{Rule \tstrgmutrebor:}
        \rvaltyping{\varcx}{\env}{\loccx_1}{\dynenv}{\rvmutref{\place}}{\tref{\mut}{\typ}}{\loccx_1[\loc\mapsto \typ]}.
        By inversion:
        (1) \pltyping{\varcx}{\env}{\loccx_1}{\dynenv}{\place}{\tptr{\loc}}{\loccx_1} and
        (2) \subtyping{\loccx_1(\loc)}{\typ}.
        By case splitting on the two typing rules for (1):% \nv{note it is complicated that it has to return the same context....}
        (3) \pltyping{\varcx}{\env}{\loccx_2}{\dynenv}{\place}{\tptr{\loc}}{\loccx_2}.
        By assumption, (2), and lemma~\ref{lemma:inclusion:sub}:
        (5) \subtyping{\loccx_2(\loc)}{\typ}.
        By (3), (5), and rule \tstrgmutrebor:
        \rvaltyping{\varcx}{\env}{\loccx_2}{\dynenv}{\rvmutref{\place}}{\tref{\mut}{\typ}}{\loccx_2[\loc\mapsto \typ]}.
        By rules \loccxinctrans, \loccxincperm, and \loccxincframe,
        \loccxinc{\varcx}{}{}{\loccx_2[\loc\mapsto \typ]}{\loccx_1[\loc\mapsto \typ]}, which concludes the proof.

        \item \textbf{Rule \tstrgrebor, \tmutmutrebor, \tshrrebor, \tderef and \tderefstrg:}
        By inductive hypothesis and the fact that in these cases the context is not used and not changed, thus
        $\loccx_{2o} = \loccx_2$,
        $\loccx_{1o} = \loccx_1$, and by assumption:   \loccxinc{\varcx}{}{}{\loccx_{2o}}{\loccx_{1o}}.
  \end{itemize}

\end{proof}


\begin{lemma}[Context Inclusion Extend]\label{lemma:contextinclusion:endend}
  If \loccxinc{\varcx}{}{}{\loccx_2}{\loccx_1},
  then
  \loccxinc{\varcx}{}{}{\loccx_2[\loc\mapsto \typ]}{\loccx_1[\loc\mapsto \typ]}
  and
  \loccxinc{\varcx}{}{}{\loccx_2,\loc\mapsto \typ}{\loccx_1,\loc\mapsto \typ}.
\end{lemma}
\begin{proof}
  By rules \loccxincperm, \loccxincframe, and \loccxinctrans.
\end{proof}


\begin{lemma}[Framing]\label{lemma:framing}
  If {\wf{\loccx_{o1}, \loccx, \loccx_{o2}}}
  and \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\ee}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv},
then \typing{\varcx}{\env}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}{\ee}{\typ}{\loccx_{o1}, \loccx, \loccx_{o2}}{\dynenv}.
\end{lemma}
\begin{proof}
  By induction on the derivation tree.
  \newline
  %%% EXPRESSIONS
    \begin{itemize}
        \item \textbf{Rule \tsub:}
        \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\ee}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv}.
        By inversion:
        (1) \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\ee}
                {\typ_1}
                {\loccx_1, \loccx_2}
                {\dynenv},
        (2) \subtyping{\typ_1}{\typ}, and
        (3) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_1, \loccx_2}{\loccx_{o1}, \loccx_{o2}}.
        By inductive hypothesis on (1):
        (4) \typing{\varcx}{\env}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}{\ee}
                {\typ_1}
                {\loccx_1, \loccx, \loccx_2}
                {\dynenv}.
        By lemma~\ref{lemma:framing:context} on (3):
        (5) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_1, \loccx, \loccx_2}{\loccx_{o1}, \loccx, \loccx_{o2}}.
        The proof concludes by (4), (2), (5), and rule \tsub.

        \item \textbf{Rule \tlet:}
        \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\blet{\xx}{\ee_{\xx}}{\ee}}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv_o}.
        By inversion:
        (1) \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx_1, \loccx_2}{\dynenv},
        (2) \typing{\varcx}{\env,\mapstoenv{\xx}{\typ_\xx}}{\loccx_1, \loccx_2}{\dynenv}{\ee}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv_o}, and
        (3) $\xx \not \in \dom{\env}$.
        By inductive hypothesis on (1) and (2):
        (4) \typing{\varcx}{\env}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx_1, \loccx, \loccx_2}{\dynenv} and
        (5) \typing{\varcx}{\env,\mapstoenv{\xx}{\typ_\xx}}{\loccx_1, \loccx, \loccx_2}{\dynenv}{\ee}{\typ}{\loccx_{o1}, \loccx, \loccx_{o2}}{\dynenv_o}.
        The proof concludes by (3)-(5) and rule \tlet.

        \item \textbf{Rule \tnew:}
        \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\blet{\xx}{\new{\lvar}}{e}}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv}.
        By inversion:
        (1) \typing{\varcx, \lvar:\sloc}
            {\env, \mapstoenv{\xx}{\tptr{\lvar}}}
            {\loccx_{i1}, \loccx_{i2}, \mapstoowned{\lvar}{\uninit{1}}}
            {\dynenv}{\ee}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv},
        (2) \wf{\typ},
        (3) \wf{\loccx_{o1}, \loccx_{o2}},
        (4) $\xx \notin \dom{\env}$, and
        (5) $\lvar \notin \dom{\varcx}$.
        By inductive hypothesis on (1):
        (6) \typing{\varcx, \lvar:\sloc}
        {\env, \mapstoenv{\xx}{\tptr{\lvar}}}
        {\loccx_{i1}, \loccx, \loccx_{i2}, \mapstoowned{\lvar}{\uninit{1}}}
        {\dynenv}{\ee}{\typ}{\loccx_{o1}, \loccx, \loccx_{o2}}{\dynenv}.
        By assumption: (7) \wf{\loccx_{o1}, \loccx, \loccx_{o2}}.
        The proof concludes by (6), (2), (7), (4), (5), and rule \tnew.
        \item \textbf{Rule \tif:}
        \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv_i}{\bif{\ee}{\ee_1}{\ee_2}}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv}.
        By inversion:
        (1) \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\ee}{\rtyp{\tbool}{\expr}}{\loccx_1, \loccx_2}{\dynenv_o},
        (2) \typing{\varcx, \expr}{\env}{\loccx_1, \loccx_2}{\dynenv}{\ee_1}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv}, and
        (3) \typing{\varcx, \lnot \expr}{\env}{\loccx_1, \loccx_2}{\dynenv}{\ee_2}{\typ}{\loccx_{o1}, \loccx_{o2}}{\dynenv}.
        The proof concludes by inductive hypothesis on (1)-(3) and the rule \tif.

        % \item \textbf{Rule \tseq:}
        % By inversion, case~\ref{lemma:framing:stmt} and inductive hypothesis, and application of the rule.

        \item \textbf{Rule \tunpack:}
        By inversion, inductive hypothesis and the well formedness assumption, and application of the rule.

        \item \textbf{Rule \tcall:}
        \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}
               {\fcall{\ee}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
               {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}}, \loccx_2}{}
        By inversion:
        \begin{enumerate}
        \item $\forall i. \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx_{i1}, \loccx_{i2}}{}$,
        \item \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{e}
               {\polysig{\overline{\tvar}}
                        {\overline{\aa: \sort}}
                        {\expr}
                        {\loccx_{i}}
                        {\overline{\typ}}
                        {\typ_o}
                        {\loccx_{o}}}
              {\loccx_1, \loccx_2 }{\dynenv},
        \item $\substvar = \subst{\overline{\aa}}{\overline{\expr}}$,
        \item \loccxinc{\varcx}{}{}{\loccx_1}{\applysubst{\substvar}{\loccx_{i}}},
        \item $\forall i.\sortck{\expr_i}{\sort_i}$,
        \item \lmodel{\varcx}{\applysubst{\substvar}{\expr}}, and
        \item \wf{\dynenv}.
        \end{enumerate}
%        (8) $\dom{\loccx_{o}} \cap \dom{\loccx_2} = \emptyset$.
        %
        By inductive hypothesis on (1) and (2):
        \begin{enumerate}
          \setcounter{enumi}{7}
          \item $\forall i. \typing{\varcx}{\env}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx_{i1}, \loccx, \loccx_{i2}}{}$,
          \item \typing{\varcx}{\env}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}{e}
                    {\polysig{\overline{\tvar}}
                              {\overline{\aa: \sort}}
                              {\expr}
                              {\loccx_{i}}
                              {\overline{\typ}}
                              {\typ_o}
                              {\loccx_{o}}}
                    {\loccx_1, \loccx, \loccx_2 }{\dynenv}.
        \end{enumerate}
        By (3)-(9) and rule \tcall, we get the following:
        $$
        \typing{\varcx}{\env}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}
               {\fcall{\ee}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
               {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}}, (\loccx, \loccx_2)}{}.
        $$

        \item \textbf{Rule \tfun:} By inversion of the rule:
        $$
        \typing{\varcx,\overline{\aa: \sort},\expr}
               {\env,
                \overline{\xx : \typ},
                \ff: \polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                             {{\expr}}{\loccx_{i}}
                             {\overline{\typ}}
                             {{\typ}}
                             {\loccx_{o}}
                }
               {\loccx_{i}}{\dynenv}
               {\ee}
               {\typ}{\loccx_o}
               {}
        $$

        \item \textbf{Rule \ttvar, \ttrue, \tfalse, \tconstint, \tfun, \ttptr, and \tumem:}
        These cases are trivial because typing preserves the location context.
        So, if
        \typing{\varcx}{\env}{\loccx_{i1}, \loccx_{i2}}{\dynenv}{\ee}{\typ}{\loccx_{i1}, \loccx_{i2}}{\dynenv},
        then \typing{\varcx}{\env}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}{\ee}{\typ}{\loccx_{i1}, \loccx, \loccx_{i2}}{\dynenv}.

        \item \textbf{Rule \tassign:} by inversion, inductive hypothesis
        and application of the rule.

        \item \textbf{Rule \tassignstrg:} by inversion, inductive hypothesis
        and application of the rule.

      \item \textbf{Rule \tstrgrebor:} by inversion, inductive hypothesis, and application of the rule.

      \item \textbf{Rule \tstrgmutrebor:}
      \rvaltyping{\varcx}{\env}{\loccx_{1}, \loccx_{2}}{\dynenv}{\rvmutref{\place}}{\tref{\mut}{\typ}}{(\loccx_{1} , \loccx_{2})[\loc\mapsto \typ]}.
      By inversion:
      (1) \pltyping{\varcx}{\env}{\loccx_{1} , \loccx_{2}}{\dynenv}{\place}{\tptr{\loc}}{\loccx_{1} , \loccx_{2}} and
      (2) \subtyping{(\loccx_{1} , \loccx_{2})(\loc)}{\typ}.
      By inductive hypothesis on (1):
      (3) \pltyping{\varcx}{\env}{\loccx_{1} , \loccx , \loccx_{2}}{\dynenv}{\place}{\tptr{\loc}}{\loccx_{1}, \loccx , \loccx_{2}}.
      By the disjointness assumption  $(\loccx_{1} , \loccx_{2})(\loc) = (\loccx_{1}  , \loccx , \loccx_{2})(\loc)$, thus (2) becomes:
      (4) \subtyping{(\loccx_{1} , \loccx , \loccx_{2})(\loc)}{\typ}.
      The proof concludes by (2), (4), and rule \tstrgmutrebor.
      \item \textbf{Rule \tmutmutrebor, \tshrrebor, \tderef and \tderefstrg:} by inversion, inductive hypothesis, and application of the rule.
      % \item \textbf{Rule \tshrrebor:} by inversion, case~\ref{lemma:framing:expr}, and application of the rule.
      % \item \textbf{Rule \tderef:} by inversion, case~\ref{lemma:framing:expr}, and application of the rule.
      % \item \textbf{Rule \tderefstrg:} by inversion, case~\ref{lemma:framing:expr}, and application of the rule.
      % \item \textbf{Rule \trvalval:} by inversion, case~\ref{lemma:framing:expr}, and application of the rule.
  \end{itemize}
\end{proof}

\begin{lemma}[Context Inclusion Subtyping]\label{lemma:inclusion:sub}
  If \loccxinc{\varcx}{}{}{\loccx_2}{\loccx_1} and \subtyping{\loccx_1(\loc)}{\typ},
  then \subtyping{\loccx_2(\loc)}{\typ}.
\end{lemma}
\begin{proof}
By induction on the context inclusion tree and by splitting cases in the
\loccxincframe rule.
\end{proof}


\begin{lemma}[Inclusion Framing]\label{lemma:framing:context}
  If \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_{i1}, \loccx_{i2}}{\loccx_{o1}, \loccx_{o2}},
  then \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_{i1}, \loccx, \loccx_{i2}}{\loccx_{o1}, \loccx, \loccx_{o2}}.
\end{lemma}
\begin{proof}
    By assumption:
    $$(1) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_{i1}, \loccx_{i2}}{\loccx_{o1}, \loccx_{o2}}.$$
    By rule \loccxincframe:
    $$(2) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx, \loccx_{i1}, \loccx_{i2}}{\loccx, \loccx_{o1}, \loccx_{o2}}.$$
    By rule \loccxincperm:
    $$(3) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_{i1}, \loccx, \loccx_{i2}}{\loccx, \loccx_{i1}, \loccx_{i2}}
    \text{ and }
    (4) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx, \loccx_{o1}, \loccx_{o2}}{\loccx_{o1}, \loccx, \loccx_{o2}}.$$
    By (3), (2), and \loccxinctrans:
    $$(5) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_{i1}, \loccx, \loccx_{i2}}{\loccx, \loccx_{o1}, \loccx_{o2}}.$$
    By (5), (4), and \loccxinctrans:
    $$(6) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx_{i1}, \loccx, \loccx_{i2}}{\loccx_{o1}, \loccx, \loccx_{o2}}.$$
    Which concludes the proof.
\end{proof}


\begin{lemma}[AVal Typing]\label{lemma:aval}
If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\aval}{\typ}{\loccx_o}{\dynenv},
then for any $\loccx$, so that \wf{\loccx},
\typing{\varcx}{\env}{\loccx}{\dynenv}{\aval}{\typ}{\loccx}{\dynenv}.
\end{lemma}
\begin{proof}
By exhaustion: the typing rules for \aval
and the type weakening part of rule \tsub, do not depent on \loccx.
\end{proof}

% \begin{lemma}[Well-formedness]\label{lemma:typing-implies-wf}
%   If \typing{\varcx{}}
%        {\env}
%        {\loccx_i}
%        {\dynenv}
%        {\ee}
%        {\typ}
%        {\loccx_o}
%        {}
% then \wf{\env}, \wf{\loccx_i}, \wf{\dynenv}, \wf{\typ} and \wf{\loccx_o}.
% \end{lemma}
% \begin{proof}
%   \todo{This does not hold, check the leaves. But we do not seem to need it.}
% \end{proof}

\begin{lemma}[Well-formed Variables]\label{lemma:wf-fv}
  Well-formedness ensures free variables are included in $\varcx$:
  \begin{itemize}
  \item If \wf{\typ} then $\fv{\typ}\subseteq \dom{\varcx}$.
  \item If \wf{\env} then $\fv{\env}\subseteq \dom{\varcx}$.
  \item If \wf{\loccx} then $\fv{\loccx}\subseteq \dom{\varcx}$.
  \item If \wf{\dynenv} then $\fv{\dynenv}\subseteq \dom{\varcx}$.
\end{itemize}
\end{lemma}
\begin{proof}
By structural induction on the type and the environments.
\end{proof}

\begin{lemma}[Id Substitution]\label{lemma:fv-subst}
When a variable is not free, substitution is identity:
  \begin{itemize}
    \item If $\aa \notin \fv{\typ}$, then $\typ[\expr/\aa]=\typ$.
    \item If $\aa \notin \fv{\env}$, then $\env[\expr/\aa]=\env$.
    \item If $\aa \notin \fv{\loccx}$, then $\loccx[\expr/\aa]=\loccx$.
    \item If $\aa \notin \fv{\dynenv}$, then $\dynenv[\expr/\aa]=\dynenv$.
  \end{itemize}
\end{lemma}
\begin{proof}
  By structural induction on the type and the environments.
\end{proof}

\begin{lemma}[Id Var Substitution]\label{lemma:subst:idvar}
$\typ[\aa/\aa]=\typ$
\end{lemma}
\begin{proof}
  By structural induction on the type.
\end{proof}


\begin{lemma}[Condition]\label{lemma:condition}
  If \lmodel{\varcx_1}{\expr}, then:
  \begin{enumerate}[label=\roman*]
  \item\label{lemma:condition:typing} If \typing{\varcx_1, \expr, \varcx_2}
           {\env}
           {\loccx_i}
           {\dynenv}
           {\ee}
           {\typ}
           {\loccx_o}
           {},
  then
  \typing{\varcx_1, \varcx_2}
           {\env}
           {\loccx_i}
           {\dynenv}
           {\ee}
           {\typ}
           {\loccx_o}
           {}.
  \item\label{lemma:condition:subtyping}
  If \subtyping[\varcx_1, \expr, \varcx_2]{\typ_1}{\typ_2},
  then \subtyping[\varcx_1, \varcx_2]{\typ_1}{\typ_2}.
  \item\label{lemma:condition:context}
  If \loccxinc{\varcx_1, \expr, \varcx_2}{\elftcx}{\llftcx}
           {\loccx_i}
           {\loccx_o},
  then
  \loccxinc{\varcx_1, \varcx_2}{\elftcx}{\llftcx}
           {\loccx_i}
           {\loccx_o}.
  \end{enumerate}
  \end{lemma}
  \begin{proof}
  By mutual induction on the derivation trees.
  \newline
  \textbf{Case \ref{lemma:condition:typing})}
  We split cases on the type derivation.
  \begin{itemize}
    \item \textbf{Rule \tsub:}
    \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee}
    {\typ}
    {\loccx_o}
    {\dynenv}.
    By inversion:
  (1) \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee}
    {\typ_1}
    {\loccx}
    {\dynenv},
  (2) \subtyping[\varcx_1, \expr, \varcx_2]{\typ_1}{\typ}, and
  (3) \loccxinc{\varcx_1, \expr, \varcx_2}{\elftcx}{\llftcx}{\loccx}{\loccx_o}.
  By inductive hypothesis on (1) we get
  (4) \typing{\varcx_1, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee}
    {\typ_1}
    {\loccx}
    {\dynenv}.
  By (2) and case~\ref{lemma:condition:subtyping}, we get
  (5) \subtyping[\varcx_1, \varcx_2]{\typ_1}{\typ}.
  By (3) and case~\ref{lemma:condition:context}, we get
  (6) \loccxinc{\varcx_1, \varcx_2}{\elftcx}{\llftcx}{\loccx}{\loccx_o}.
  By (4), (5), (6), and rule \tsub, we conclude the proof.
    \item \textbf{Rule \tlet:}
    $\typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\blet{\xx}{\ee_{\xx}}{\ee}}{\typ}{\loccx_o}{\dynenv_o}$.
    By inversion:
    (1) \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv} and
    (2) \typing{\varcx_1, \expr, \varcx_2}{\env,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv_o}.
    By inductive hypothesis:
    (3) \typing{\varcx_1, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv} and
    (4) \typing{\varcx_1, \varcx_2}{\env,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv_o}.
    By (3), (4), and rule \tlet, we conclude the proof.
    \item \textbf{Rule \tnew:}
    \typing{\varcx_1, \expr, \varcx_2}
              {\env}{\loccx_i}{\dynenv}{\blet{\xx}{\new{\lvar}}{e}}{\typ}{\loccx_o}{\dynenv}.
    By inversion:
    (1) \typing{\varcx_1, \expr, \varcx_2, \lvar:\sloc}
    {\env, \mapstoenv{\xx}{\tptr{\lvar}}}
    {\loccx_i, \mapstoowned{\lvar}{\uninit{1}}}
    {\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv},
    (2) \wf[\varcx_1, \expr, \varcx_2]{\typ}, and
    (3) \wf[\varcx_1, \expr, \varcx_2]{\loccx_o}.
    By inductive hypothesis on (1), and lemma~\ref{lemma:condition:weaken} on (2) and (3):
    (4) \typing{\varcx_1, \varcx_2, \lvar:\sloc}
    {\env, \mapstoenv{\xx}{\tptr{\lvar}}}
    {\loccx_i, \mapstoowned{\lvar}{\uninit{1}}}
    {\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv},
    (5) \wf[\varcx_1, \varcx_2]{\typ}, and
    (6) \wf[\varcx_1, \varcx_2]{\loccx_o}.
    By (4), (5), (6), and rule \tnew, we conclude the proof.
    \item \textbf{Rule \tif:}
    (1) $\typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv_i}{\bif{\ee}{\ee_1}{\ee_2}}{\typ}{\loccx}{\dynenv}$.
    By inversion:
    (2) \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee}{\rtyp{\tbool}{\expr_\ee}}{\loccx_o}{\dynenv_o},
    (3) \typing{\varcx_1, \expr, \varcx_2, \expr_\ee}{\env}{\loccx_o}{\dynenv}{\ee_1}{\typ}{\loccx}{\dynenv}, and
    (4) \typing{\varcx_1, \expr, \varcx_2, \lnot \expr_\ee}{\env}{\loccx_o}{\dynenv}{\ee_2}{\typ}{\loccx}{\dynenv}.
    By inductive hypothesis:
    (5) \typing{\varcx_1, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee}{\rtyp{\tbool}{\expr_\ee}}{\loccx_o}{\dynenv_o},
    (6) \typing{\varcx_1, \varcx_2, \expr_\ee}{\env}{\loccx_o}{\dynenv}{\ee_1}{\typ}{\loccx}{\dynenv}, and
    (7) \typing{\varcx_1, \varcx_2, \lnot \expr_\ee}{\env}{\loccx_o}{\dynenv}{\ee_2}{\typ}{\loccx}{\dynenv}.
    By (5), (6), (7), and rule \tif we conclude the proof.
    % \item \textbf{Rule \tseq:}
    % (1) \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\bseq{\stmt}{\rexpr}}{\typ}{\loccx_o}{\dynenv_o}.
    % By inversion:
    % (2) \stmtyping{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\stmt}{\loccx_{\stmt}}{\dynenv_{\stmt}} and
    % (3) \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_{\stmt}}{\dynenv}{\rexpr}{\typ}{\loccx_o}{\dynenv_o}.
    % By case~\ref{lemma:condition:statements} on (2) and inductive hypothesis on (3):
    % (4) \stmtyping{\varcx_1, \varcx_2}{\env}{\loccx_i}{\dynenv}{\stmt}{\loccx_{\stmt}}{\dynenv_{\stmt}} and
    % (5) \typing{\varcx_1, \varcx_2}{\env}{\loccx_{\stmt}}{\dynenv}{\rexpr}{\typ}{\loccx_o}{\dynenv_o}.
    % By (4), (5), and rule \tseq we conclude the proof.
    \item \textbf{Rule \tunpack:}
    (1) \typing{\varcx_1, \expr, \varcx_2}{\env_1,\mapstoenv{\xx}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}, \env_2}
                 {\loccx_i}{\dynenv}
                 {\eunpack{\xx}{\aa}{e}}{\typ}
                 {\loccx_o}{\dynenv}.
    By inversion:
    (2) \typing{\varcx_1, \expr, \varcx_2, \aa : \getsort{\tcon}, \expr}{\env_1,\mapstoenv{\xx}{\rtyp{\tcon}{\aa}}, \env_2}
                 {\loccx_i}{\dynenv}
                 {\ee}{\typ}
                 {\loccx_o}{\dynenv}.
    By inductive hypothesis:
    (2) \typing{\varcx_1, \varcx_2, \aa : \getsort{\tcon}, \expr}{\env_1,\mapstoenv{\xx}{\rtyp{\tcon}{\aa}}, \env_2}
                 {\loccx_i}{\dynenv}
                 {\ee}{\typ}
                 {\loccx_o}{\dynenv}.
    Which concludes the proof by rule \tunpack.
    \item \textbf{Rule \tcall:}
    (1)         \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx}{\dynenv}
    {\fcall{e}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
    {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}}, \loccx_2}{}.
    By inversion, for $\substvar = \subst{\overline{\aa}}{\overline{\expr}}$:
    (2) $ \forall i. \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx}{}$,
    (3) $\typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx}{\dynenv}{e}
           {\polysig{\overline{\tvar}}
                    {\overline{\aa: \sort}}
                    {\expr}
                    {\loccx_{i}}
                    {\overline{\typ}}
                    {\typ_o}
                    {\loccx_{o}}}
          {\loccx_1, \loccx_2 }{\dynenv}$,
    (4) \loccxinc{\varcx_1, \expr, \varcx_2}{}{}{\loccx_1}{\applysubst{\substvar}{\loccx_{i}}},
    (5) $ \forall i.\sortck[\varcx_1, \expr, \varcx_2]{\expr_i}{\sort_i}$,
    (6) \lmodel{\varcx_1, \expr, \varcx_2}{\applysubst{\substvar}{\expr}}, and
    (7) \wf[\varcx_1, \expr, \varcx_2]{\dynenv}.
    By inductive hypothesis on (2) and (3),
    case~\ref{lemma:condition:context} on (4),
    assumption~\ref{assumption:model:cut} on (6), and
    lemma~\ref{lemma:condition:weaken} on (5) and (7):
    (8) $ \forall i. \typing{\varcx_1,  \varcx_2}{\env}{\loccx}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx}{}$,
    (9) $\typing{\varcx_1,  \varcx_2}{\env}{\loccx}{\dynenv}{e}
           {\polysig{\overline{\tvar}}
                    {\overline{\aa: \sort}}
                    {\expr}
                    {\loccx_{i}}
                    {\overline{\typ}}
                    {\typ_o}
                    {\loccx_{o}}}
          {\loccx_1, \loccx_2 }{\dynenv}$,
    (10) \loccxinc{\varcx_1,  \varcx_2}{}{}{\loccx_1}{\applysubst{\substvar}{\loccx_{i}}},
    (11) $ \forall i.\sortck[\varcx_1,  \varcx_2]{\expr_i}{\sort_i}$,
    (12) \lmodel{\varcx_1,  \varcx_2}{\applysubst{\substvar}{\expr}}, and
    (13) \wf[\varcx_1,  \varcx_2]{\dynenv}.
    BY (8)-(13) and rule \tcall we conclude the proof.
    \item \textbf{Rule \tfun:}
    (1) \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx}{\dynenv}
                 {\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}}
                 {\polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                            {\expr}{\loccx_{i}}{\overline{\typ}}
                            {\typ}{\loccx_{o}}
                 }
                 {\loccx}{\dynenv}.
    By inversion:
    (2) \typing{\varcx_1, \expr, \varcx_2,\overline{\aa: \sort},\expr}
                 {\env,
                  \overline{\xx : \typ},
                  \ff: \polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                               {{\expr}}{\loccx_{i}}
                               {\overline{\typ}}
                               {{\typ}}
                               {\loccx_{o}}
                  }
                 {\loccx_i}{\dynenv}
                 {\ee}
                 {\typ}{\loccx_o}
                 {}.
    By inductive hypothesis:
    (3) \typing{\varcx_1, \varcx_2,\overline{\aa: \sort},\expr}
                 {\env,
                  \overline{\xx : \typ},
                  \ff: \polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                               {{\expr}}{\loccx_{i}}
                               {\overline{\typ}}
                               {{\typ}}
                               {\loccx_{o}}
                  }
                 {\loccx_i}{\dynenv}
                 {\ee}
                 {\typ}{\loccx_o}
                 {}.
     (3) and rule \tfun concludes the proof.
    \item \textbf{Rules \ttvar, \ttrue, \tfalse, \tconstint, \ttptr, and \tumem:}
    are trivial since they do not depend on the logical environment.

    % \item \textbf{Rule \tskip:}
    % \stmtyping{\varcx_1, \expr, \varcx_2}{\env}{\loccx}{\dynenv}{\sskip}{\loccx}{\dynenv}.
    % By rule \tskip,
    % \stmtyping{\varcx_1, \varcx_2}{\env}{\loccx}{\dynenv}{\sskip}{\loccx}{\dynenv},
    % which concludes the proof.

    \item \textbf{Rule \tassign:}
    (1) \typing{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\sassign{\place}{\ee}}{\uninit{1}}{\loccx_o}{}.
    By inversion:
    (2) \rvaltyping{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee'}{\typ_v}{\loccx_i},
    (3) \pltyping{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\place}{\tref{\mut}{\typ}}{\loccx_i}, and
    (4) \subtyping[\varcx_1, \expr, \varcx_2]{\typ_v}{\typ}.
    By inductive hypothesis on (2) and case~\ref{lemma:condition:subtyping} on (4):
    (5) \rvaltyping{\varcx_1, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee'}{\typ_v}{\loccx_i},
    (6) \subtyping[\varcx_1, \varcx_2]{\typ_v}{\typ}.
    By (5), (3), (6), and rule \tassign, we conclude the proof.

    \item \textbf{Rule \tassignstrg:}
    (1) \stmtyping{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\sassign{\place}{\ee'}}{\loccx_o[\loc \mapsto \typ]}{}.
    By inversion:
    (2) \rvaltyping{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee'}{\typ}{\loccx_o} and
    (3) \pltyping{\varcx_1, \expr, \varcx_2}{\env}{\loccx_i}{\place}{\tptr{\loc}}{\loccx_i}.
    By inductive hypothesis on (2):
    (4) \rvaltyping{\varcx_1, \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee'}{\typ}{\loccx_o}.
    By (4), (3), and rule \tassignstrg we conclude the proof.

    \item \textbf{Rule \tstrgmutrebor and \tshrrebor:}
    By inversion, application of case~\ref{lemma:condition:subtyping},
    and application of the respective rule.

    \item \textbf{Rule \tstrgrebor, \tmutmutrebor, \tderef, and \tderefstrg:}
    These cases are trivial since they do not depend on the logical environment.
  \end{itemize}


  \textbf{Case \ref{lemma:condition:subtyping})} We split cases on the subtyping derivation:
  \begin{itemize}
    \item \textbf{Rule \tstrgrebor:}
    \subtyping[\varcx_1, \expr, \varcx_2, \aa: \getsort{\tcon}, \expr_\aa]
    {\rtyp{\tcon}{\aa}}
    By inductive hypothesis:
    (3) \subtyping
    [\varcx_1, \varcx_2, \aa: \getsort{\tcon}, \expr_\aa]
    {\rtyp{\tcon}{\aa}}
    {\typ}.
    (3) and rule \subunpack conclude the proof.
    \item \textbf{Rule \subexists:}
    (1) \subtyping[\varcx_1, \expr, \varcx_2]
                  {\rtyp{\tcon}{\expr_1}}
                  {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_2}}.
    By inversion:
    (2) \entailment{\varcx_1, \expr, \varcx_2}{\expr_2[\expr_1/\aa]}.
    By hypothesis, (2), and assumption~\ref{assumption:model:cut}:
    (3) \entailment{\varcx_1, \varcx_2}{\expr_2[\expr_1/\aa]}.
    (3) and rule \subexists conclude the proof.
    \item \textbf{Rule \subborshr:}
    \subtyping[\varcx_1, \expr, \varcx_2]
    {\tbor{\lft}{\shr}{\typ_1}}
    {\tbor{\lft}{\shr}{\typ_2}}.
    By inversion:
    \subtyping[\varcx_1, \expr, \varcx_2]{\typ_1}{\typ_2}.
    By inductive hypothesis:
    \subtyping[\varcx_1, \varcx_2]{\typ_1}{\typ_2},
    which, by rule \subborshr concludes the proof.
    \item \textbf{Rule \subbormut:}
    \subtyping[\varcx_1, \expr, \varcx_2]
    {\tbor{\lft}{\mut}{\typ_1}}
    {\tbor{\lft}{\mut}{\typ_2}}.
    By inversion:
    \subtyping[\varcx_1, \expr, \varcx_2]{\typ_1}{\typ_2} and
    \subtyping[\varcx_1, \expr, \varcx_2]{\typ_2}{\typ_1}.
    By inductive hypothesis:
    \subtyping[\varcx_1, \varcx_2]{\typ_1}{\typ_2} and
    \subtyping[\varcx_1, \varcx_2]{\typ_2}{\typ_1},
    which, by rule \subbormut concludes the proof.
  \end{itemize}

  \textbf{Case \ref{lemma:condition:context})}
  We split cases on the context derivation:
  \begin{itemize}
    \item \textbf{Rule \loccxincperm:}
    \loccxinc
    {\varcx_1, \expr, \varcx_2}
    {\elftcx}{\llftcx}
    {\loccx}
    {\loccx'}.
    By inversion $\loccx'$  is a permutation of  $\loccx$.
    By rule \loccxincperm,
    \loccxinc
    {\varcx_1, \varcx_2}
    {\elftcx}{\llftcx}
    {\loccx}
    {\loccx'}, which concludes the proof.
    \item \textbf{Rule \loccxincweaken:}
    \loccxinc{\varcx_1, \expr, \varcx_2}
                  {\elftcx}{\llftcx}
                  {\loccx,\loccx'}
                  {\loccx}.
    By rule \loccxincweaken:
    \loccxinc{\varcx_1, \varcx_2}
    {\elftcx}{\llftcx}
    {\loccx,\loccx'}
    {\loccx}, which concludes the proof.
    \item \textbf{Rule \loccxincframe:}
    \loccxinc
    {\varcx_1, \expr, \varcx_2}
    {\elftcx}{\llftcx}
    {\loccx,\loccx_1}
    {\loccx, \loccx_2}.
    By inversion:
    \loccxinc{\varcx_1, \expr, \varcx_2}
             {\elftcx}{\llftcx}
             {\loccx_1}{\loccx_2}.
    By inductive hypothesis:
    \loccxinc{\varcx_1, \varcx_2}
             {\elftcx}{\llftcx}
             {\loccx_1}{\loccx_2}.
    By which and rule \loccxincframe we conclude the proof.
    \item \textbf{Rule \loccxincsub:}
    \loccxinc{\varcx_1, \expr, \varcx_2}
                  {\elftcx}{\llftcx}
                  {\mapstoowned{\loc}{\typ_1}}
                  {\mapstoowned{\loc}{\typ_2}}.
    By inversion: \subtyping[\varcx_1, \expr, \varcx_2]{\typ_1}{\typ_2}.
    By case~\ref{lemma:condition:subtyping},
    By inversion: \subtyping[\varcx_1, \varcx_2]{\typ_1}{\typ_2}.
    Which concludes the proof by rule \loccxincsub.
  \end{itemize}
  \end{proof}

  \begin{lemma}[Condition Weakening]\label{lemma:condition:weaken}.
    \begin{enumerate}
    \item\label{lemma:condition:wftyp}
    If \wf[\varcx_1, \expr, \varcx_2]{\typ}, then \wf[\varcx_1, \varcx_2]{\typ}.
    \item\label{lemma:condition:context:wft}
    If \wf[\varcx_1, \expr, \varcx_2]{\loccx}, then \wf[\varcx_1, \varcx_2]{\loccx}.
    \item\label{lemma:condition:context:sort}
    If \sortck[\varcx_1, \expr, \varcx_2]{\expr}{\sort}, \sortck[\varcx_1, \varcx_2]{\expr}{\sort}.
    \end{enumerate}
  \end{lemma}
  \begin{proof}
  By mutual induction on the derivation trees.
  Note that all three derivations depend on the bindings and not
  the expressions of the logical environment.
  \end{proof}


\begin{lemma}[Substitution]\label{lemma:program-substitution}\label{lemma:program-substitution-2}
  If  \typing{\varcx}{\env_1}{\loccx_i}{\dynenv}{\val}{\typ_x}{\loccx_i}{}, then
  If \typing{\varcx}
         {\env_1,\mapstoenv{\xx}{\typ_x},\env_2}
         {\loccx_i}
         {\dynenv}
         {\ee}
         {\typ}
         {\loccx_o}
         {},
  then
  \typing{\varcx}
         {\env_1,\env_2}
         {\loccx_i}
         {\dynenv}
         {\ee[\val/\xx]}
         {\typ}
         {\loccx_o}
         {}.
  \end{lemma}
  \begin{proof}
    By induction on the derivation tree.
\begin{itemize}
\item \textbf{Rule \tsub:}
(1) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\ee[\val/\xx]}
{\typ}
{\loccx_o}
{\dynenv}.
By inversion:
(2) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\ee[\val/\xx]}
                {\typ_1}
                {\loccx}
                {\dynenv},
(3) \subtyping{\typ_1}{\typ}, and
(4) \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx}{\loccx_o}.
By inductive hypothesis on (2):
(5) \typing{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\ee[\val/\xx]}
                {\typ_1}
                {\loccx}
                {\dynenv}.
By (5), (3), (4), and rule \tsub, we conclude the proof.
\item \textbf{Rule \tlet:}
(1) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\blet{\xx}{\ee_{\xx}}{\ee}}{\typ}{\loccx_o}{\dynenv_o}.
By inversion we get
(2) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv},
(3) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv_o}, and
(4) $\xx \not \in \dom{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}$.
By inductive hypothesis on (2) and (3) we get:
(5) \typing{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\ee_{\xx}[\val/\xx]}{\typ_{\xx}}{\loccx}{\dynenv} and
(6) \typing{\varcx}{\env_1,\env_2,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee[\val/\xx]}{\typ}{\loccx_o}{\dynenv_o}.
By (7), we get  $\xx \not \in \dom{\env_1,\env_2}$.
By (5)-(7) and rule \tlet we conclude the proof.

\item \textbf{Rule \tnew:}
(1) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\blet{\yy}{\new{\lvar}}{e}}{\typ}{\loccx_o}{\dynenv}.
By inversion:
(2) \typing{\varcx, \lvar:\sloc}
            {\env_1,\mapstoenv{\xx}{\typ_x},\env_2, \mapstoenv{\yy}{\tptr{\lvar}}}
            {\loccx_i, \mapstoowned{\lvar}{\uninit{1}}}
            {\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv},
     (3) \wf{\typ},
     (4) \wf{\loccx_o}, and
     (5) $\yy \not \in \dom{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}$.
By inductive hypothesis on (2):
(6) \typing{\varcx, \lvar:\sloc}
            {\env_1,\env_2, \mapstoenv{\yy}{\tptr{\lvar}}}
            {\loccx_i, \mapstoowned{\lvar}{\uninit{1}}}
            {\dynenv}{\ee[\val/\xx]}{\typ}{\loccx_o}{\dynenv}.
By (5) we get (7): $\yy \not \in \dom{\env_1,\env_2}$.
By (6), (3), (4), (7), and rule \tnew we conclude the proof.

\item \textbf{Rule \tif:}
(1) {\typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv_i}{\bif{\ee}{\ee_1}{\ee_2}}{\typ}{\loccx}{\dynenv}}.
By inversion:
(2) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\ee}{\rtyp{\tbool}{\expr}}{\loccx_o}{\dynenv_o},
(3) \typing{\varcx, \expr}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_o}{\dynenv}{\ee_1}{\typ}{\loccx}{\dynenv}, and
(4) \typing{\varcx, \lnot \expr}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_o}{\dynenv}{\ee_2}{\typ}{\loccx}{\dynenv}.
By inductive hypothesis on (2) - (4):
(5) \typing{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\ee[\val/\xx]}{\rtyp{\tbool}{\expr}}{\loccx_o}{\dynenv_o},
(6) \typing{\varcx, \expr}{\env_1,\env_2}{\loccx_o}{\dynenv}{\ee_1[\val/\xx]}{\typ}{\loccx}{\dynenv}, and
(7) \typing{\varcx, \lnot \expr}{\env_1,\env_2}{\loccx_o}{\dynenv}{\ee_2[\val/\xx]}{\typ}{\loccx}{\dynenv}.
The proof concludes by (5)-(7) and rule \tif.

% \item \textbf{Rule \tseq:}
% (1) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\bseq{\stmt}{\rexpr}}{\typ}{\loccx_o}{\dynenv_o}.
% By inversion:
% (2) \stmtyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_i}{\dynenv}{\stmt}{\loccx_{\stmt}}{\dynenv_{\stmt}} and
% (3) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx_{\stmt}}{\dynenv}{\rexpr}{\typ}{\loccx_o}{\dynenv_o}.
% By case~\ref{lemma:program:substitution:stmt} on (2) and inductive hypothesis on (3):
% (4) \stmtyping{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\stmt[\val/\xx]}{\loccx_{\stmt}}{\dynenv_{\stmt}} and
% (5) \typing{\varcx}{\env_1,\env_2}{\loccx_{\stmt}}{\dynenv}{\rexpr[\val/\xx]}{\typ}{\loccx_o}{\dynenv_o}.
% The proof concludes by rule \tseq.
\item \textbf{Rule \tunpack:}
Let the environment of the typing rule be
$\env_{u1},\mapstoenv{\xx_u}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}, \env_{u2}$.
We split three cases depending on where the substituted variable \xx is:
\begin{itemize}
  \item $\xx \in \env_{u1}:$
  (1) $\typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2,\mapstoenv{\xx_u}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}, \env_{u2}}
  {\loccx_i}{\dynenv}
  {\eunpack{\xx_u}{\aa}{e}}{\typ}
  {\loccx_o}{\dynenv}$.
  By inversion, (2)
  \typing{\varcx, \aa : \getsort{\tcon}, \expr}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2,\mapstoenv{\xx_u}{\rtyp{\tcon}{\aa}}, \env_{u2}}
  {\loccx_i}{\dynenv}
  {\ee}{\typ}
  {\loccx_o}{\dynenv}.
  By inductive hypothesis
  (3)
  \typing{\varcx, \aa : \getsort{\tcon}, \expr}{\env_1,\env_2,\mapstoenv{\xx_u}{\rtyp{\tcon}{\aa}}, \env_{u2}}
  {\loccx_i}{\dynenv}
  {\ee[\val/\xx]}{\typ}
  {\loccx_o}{\dynenv}.
  The proof concludes by rule \tunpack, since  $(\eunpack{\xx_u}{\aa}{e})[\val/\xx] = \eunpack{\xx_u}{\aa}{e[\val/\xx]}$.
  \item $\xx  = \xx_u:$
  (1) $\typing{\varcx}{\env_1,\mapstoenv{\xx}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}, \env_{2}}
  {\loccx_i}{\dynenv}
  {\eunpack{\xx_}{\aa}{e}}{\typ}
  {\loccx_o}{\dynenv}$.
  By inversion:
  (2)
  \typing{\varcx, \aa : \getsort{\tcon}, \expr}{\env_1,\mapstoenv{\xx}{\rtyp{\tcon}{\aa}}, \env_2}
               {\loccx_i}{\dynenv}
               {\ee}{\typ}
               {\loccx_o}{\dynenv}.
  By inductive hypothesis:
  $$(3)\
  \typing{\varcx, \aa : \getsort{\tcon}, \expr}{\env_1, \env_2}
               {\loccx_i}{\dynenv}
               {\ee[\val/\xx]}{\typ}
               {\loccx_o}{\dynenv}.$$
%
By hypothesis: $\typing{\varcx}{\env_1}{\loccx_i}{\dynenv}{\val}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}{\loccx_i}{}$
and lemma~\ref{lemma:value-refinement}:
$$(4)\
\sortck[\varcx]{\interp{\val}}{\getsort{\tcon}}\ \text{and}\
(5)\
\lmodel{\varcx}{\expr[\interp{\val}/\aa]}.$$
By (3), (4), and lemma~\ref{lemma:type-substitution}:
$$(6)\
\typing{\varcx, \expr[\interp{\val}/\aa]}{\env_1[\interp{\val}/\aa], \env_2[\interp{\val}/\aa]}
             {\loccx_i[\interp{\val}/\aa]}{\dynenv[\interp{\val}/\aa]}
             {\ee[\val/\xx][\interp{\val}/\aa]}{\typ[\interp{\val}/\aa]}
             {\loccx_o[\interp{\val}/\aa]}{\dynenv[\interp{\val}/\aa]}.$$
By (6), (5), and lemma~\ref{lemma:condition}:
$$(7)\
\typing{\varcx}{\env_1[\interp{\val}/\aa], \env_2[\interp{\val}/\aa]}
             {\loccx_i[\interp{\val}/\aa]}{\dynenv[\interp{\val}/\aa]}
             {\ee[\val/\xx][\interp{\val}/\aa]}{\typ[\interp{\val}/\aa]}
             {\loccx_o[\interp{\val}/\aa]}{\dynenv[\interp{\val}/\aa]}.$$
By the well-formedness premise and lemmata~\ref{lemma:fv-subst} and~\ref{lemma:wf-fv}:
$$(8)\
\typing{\varcx}{\env_1, \env_2}
             {\loccx_i}{\dynenv}
             {\ee[\val/\xx][\interp{\val}/\aa]}{\typ}
             {\loccx_o}{\dynenv}$$
Which concludes the proof, since
$(\eunpack{\xx}{\aa}{e})[\val/\xx] = \ee[\val/\xx]\subst{\aa}{\interp{\val}}$.
  \item $\xx \in \env_{u2}:$ Similar to first case.
\end{itemize}


\item \textbf{Rule \tcall:}
(1) \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx}{\dynenv}
               {\fcall{\ee}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
               {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}}, \loccx_2}{}.
By inversion, for $\substvar = \subst{\overline{\aa}}{\overline{\expr}}$:
(2) $ \forall i. \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx}{}$,
(3) $ \typing{\varcx}{\env_1,\mapstoenv{\xx}{\typ_x},\env_2}{\loccx}{\dynenv}{e}
       {\polysig{\overline{\tvar}}
                {\overline{\aa: \sort}}
                {\expr}
                {\loccx_{i}}
                {\overline{\typ}}
                {\typ_o}
                {\loccx_{o}}}
      {\loccx_1, \loccx_2 }{\dynenv}$,
(4) $\loccxinc{\varcx}{}{}{\loccx_1}{\applysubst{\substvar}{\loccx_{i}}}$,
(5) $ \forall i.\sortck{\expr_i}{\sort_i}$,
(6) \lmodel{\varcx}{\applysubst{\substvar}{\expr}}, and
(7) \wf{\dynenv}.
The proof concludes by inductive hypothesis on (2) and (3) and application of the \tcall rule.

\item \textbf{Rule \ttvar:}
(1) \typing{\varcx}{\env_1,\mapstoenv{\yy}{\typ_\yy},\env_2}{\loccx}{\dynenv}{\xx}{\selfty{\typ}{\xx}}{\loccx}{\dynenv}.
By inversion: (2) $\mapstoenv{\xx}{\typ} \in \env_1,\mapstoenv{\yy}{\typ_\yy},\env_2$.
We split cases on wheather $\xx = \yy$:
\begin{itemize}
  \item \textbf{$\xx \not = \yy$:}
  $\xx[\val/\yy] = \xx$ and by (2)
  $\mapstoenv{\xx}{\typ} \in \env_1,\env_2$. So, rule \ttvar concludes the proof.
  \item \textbf{$\xx = \yy$}
  $\xx[\val/\yy] = \val$ and by (2)
  $\typ = \typ_\yy$. So, the assumption, strengthened by lemma~\ref{lemma:strengthen} with $\env_2$,
  concludes the proof.
\end{itemize}

\item \textbf{Rule \tfun:}
(1) \typing{\varcx}{\env_1,\mapstoenv{\yy}{\typ_\yy},\env_2}{\loccx}{\dynenv}
               {\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}}
               {\polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                          {\expr}{\loccx_{i}}{\overline{\typ}}
                          {\typ}{\loccx_{o}}
               }
               {\loccx}{\dynenv}.
By inversion,
(2) \typing{\varcx,\overline{\aa: \sort},\expr}
{\env_1,\mapstoenv{\yy}{\typ_\yy},\env_2,
 \overline{\xx : \typ},
 \ff: \polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
              {{\expr}}{\loccx_{i}}
              {\overline{\typ}}
              {{\typ}}
              {\loccx_{o}}
 }
{\loccx_i}{\dynenv}
{\ee}
{\typ}{\loccx_o}
{}.
By inductive hypothesis,
(3) \typing{\varcx,\overline{\aa: \sort},\expr}
{\env_1,\env_2,
 \overline{\xx : \typ},
 \ff: \polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
              {{\expr}}{\loccx_{i}}
              {\overline{\typ}}
              {{\typ}}
              {\loccx_{o}}
 }
{\loccx_i}{\dynenv}
{\ee[\val/\yy]}
{\typ}{\loccx_o}
{}.
By rule \tfun:
(4) \typing{\varcx}{\env_1,\env_2}{\loccx}{\dynenv}
               {\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e[\val/\yy]}}}
               {\polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                          {\expr}{\loccx_{i}}{\overline{\typ}}
                          {\typ}{\loccx_{o}}
               }
               {\loccx}{\dynenv}.
Because \yy is in the original typing environment,
by the premise of the rule it is different than \ff and $\overline{\xx}$,
so (5) $(\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}})[\val/\yy] = \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e[\val/\yy]}}$,
which concludes the proof.
\item \textbf{Rules \ttrue, \tfalse, \tconstint, \ttptr, and \tumem:}
Trivial because $\ee[\val/\xx] = \ee$ and typing does not depend on the environment \env.

    % \item \textbf{Rule \tskip:}
    % \stmtyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_\xx},\env_2}{\loccx}{\dynenv}{\sskip}{\loccx}{\dynenv}.
    % By rule \tskip, trivially,
    % \stmtyping{\varcx}{\env_1,\env_2}{\loccx}{\dynenv}{\sskip\subst{\xx}{\val}}{\loccx}{\dynenv}.

    \item \textbf{Rule \tassign:}
    (1) \stmtyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_\xx},\env_2}{\loccx_i}{\dynenv}{\sassign{\place}{\ee'}}{\loccx_o}{}.
    By inversion:
    (2) \rvaltyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_\xx},\env_2}{\loccx_i}{\dynenv}{\ee'}{\typ_v}{\loccx_o},
    (3) \pltyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_\xx},\env_2}{\loccx_i}{\dynenv}{\place}{\tref{\mut}{\typ}}{\loccx_i}, and
    (4) \subtyping{\typ_v}{\typ}.
    By inductive hypothesis on (2) and (3):
    (5) \rvaltyping{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\rval\subst{\xx}{\ee'}}{\typ_v}{\loccx_o},
    (6) \pltyping{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\place\subst{\xx}{\ee'}}{\tref{\mut}{\typ}}{\loccx_i}.
    The proof concludes by rule (5), (6), (4), and \tassign.

    \item \textbf{Rule \tassignstrg:}
    (1) \stmtyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_\xx},\env_2}{\loccx_i}{\dynenv}{\sassign{\place}{\ee'}}{\loccx_o[\loc \mapsto \typ]}{}.
    By inversion:
    (2) \rvaltyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_\xx},\env_2}{\loccx_i}{\dynenv}{\ee'}{\typ}{\loccx_o} and
    (3) \pltyping{\varcx}{\env_1,\mapstoenv{\xx}{\typ_\xx},\env_2}{\loccx_i}{\dynenv}{\place}{\tptr{\loc}}{\loccx_i}.
    By inductive hypothesis on (2) and (3):
    (4) \rvaltyping{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\rval\subst{\xx}{\ee'}}{\typ}{\loccx_o} and
    (5) \pltyping{\varcx}{\env_1,\env_2}{\loccx_i}{\dynenv}{\place\subst{\xx}{\ee'}}{\tptr{\loc}}{\loccx_i}.
    The proof concludes by (4), (5), and rule \tassignstrg.

    \item \textbf{Rules \tstrgrebor, \tstrgmutrebor, \tmutmutrebor and \tshrrebor} The proof goes by case splitting on the rules,
inversion, application of the inductive hypothesis, and application of the respective rule.

\end{itemize}
\end{proof}

% \begin{lemma}[Existential Values]\label{existential:values}
% If $\typing{\varcx}{\env_1}{\loccx}{\dynenv}{\val}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}{\loccx}{}$
% then
% \sortck[\varcx]{\interp{\val}}{\getsort{\tcon}}
% and
% \lmodel{\varcx}{\expr[\interp{\val}/\aa]}.
% \end{lemma}
% \begin{proof}
%     Let {\tcon = \tint: }
%     By lemma~\ref{lemma:canonical}, $\val = \interp{\val} = n$, for some $n \in \mathbb{Z}$.
%     Thus, \sortck[\varcx]{n}{\getsort{\tint}} holds.
%     Since subtyping is reflexive and transitive (lemmata\ref{lemma:subtype:trans} and~\ref{lemma:subtype:refl}),
% the value derivation tree was the following:
% $$
% \inferrule*[Right=\tsub]
%         {
%           {\inferrule*[Right=\tconstint]
%           {}
%           {\typing{\varcx}{\env}{\loccx}{\dynenv}{n}{\rtyp{\tint}{n}}{\loccx}{\dynenv}}} \\
%           \\
%             \subtyping{\rtyp{\tint}{n}}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}} \\
%             \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx}{\loccx}\\
%         }
%         {
%             \typing{\varcx}{\env}{\loccx_i}{\dynenv}{n}
%                 {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}
%                 {\loccx}
%                 {\dynenv}
%         }
% $$
% Thus, by inversion \subtyping{\rtyp{\tint}{n}}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}.
% By inverting the rule \subexists
% we get the requirement \entailment{\varcx}{\expr[n/\aa]}.

% The proof is the same for $\tcon = \tbool$.

% \end{proof}

\begin{lemma}[Subtyping Reflexive]\label{lemma:subtype:refl}
  \subtyping{\typ}{\typ}
\end{lemma}
\begin{proof}
By induction on the structure of \typ:
\begin{itemize}
  \item $\typ \equiv \rtyp{\tcon}{\expr}$.
  Since, by assumption~\ref{assumption:model:reflexive} \entailment{\varcx}{\expr = \expr},
  by rule \subrtyp we get
  \subtyping{\rtyp{\tcon}{\expr}}{\rtyp{\tcon}{\expr}}.
  \item $\typ \equiv \texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}$.
  By assumption~\ref{assumption:model:identity}, we have
  (1) \entailment{\varcx, \aa:\getsort{\tcon}, \expr}{\expr}.
  By lemma~\ref{lemma:subst:idvar}, we have:
  (2) \entailment{\varcx, \aa:\getsort{\tcon}, \expr}{\expr\subst{\aa}{\aa}}.
  By (2) and rule \subexists,
  (3) \subtyping[\varcx, \aa:\getsort{\tcon}, \expr]
            {\rtyp{\tcon}{\aa}}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}.
  By (3) and rule \subunpack, we conclude the proof.
  \item $\typ \equiv \tptr{\loc}$. Trivially, by rule \subptr.
  \item $\typ \equiv \uninit{n}$. Trivially, by rule \submem.
  \item $\typ \equiv \tbor{\lft}{\shr}{\typ'}$.
  By inductive hypothesis on $\typ'$ and rule \subborshr.
  \item $\typ \equiv \tbor{\lft}{\mut}{\typ'}$.
  By inductive hypothesis on $\typ'$ and rule \subbormut.
  \item $\typ \equiv \polysig{\overline{\tvar}}
  {\overline{\aa: \sort}}
  {\expr}
  {\loccx_i}
  {\overline{\typ}}
  {\typ_o}
  {\loccx_o}$.
  By assumption~\ref{assumption:model:identity}:
  (1) \entailment{\varcx, \overline{\aa: \sort}}{\expr \Rightarrow \expr}.
  By lemma~\ref{context:reflexive}
  (2) \loccxinc
  {\varcx, \overline{\aa: \sort}}
  {\elftcx}{\llftcx}
  {\loccx_{i}}
  {\loccx_{i}} and
  (3) \loccxinc
  {\varcx, \overline{\aa: \sort}}
  {\elftcx}{\llftcx}
  {\loccx_{o}}
  {\loccx_{o}}.
  By inductive hypothesis:
  (4) $\forall i. \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{i}}{\typ_{i}}$ and
  (5) \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{o}}{\typ_{o}}.
  The proof concludes by (1)-(5) and rule \subfun.
\end{itemize}
\end{proof}

\begin{lemma}[Context Inclusion Reflexive]\label{context:reflexive}
  Forall \varcx and \loccx, \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx}{\loccx}.
\end{lemma}
\begin{proof}
  By rule \loccxincperm.
\end{proof}


\begin{lemma}[Strengthening]\label{lemma:strengthen}
  Let \env be an environment that does not contain any variables bound at \ee, $\env_1$, or $\env_2$.
  If \typing{\varcx}{\env_1, \env_2}{\loccx_i}{\dynenv}{\ee}{\typ}{\loccx_o}{},
  then \typing{\varcx}{\env_1, \env, \env_2}{\loccx_i}{\dynenv}{\ee}{\typ}{\loccx_o}{}.
\end{lemma}
\begin{proof}
By induction on the derivation tree.
\newline
%%% EXPRESSIONS
We split cases on the typing derivation tree:
  \begin{itemize}
      \item \textbf{Rule \tsub:}
      By inductive hypothesis and rule \tsub.
      \item \textbf{Rule \tlet:}
      (1) \typing{\varcx}{\env_1, \env_2}{\loccx_i}{\dynenv}{\blet{\xx}{\ee_{\xx}}{\ee}}{\typ}{\loccx_o}{\dynenv_o}.
      By inversion:
      (2) \typing{\varcx}{\env_1, \env_2}{\loccx_i}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv},
      (3) \typing{\varcx}{\env_1, \env_2,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv_o}, and
      (4) $\xx \not \in \dom{\env_1, \env_2}$.
      By inductive hypothesis on (2) and (3):
      (5) \typing{\varcx}{\env_1, \env, \env_2}{\loccx_i}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv} and
      (6) \typing{\varcx}{\env_1, \env, \env_2,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv_o}.
      By hypothesis and (4): (7) $\xx \not \in \dom{\env_1,\env, \env_2}$.
      By (5)-(7) and rule \tlet we conclude the proof.

      \item \textbf{Rule \tnew:}
      By inductive hypothesis, assumption, and rule \tnew.
      \item \textbf{Rule \tif:}
      By inductive hypothesis and rule \tif.
      % \item \textbf{Rule \tseq:}
      % By induction hypothesis, case~\ref{lemma:strengthen:stmt}, and rule~\tseq.
      \item \textbf{Rule \tunpack:}
      We split two cases based on the location of \xx. Both go by inductive hypothesis and rule \tunpack.
      \item \textbf{Rule \tcall:}
      By inductive hypothesis and rule \tcall.
      \item \textbf{Rule \ttvar:}
      Since the domains of the environments are disjoint,
      $\mapstoenv{\xx}{\typ} \in \env_1,\env, \env_2$.
      \item \textbf{Rule \tfun:}
      By inductive hypothesis and rule \tfun.
      \item \textbf{Rules \ttrue, \tfalse, \tconstint, \ttptr, \tumem:}
      Trivial since the rules do not depend on the typing environment.

      \item \textbf{Rules \tassign and \tassignstrg} By inductive hypothesis.

      \item \textbf{Rules \tstrgrebor, \tstrgmutrebor, \tmutmutrebor, \tshrrebor , \tderef and \tderefstrg:} By inductive hypothesis.
  \end{itemize}
\end{proof}



\begin{lemma}[Well Formedness]\label{lemma:wf}
  If \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv}
  and \wf{\env}, \wf{\loccx_i}, \wf{\dynenv},
  then \wf{\loccx_o} and \wf{\typ}.
\end{lemma}
\begin{proof}
By induction on the type derivation trees.
\end{proof}

\begin{lemma}[Subtyping weakening]\label{lemma:varcx-subtyping-weakening}
    \quad
    \begin{enumerate}
    \item If \subtyping[\varcx_1,\varcx_2]{\typ_1}{\typ_2} then \subtyping[\varcx_1,\varcx',\varcx_2]{\typ_1}{\typ_2}.
    \item If \loccxinc{\varcx_1,\varcx_2}{}{}{\loccx_1}{\loccx_2} then \loccxinc{\varcx_1,\varcx',\varcx_2}{}{}{\loccx_1}{\loccx_2}.
    \end{enumerate}
\end{lemma}
\begin{proof}
    By mutual induction in the definition of subtyping and context inclusion generalizing over $\varcx_2$.
    \begin{itemize}
        \item \textbf{Case \subptr, \submem:} Direct by applying the rules since they do not depend on the logical context.
        \item \textbf{Case \subbormut, \subborshr:} By applying the induction hypothesis for (1)
        \item \textbf{Case \subrtyp:} By assumption~\ref{assumption:model:weakening}
        \item \textbf{Case \subunpack:} By applying the induction hypothesis for (1) picking
        $\varcx_2,\aa:\getsort{B},\expr$ for the generalized logical context.
        \item \textbf{Case \subexists:} By assumption~\ref{assumption:model:weakening}.
        \item \textbf{Case \subfun:} By inductive hypotheses and assumption~\ref{assumption:model:weakening}.
        \item \textbf{Case \loccxincperm,\loccxincweaken:} Direct by applying the rules since they do not depend on the logical context.
        \item \textbf{Case \loccxincframe, \loccxincsub:} By inductive hypotheses.
    \end{itemize}
\end{proof}

\begin{restatable}[Value refinement]{lemma}{valuerefinement}
\label{lemma:value-refinement}
Given $\typing{\varcx}{\env}{\loccx}{\dynenv}{\val}{\typ}{\loccx}{}$.
The following holds:
\begin{enumerate}
    \item If $\typ = \bty[\expr]$ then \sortck{\interp{\val}}{\getsort{\tcon}} and \entailment{\varcx}{\expr = \interp{\val}}.
    \item If $\typ = \texists{\aa}{\bty[\aa]}{\expr}$ then \sortck{\interp{\val}}{\getsort{\bty}} and \entailment{\varcx}{\expr[\interp{\val}/\aa]}
\end{enumerate}
\end{restatable}
\begin{proof}
    By induction on the typing derivation generalizing over \varcx.
    The following cases apply to values.
    \begin{itemize}
        \item \textbf{Case \tconstint,\ttrue, \tfalse:} Only the premise of (1) holds.
        The conclusion is direct since the rules assign the exact value to the index.

        \item \textbf{Case \tvecvec:} Only the premise of (1) holds.
        The conclusion is direct since the rule assigns the length of the vector as the index which
        is exactly the interpretation of vectors.

        \item \textbf{Case \tsub:} By inversion of the rule we have:
        \begin{enumerate}
            \setcounter{enumi}{2}
            \item \typing{\varcx}{\env}{\loccx}{\dynenv}{\val}{\typ'}{\loccx}{}
            \item \subtyping{\typ'}{\typ}
        \end{enumerate}
        We prove (1) and (2) separately, assuming the premise in each case:
        \begin{itemize}
            \item $\typ = \bty[\expr]$. By inversion of (4) we have two cases
            \begin{itemize}
                \item \textbf{Case \subrtyp:} (4) becomes \subtyping{\bty[\rexpr']}{\bty[\rexpr]}.
                The conclusion of (1) then follows from the premise of \subrtyp, the inductive hypotheses applied to (3) and
                Assumption~\ref{assumption:model:transitive}.

                \item \textbf{Case \subunpack:} (3) becomes
                \typing{\varcx}{\env}{\loccx}{\dynenv}{\val}{\texists{\aa}{\bty[\aa]}{\expr'}}{\loccx}{}.
                and (4) becomes \subtyping{\texists{\aa}{\bty[\aa]}{\expr'}}{\bty[\expr]}.
                By inversion of (4) we have \subtyping[\varcx,\aa:\getsort{B},\expr']{\bty[\aa]}{\bty[\expr]}, and
                again by inversion we have \entailment{\varcx,\aa:\getsort{B},\expr'}{\aa = \expr}.
                By the inductive hypothesis applied to (3) we have \entailment{\varcx}{\expr'[\interp{\val}/\aa]} and
                \sortck{\interp{\val}}{\getsort{\bty}}.
                By Lemma~\ref{lemma:existential-indexed-value} applied to (3) we have
                (5) \typing{\varcx,\aa:\getsort{B},\expr'}{\env}{\loccx}{\dynenv}{\val}{\bty[\aa]}{\loccx}{}.
                Applying the inductive hypothesis to (5) we get \entailment{\varcx,\aa:\getsort{B},\expr'}{\aa = \interp{\val}}.
                Summarizing, we have
                (a) \entailment{\varcx,\aa:\getsort{B},\expr'}{\aa = \expr},
                (b) \entailment{\varcx}{\expr'[\interp{\val}/\aa]}, and
                (c) \entailment{\varcx,\aa:\getsort{B},\expr'}{\aa = \interp{\val}}.
                We can apply Assumption~\ref{assumption:model:substitution} with (a) and (b).
                To get \entailment{\varcx,\expr'[\interp{\val}/\aa]}{\interp{\val} = \expr} and then apply
                Assumption~\ref{assumption:model:cut} to get \entailment{\varcx}{\interp{\val}=\expr} which concludes
                this part of the proof.
            \end{itemize}
            \item $\typ = \texists{\aa}{\bty[\aa]}{\expr}$. By inversion of (4) we have two cases:

            \begin{itemize}
                \item \textbf{Case \subexists:} (4) becomes \subtyping{\bty[\expr']}{\texists{\aa}{\bty[\aa]}{\expr}}.
                By inversion of (4) we have (5) \entailment{\varcx}{\expr[\expr'/\aa]}. By applying the inductive
                hypothesis to (3) we have \sortck{\interp{\val}}{\getsort{\bty}} and
                (6) \entailment{\varcx}{\expr' = \interp{\val}}.
                We conclude this part of the proof by Assumption~\ref{assumption:model:congruence}.
                \item \textbf{Case \subunpack:} (3) becomes
                \typing{\varcx}{\env}{\loccx}{\dynenv}{\val}{\texists{\aa}{\bty[\aa]}{\expr'}}{\loccx}{}
                and (4) becomes \subtyping{\texists{\aa}{\bty[\aa]}{\expr'}}{\texists{\aa}{\bty[\aa]}{\expr}}.
                By inverting (4) twice we get \entailment{\varcx,\aa:\getsort{B},\expr'}{\expr}.
                Applying the inductive hypothesis to (3) we get \entailment{\varcx}{\expr'[\interp{\val}/\aa]}
                and \sortck{\interp{\val}}{\getsort{\bty}}.
                By using Assumption~\ref{assumption:model:substitution} we get \entailment{\varcx,\expr'[\interp{\val}/\aa]}{\expr[\interp{\val}/\aa]}.
                We conclude by using Assumption~\ref{assumption:model:cut}.
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{proof}

\begin{lemma}\label{lemma:existential-indexed-value}
    If \typing{\varcx}{\env}{\loccx}{\dynenv}{\val}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}{\loccx}{} then
    \typing{\varcx,\aa:\getsort{B},\expr}{\env}{\loccx}{\dynenv}{\val}{\rtyp{\tcon}{\aa}}{\loccx}{}
\end{lemma}
\begin{proof}
    By applying \tsub and using \tunpack and Lemma~\ref{lemma:varcx-typing-weakening} to prove its premises.
\end{proof}


\begin{lemma}[Logical context weakening]\label{lemma:varcx-typing-weakening}
    If \typing{\varcx_1,        \varcx_2}{\env}{\loccx_i}{\dynenv}{\ee}{\typ}{\loccx_o}{} then
       \typing{\varcx_1,\varcx',\varcx_2}{\env}{\loccx_i}{\dynenv}{\ee}{\typ}{\loccx_o}{}.
\end{lemma}
\begin{proof}
    By induction in the typing derivation generalizing over $\varcx_2$.
    Most cases follow by applying the rule directly or by the inductive hypotheses.
    The interesting cases are:
    \begin{itemize}
        \item \textbf{Case \tassign,\tshrrebor,\tstrgmutrebor,\tsub} By applying the inductive hypotheses
        and Lemma~\ref{lemma:varcx-subtyping-weakening}.
        \item \textbf{Case \tcall:} Follows from assumption~\ref{assumption:model:weakening},
        the inductive hypothesss, and Lemma~\ref{lemma:varcx-subtyping-weakening}.
    \end{itemize}
\end{proof}


==> metatheory/memory-events-lemmata.tex <==
\begin{lemma}[Allocation event]\label{lemma:event:alloc}
If
\begin{itemize}
  \item \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i} and
  \item \transnew{\sbstate_i}{\sbstate_o}
\end{itemize}
then

\statetyping[\varcx][\loccx,\mapstoowned{\cloc}{\uninit{1}}][\dynenv,\mapstoowned{(\cloc, \ptrtag)}{\tptr{\cloc}}]{\hp\hbind{\cloc}{\poison}}{\sbstate_o}
\end{lemma}
\begin{proof}
    Since \transnew{\sbstate_i}{\sbstate_o} we know by inversion of \osdealloc that $\cloc\notin\dom{\sbstate_i\dotstacks}$.
    Then, by definition of \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i}, we have that $\cloc\notin\dom{\hp}$,
    consequently the update does not invalidate any of the other locations.
    We also have by \tumem that \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv}{\poison}{\uninit{1}}.
    It remains to show that
    \stacktyping[\varcx][\dynenv,(\cloc,\ptrtag)\mapsto\tptr{\cloc}]{\shr}{\cloc}{(\unique, \ptrtag, \bot)}{\uninit{1}}
    which follows directly by the definition of well-typed stacks.
\end{proof}


\begin{lemma}[Strong-Reborrow event]\label{lemma:event:strg-rebor}
If
\begin{itemize}
    \item \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i},
    \item $\dynenv(\cloc, \ptrtag) = \tptr{\cloc}$ and
    \item \transreborrow{\sbstate_i}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\mut}}{\sbstate_o}
\end{itemize}
then

\statetyping[\varcx][\loccx][\dynenv,\mapstoowned{(\cloc,\ptrtag')}{\tptr{\cloc}}]{\hp}{\sbstate_o}
\end{lemma}
\begin{proof}
    Since \transreborrow{\sbstate_i}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\mut}}{\sbstate_o}
    we know that $\sbstate_o\dotstacks(\cloc)$ must contain $(\unique, \ptrtag', \_)$ at the top
    followed by $(\unique, \ptrtag, \_)$.
    Since \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i} and $\dynenv(\cloc,\ptrtag)=\tptr{\cloc}$,
    then \hpstrg must have been used to derive the prefix of the stack was well-typed, thus \hpstrg also holds
    if we add $(\unique, \ptrtag', \_)$ to the top of the stack.
\end{proof}

\begin{lemma}[Weaken-Reborrow event]\label{lemma:event:weaken-rebor}
If
\begin{itemize}
    \item \subtyping{\loccx(\cloc)}{\typ},
    \item $\dynenv(\cloc, \ptrtag) = \tptr{\cloc}$,
    \item \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i} and
    \item \transreborrow{\sbstate_i}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\mut}}{\sbstate_o}
\end{itemize}
then

$\statetyping[\varcx][\loccx[\cloc\mapsto\typ]][\dynenv,\mapstoowned{(\cloc,\ptrtag')}{\tref{\mut}{\typ}}]{\hp}{\sbstate_o}$
\end{lemma}
\begin{proof}
    Similar to Lemma~\ref{lemma:event:strg-rebor} we know that $\sbstate_o\dotstacks(\cloc)$ must
    contain $(\unique, \ptrtag', \_)$ at the top followed by $(\unique, \ptrtag, \_)$.
    We can apply \hptracked to show the heaplet is well-typed after the update applying
    \hpmut to show the stack is well typed.
    Let $\dynenv' = \dynenv,\mapstoowned{(\cloc,\ptrtag')}{\tref{\mut}{\typ}}  $
    It suffices to show \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv'}{\hp(\cloc)}{\typ}.
    Since $\cloc \in \loccx$ then \hptracked must have been applied to prove well-typedness of the
    initial state, therefore we have \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv}{\hp(\cloc)}{\loccx(\cloc)}.
    By Lemma~\ref{lemma:weakening} we have
    \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv'}{\hp(\cloc)}{\loccx(\cloc)} and by subsumption
    \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv'}{\hp(\cloc)}{\typ}.
\end{proof}

\begin{lemma}[Mut-Reborrow event]\label{lemma:event:mut-rebor}
If
\begin{itemize}
    \item $\dynenv(\cloc, \ptrtag) = \tref{\mut}{\typ}$
    \item \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i} and
    \item \transreborrow{\sbstate_i}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\mut}}{\sbstate_o}
\end{itemize}
then

\statetyping[\varcx][\loccx][\dynenv,\mapstoowned{(\cloc,\ptrtag')}{\tref{\mut}{\typ}}]{\hp}{\sbstate_o}
\end{lemma}
\begin{proof}
    Since \transreborrow{\sbstate_i}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\mut}}{\sbstate_o} we have
    that $\sbstate_o\dotstacks(\cloc)$ must contain $(\unique, \ptrtag',\_)$ at the top.
    We also know the prefix of the stack must be well-typed.
    We conclude by applying \hpmut to show the stack updated with the new item is well-typed.
\end{proof}

\begin{lemma}[Shared-Reborrow event]\label{lemma:event:shr-rebor}
If
\begin{itemize}
    \item $\dynenv(\cloc, \ptrtag) = \tref{\bormode}{\typ}$
    \item \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i} and
    \item \transreborrow{\sbstate_i}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\shr}}{\sbstate_o}
\end{itemize}
then

\statetyping[\varcx][\loccx][\dynenv,\mapstoowned{(\cloc,\ptrtag')}{\tref{\shr}{\typ}}]{\hp}{\sbstate_o}
\end{lemma}
\begin{proof}
    By well-typedness of the input stack either \hpmut or \hpshr was applied.
    In both cases we know $\subtyping{\typ}{\typ'}$ for some $\typ'$.
    We also know the retag transition only remove items from the stack, thus the prefix of the
    output stack must also be well-typed.
    We conclude by applying \hpshr to prove the output stack is well-typed after the update.
\end{proof}

\begin{lemma}[Read event]\label{lemma:event:read}
If
\begin{itemize}
    \item $\statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i}$,
    \item $\dynenv(\cloc, \ptrtag) = \tref{\bormode}{\typ}$ and
    \item \transread{\sbstate_i}{\cloc}{\ptrtag}{\sbstate_o}
\end{itemize}
then
\begin{itemize}
    \item $\valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\hp(\cloc)}{\typ}$ and
    \item $\statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_o}$.
\end{itemize}
\end{lemma}
\begin{proof}
    Since \transread{\sbstate_i}{\cloc}{\ptrtag}{\sbstate_o} the stack must have a granting
    item with tag $\ptrtag$.
    Because the initial stack is well-typed then either one of \hpshr or \hpmut must have been
    used for the granting item.
    In both cases we know \subtyping{\typ'}{\typ} for some \typ'.
    In both cases we know \valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\hp(\cloc)}{\typ'}
    because either \hptracked or \hpuntracked must apply.
    The by subsumption we know \valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\hp(\cloc)}{\typ} which
    is the first part of the conclusion.
    The second part follows from the fact that the read access transition can only change
    \unique permissions into \disabled, and thus we can apply \hpdisabled to prove the output
    stack is well-typed.
\end{proof}

\begin{lemma}[Strong read event]\label{lemma:event:strg-read}
If
\begin{itemize}
    \item $\cloc \in \dom{\loccx}$
    \item $\statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_i}$,
    \item \transread{\sbstate_i}{\cloc}{\ptrtag}{\sbstate_o}
\end{itemize}
then
\begin{itemize}
    \item $\valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\hp(\cloc)}{\loccx(\cloc)}$ and
    \item $\statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate_o}$.
\end{itemize}
\end{lemma}
\begin{proof}
    The first part of the conclusion follows directly by the definition of well-formed heaps since
    \hptracked must apply.
    The second part follows from the fact that the read access transition can only change
    \unique permissions into \disabled, and thus we can apply \hpdisabled to prove the output
    stack is well-typed.
\end{proof}

\begin{lemma}[Weak write event]\label{lemma:event:weak-write}
If
\begin{itemize}
    \item \statetyping{\hp}{\sbstate_i},
    \item \dynenv(\cloc, \ptrtag) = \tref{\mut}{\typ},
    \item \valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\val}{\typ}, and
    \item \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate_o}.
\end{itemize}
then

\statetyping{\hp\hbind{\cloc}{\val}}{\sbstate_o}
\end{lemma}
\begin{proof}
    After the update $\sbstate_o\dotstacks(\cloc)$ must contain $(\unique,\ptrtag, \_)$ at the top.
    Because the stack was well-typed before the update by inversion of \hpmut
    we have (1) \subtyping{\typ}{\loccx(\cloc)}.
    By (1) and subsumption we have \valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\val}{\loccx(\cloc)},
    thus we can stil use \hptracked to prove the heaplet is well-typed after the update.
    We conclude by noting that the output stack must also be well-typed because items
    are only popped from it.
\end{proof}

\begin{lemma}[Strong write event]\label{lemma:event:strg-write}
If
\begin{itemize}
    \item \statetyping{\hp}{\sbstate_i},
    \item \dynenv(\cloc, \ptrtag) = \tptr{\cloc},
    \item \valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\val}{\typ}
    \item \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate_o} and
\end{itemize}
then

\begin{itemize}
    \item \statetyping[\varcx][\loccx[\cloc\mapsto\typ]]{\hp\hbind{\cloc}{\val}}{\sbstate_o}
\end{itemize}
\end{lemma}
\begin{proof}
    After the transition, $\sbstate_o\dotstacks(\cloc)$ must contain $(\unique, \ptrtag, \_)$ at
    the top and because $\dynenv(\cloc,\ptrtag) = \tptr{\cloc}$, the output stack only contains tags
    that are mapped to pointers in \dynenv.
    Therefore, there is nothing else to prove to show the output stack is well-typed.
    Finally, the heap is well-typed because we are updating \loccx to point to the new type \typ.
\end{proof}

\subsubsection{Lemmata about Vector Memory Events}

\begin{lemma}[Vec push empty]\label{lemma:vec:push-empty}
Let
\begin{itemize}
    \item $\hp_i=\hp\hbind{\cloc}{\vvec{0}{\val'}}$ and
    \item $\hp_o=\hp\hbind{\cloc}{\vvec{1}{\vptr{\cloc'}{\ptrtag'}}}\hbind{\cloc'}{\val}$.
\end{itemize}
If
\begin{itemize}
    \item $\dynenv(\cloc, \ptrtag) = \tptr{\cloc}$
    \item \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv}{\val}{\typ},
    \item \statetyping[\varcx][\loccx][\dynenv]{\hp_i}{\sbstate_i}, and
    \item \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate},
    \item \transalloc{\sbstate}{\cloc'}{\ptrtag'}{1}{\sbstate_o},
\end{itemize}
then

\statetyping
    [\varcx]
    [\loccx[\cloc \mapsto \rtyp{\tvec}{1}]]
    [\dynenv,(\cloc', \ptrtag') \mapsto \tref{\mut}{\typ}]
    {\hp_o}
    {\sbstate_o} and
\end{lemma}
\begin{proof}
    Let $\dynenv_o=\dynenv,(\cloc', \ptrtag') \mapsto \tref{\mut}{\typ}$.
    We can apply \tvecvec to show
    \typing{\varcx}{\emptyset}{\emptyset}{\dynenv_o}{\vvec{1}{\vptr{\cloc'}{\ptrtag'}}}{\rtyp{\tvec}{1}}{\emptyset}{}.
    Since \val has type \typ then the output stack will be well-typed in $\dynenv_o$.
    We conclude by using the same argument in Lemma~\ref{lemma:event:strg-write} to prove we can
    update the type of \cloc in \loccx.
\end{proof}

\begin{lemma}[Vec push]\label{lemma:vec:push}
Let
\begin{itemize}
    \item $\hp_i=\hp\hbind{\cloc}{\vvec{n}{\vptr{\cloc'}{\ptrtag'}}}\hbindn{n}{\cloc'}{\overline{\val}}$,
    \item $\hp_o=\hp\hbind{\cloc}{\vvec{n+1}{\vptr{\cloc''}{\ptrtag''}}}\hbindn{n+1}{\cloc''}{\overline{\val} \append [\val]}$, and
    \item $\dynenv_o=(\dynenv_i - (\cloc', \_))[(\cloc'' + i, \ptrtag') \mapsto \tref{\mut}{\typ} | i \in [0, n]]$.
\end{itemize}
If
\begin{itemize}
    \item \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv_i}{\val}{\typ},
    \item \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate},
    \item \transdealloc{\sbstate}{\cloc'}{\ptrtag'}{n}{\sbstate'},
    \item \transalloc{\sbstate'}{\cloc''}{\ptrtag''}{n+1}{\sbstate_o},
    \item \statetyping[\varcx][\loccx][\dynenv_i]{\hp_i}{\sbstate_i}, and
    \item $\dynenv(\cloc, \ptrtag) = \tptr{\cloc}$
\end{itemize}
then

\statetyping
    [\varcx]
    [\loccx[\cloc \mapsto \rtyp{\tvec}{n + 1}]]
    [\dynenv_o]
    {\hp_o}
    {\sbstate_o} and
\end{lemma}
\begin{proof}
    By well-typedness of the input state we know
    \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv_i}{\vvec{n}{\vptr{\cloc'}{\ptrtag'}}}{\rtyp{\tvec}{n}}.
    Then, by inversion of \tvecvec we know $\dynenv_i(\cloc' + i, \ptrtag') = \tref{\mut}{\typ}$ for $i \in [0, n)$
    which together with well-typedness of the input state implies
    \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv_i}{\hp_i(\cloc + i)}{\typ}.
    Thus, since the new value \val also has type \typ, after the update all the relocated values have type \typ.
    We can then apply \tvecvec to prove \vvec{n+1}{\vptr{\cloc''}{\ptrtag''}} has type \rtyp{\tvec}{n+1} under $\dynenv_o$, and
    conclude using the same argument in Lemma~\ref{lemma:event:strg-write} to prove we can update the type of \cloc in \loccx.
\end{proof}

\begin{lemma}[Vec index mut]\label{lemma:vec:indexmut}
If
\begin{itemize}
    \item $\dynenv(\cloc, \ptrtag) = \tref{\mut}{\rtyp{\tvec}{n}}$,
    \item $\hp(\cloc) = \vvec{n}{\vptr{\cloc'}{\ptrtag'}}$,
    \item \transread{\sbstate_i}{\cloc}{\ptrtag}{\sbstate}, and
    \item \transreborrow{\sbstate}{\cloc' + i}{\ptrtag'}{\ptrtag''}{\mut}{\sbstate_o}
    \item \statetyping{\hp}{\sbstate_i}
\end{itemize}
then

\statetyping
    [\varcx]
    [\loccx]
    [\dynenv,(\cloc' + i, \ptrtag'') \mapsto \tref{\mut}{\typ}]
    {\hp}
    {\sbstate_o} and
\end{lemma}
\begin{proof}
    By Lemma~\ref{lemma:event:read} we have
    \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv}{\vvec{n}{\vptr{\cloc'}{\ptrtag'}}}{\rtyp{\tvec}{n}}.
    By inversion of \tvecvec we have $\dynenv(\cloc' + i , \ptrtag') = \tref{\mut}{\typ}$ for $i \in [0, n)$.
    We conclude by applying Lemma~\ref{lemma:event:mut-rebor}.
\end{proof}


==> metatheory/models.tex <==
\subsection{Implication Checking}

Implication checking \lmodel{\varcx}{\expr} is implemented via SMT.
Here we axiomatize the properties we need for the proof.

\begin{assumption}[Weakening]\label{assumption:model:weakening}
    If \lmodel{\varcx_1,\varcx_2}{\expr} then \lmodel{\varcx_1, \varcx', \varcx_2}{\expr}.
\end{assumption}

% \begin{assumption}[Strengthening]\label{assumption:model:strengthening}
%     If \lmodel{\varcx_1}{\expr} and $\dom{\varcx_1} \cap \dom{\varcx_2} = \emptyset$,
%     then \lmodel{\varcx_1, \varcx_2}{\expr}.
% \end{assumption}

\begin{assumption}[Cut]\label{assumption:model:cut}
    If \lmodel{\varcx_1}{\expr_1} and
       \lmodel{\varcx_1, \expr_1, \varcx_2}{\expr_2},
    then \lmodel{\varcx_1, \varcx_2}{\expr_2}.
\end{assumption}

\begin{assumption}[Identity]\label{assumption:model:identity}
    Forall \varcx and \expr, \lmodel{\varcx, \expr}{\expr}.
\end{assumption}

\begin{assumption}[Substitution]\label{assumption:model:substitution}
    If \sortck[\varcx_1]{\expr_\aa}{\sort} and \entailment{\varcx_1, \aa:\sort, \varcx_2}{\expr},
    then \entailment{\varcx_1, \varcx_2[\expr_\aa/\aa]}{\expr[\expr_\aa/\aa]}.
\end{assumption}

\begin{assumption}[Transitive]\label{assumption:model:transitive}
    If \entailment{\varcx}{\expr_1 = \expr_2} and \entailment{\varcx}{\expr_2 = \expr_3},
    then \entailment{\varcx}{\expr_1 = \expr_3}.
\end{assumption}

\begin{assumption}[Transitivity of Implication]\label{assumption:model:transitive:implication}
    If \entailment{\varcx}{\expr_1 \Rightarrow \expr_2} and \entailment{\varcx}{\expr_2 \Rightarrow \expr_3},
    then \entailment{\varcx}{\expr_1 \Rightarrow \expr_3}.
\end{assumption}

\begin{assumption}[Congruence]\label{assumption:model:congruence}\label{assumption:model:equality}
    If \entailment{\varcx}{\expr_1 = \expr_2} and \entailment{\varcx}{\expr[\expr_2/\aa]},
    then \entailment{\varcx}{\expr[\expr_1/\aa]}.
\end{assumption}

\begin{assumption}[Reflexivity]\label{assumption:model:reflexive}
    \lmodel{\varcx}{\expr = \expr}.
\end{assumption}


==> metatheory/operational.tex <==
The operational semantics follows a sandard call-by-value evaluation.
%
Note that function arguments are A-values and thus they must not be
further evaluated.
%
We use the convention that a rule with a stacked borrow transition
as a premise does not get stuck if the transition does not hold but
instead evaluates to an error.
%
In \opvecindexmut{}, for example, evaluation will return an error
if either the \text{EAccess} or \text{ERetag} transition does not hold,
but it will get stuck if the index does not point to a valid location.

$$
\begin{array}{rrcll}
    \syntaxcat{Heap} &
        \hp  & ::= & \emptyset \mid \hp\hbind{\cloc}{\hval}  \\
    \syntaxcat{Contexts} &
        \CC  & ::= & \bullet \mid \blet{\xx}{\CC}{e}
              \mid \bif{\CC}{\ee}{\ee}
              \mid \fcall{\CC}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}
              \mid \sassign{\place}{\CC} \\
\end{array}
$$

\begin{judgment}{Operational Semantics}{\eval{\hp}{\sbstate}{\rexpr}{\hp}{\sbstate}{\rexpr} or \evalerr{\hp}{\sbstate}{\ee}}
  \inferrule[\opprop]
    { \eval{\hp_i}{\sbstate_i}{\ee}{\hp_o}{\sbstate_o}{\ee'}}
    {\eval{\hp_i}{\sbstate_i}{\CC[\ee]}
          {\hp_o}{\sbstate_o}{\CC[\ee']}}


  \inferrule[\opproperr]
    {\evalerr{\hp_i}{\sbstate_i}{\ee}}
    {\evalerr{\hp_i}{\sbstate_i}{\CC[\ee]}}


  \inferrule[\opnew]
    {\fresh{\cloc}{\hp} \\ \transnew{\sbstate}{\sbstate'} }
    {\eval{\hp}{\sbstate}{\blet{\xx}{\new{\lvar}}{\rexpr}}
          {\hp\hbind{\cloc}{\poison}}{\sbstate'}{\rexpr[\cloc/\lvar][\vptr{\cloc}{\ptrtag}/\xx]}}

  \inferrule[\oplet]
    {}
    {\eval{\hp}{\sbstate}{\blet{\xx}{\val}{\rexpr}}
          {\hp}{\sbstate}{\rexpr[\val/\xx]}}

  \inferrule[\opifTrue]
    {}
    {\eval{\hp}{\sbstate}{\bif{\ctrue}{\rexpr_1}{\rexpr_2}}
          {\hp}{\sbstate}{\rexpr_1}}

  \inferrule[\opifFalse]
    {}
    {\eval{\hp}{\sbstate}{\bif{\cfalse}{\rexpr_1}{\rexpr_2}}
          {\hp}{\sbstate}{\rexpr_2}}

  \inferrule[\opcall]
    {}
    {\eval{\hp}{\sbstate}{\fcall{(\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr})}{\overline{\typ}}{\overline{\expr}}{\overline{\val}}}
          {\hp}{\sbstate}{\rexpr[\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr}/\ff,\overline{\val}/\overline{\xx}, \overline{\expr}/\overline{\aa}]}}

  \inferrule[\opunpack]
    {}
    {\eval{\hp}{\sbstate}{\bunpack{\xx}{\aa}{\rexpr}}
          {\hp}{\sbstate}{\rexpr}}

    \inferrule[\opass]
    { \transwrite{\sbstate}{\cloc}{\ptrtag}{\sbstate'} }
    {\eval{\hp\hbind{\cloc}{\val}}{\sbstate}{\sassign{\vptr{\cloc}{\ptrtag}}{\val'}}
          {\hp\hbind{\cloc}{\val'}}{\sbstate'}{\poison}}

  \inferrule[\opstrgrebor]
    {\transreborrow{\sbstate}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\mut}}{\sbstate'}}
    {
      \eval{\hp}{\sbstate}{\rvstrgref{\vptr{\cloc}{\ptrtag}}}
           {\hp}{\sbstate'}{\vptr{\cloc}{\ptrtag'}}
    }

  \inferrule[\opmutrebor]
    {\transreborrow{\sbstate}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\mut}}{\sbstate'}}
    {
      \eval{\hp}{\sbstate}{\rvmutref{\vptr{\cloc}{\ptrtag}}}
           {\hp}{\sbstate'}{\vptr{\cloc}{\ptrtag'}}
    }

  \inferrule[\opshrrebor]
    {\transreborrow{\sbstate}{\cloc}{\ptrtag}{\ptrtag'}{\SbRef{\shr}}{\sbstate'}}
    {
      \eval{\hp}{\sbstate}{\rvshrref{\vptr{\cloc}{\ptrtag}}}
           {\hp}{\sbstate'}{\vptr{\cloc}{\ptrtag'}}
    }

  \inferrule[\opderef]
    {
      \transread{\sbstate}{\cloc}{\ptrtag}{\sbstate'}
    }
    {
      \eval{\hp}{\sbstate}{\deref{\vptr{\cloc}{\ptrtag}}}
           {\hp}{\sbstate'}{\hp(\cloc)}
    }
\end{judgment}


\begin{judgment}{Operational Semantics (vectors)}{\eval{\hp}{\sbstate}{\ee}{\hp}{\sbstate}{\rexpr}}
    \inferrule[\opvecnew]
    {}
    {
        \eval
          {\hp}{\sbstate}
          {\fcall{\vecnew}{}{}{}}
          {\hp}{\sbstate}
          {\vvec{0}{\poison}}
    }

    \inferrule[\opvecpush]
    {
        \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate} \\\\
        \transdealloc{\sbstate}{\cloc'}{\ptrtag'}{n}{\sbstate'} \\\\
        \transalloc{\sbstate'}{\cloc''}{\ptrtag''}{n+1}{\sbstate_o} \\\\
        [\cloc'', \cloc'' + n] \mathrel{\#} \dom{\hp} \\\\
        \hp_i = \hp\hbind{\cloc}{\vvec{n}{\vptr{\cloc'}{\ptrtag'}}}\hbindn{n}{\cloc'}{\overline{\val}} \\\\
        \hp_o = \hp\hbind{\cloc}{\vvec{n+1}{\vptr{\cloc''}{\ptrtag''}}}\hbindn{n+1}{\cloc''}{\overline{\val} \append [\val]}
    }
    {
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecpush}{}{\cloc}{\vptr{\cloc}{\ptrtag}, \val}}
          {\hp_o}{\sbstate_o}
          {\poison}
    }

    \inferrule[\opvecpushempty]
    {
        \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate} \\\\
        \transalloc{\sbstate}{\cloc'}{\ptrtag'}{1}{\sbstate_o} \\\\
        \cloc' \notin \dom{\hp} \\\\
        \hp_i = \hp\hbind{\cloc}{\vvec{0}{\val'}} \\\\
        \hp_o = \hp\hbind{\cloc}{\vvec{1}{\vptr{\cloc'}{\ptrtag'}}}\hbind{\cloc'}{\val}
    }
    {
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecpush}{}{\cloc}{\vptr{\cloc}{\ptrtag}, \val}}
          {\hp_o}{\sbstate_o}
          {\poison}
    }

    \inferrule[\opvecindexmut]
    {
        \cloc + i \in \dom{\hp} \\\\
        \transread{\sbstate_i}{\cloc}{\ptrtag}{\sbstate} \\\\
        \transreborrow{\sbstate}{\cloc' + i}{\ptrtag'}{\ptrtag''}{\mut}{\sbstate_o} \\\\
        \hp = \hp'\hbind{\cloc}{\vvec{n}{\vptr{\cloc'}{\ptrtag'}}}
    }
    {
        \eval
          {\hp}{\sbstate_i}
          {\fcall{\vecindexmut}{}{}{\vptr{\cloc}{\ptrtag}, i}}
          {\hp}{\sbstate_o}
          {\vptr{\cloc' + i}{\ptrtag''}}
    }
\end{judgment}


==> metatheory/proofs/preservation.tex <==
\preservation*
\begin{proof}
By induction on the type derivation tree.
\begin{itemize}
  \item \textbf{Rule \tsub:}
    By inversion of the rule:
    (1) \typing{\varcx}{\env}{\loccx_i}{\dynenv_i}{\ee}
    {\typ_1}
    {\loccx'}
    {\dynenv},
    (2) \subtyping{\typ_1}{\typ}, and
    (3) \loccxinc{\varcx}{}{}{\loccx'}{\loccx}.
    By inductive hypothesis on (1):
    then there exist $\loccx_o$ and $\dynenv_o \supseteq \dynenv_i$, such that
    (4) \typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\rexpr_o}{\typ_1}{\loccx}{\dynenv}
    and
    (5) \statetyping[\varcx][\loccx_o][\dynenv_o]{\hp}{\sbstate}.
    The proof concludes by (4), (2), (3), and rule \tsub.

    \item \textbf{Rule \tif:}
    Let $\ee \equiv \bif{\ee_0}{\ee_1}{\ee_2}$.
    By inversion of the rule:

    \begin{enumerate}
      \item \typing{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\ee_0}{\rtyp{\tbool}{\expr}}{\loccx_0}{\dynenv_o}
      \item \typing{\varcx, \expr}{\emptyset}{\loccx_0}{\dynenv_i}{\ee_1}{\typ}{\loccx}{\dynenv}
      \item \typing{\varcx, \lnot \expr}{\emptyset}{\loccx_0}{\dynenv_i}{\ee_2}{\typ_2}{\loccx}{\dynenv}.
    \end{enumerate}
%
    Since \ee steps, there are three cases:
    \begin{itemize}
    \item \textbf{Rule \opprop:}
    $\eval{\hp_i}{\sbstate_i}{\bif{\ee_0}{\ee_1}{\ee_2}}
    {\hp_o}{\sbstate_o}{\bif{\ee'_0}{\ee_1}{\ee_2}}$.
    By inversion:
    $\eval{\hp_i}{\sbstate_i}{\ee_0}
    {\hp_o}{\sbstate_o}{\ee'_0}$.
    By (1) and inductive hypothesis:
    there exists $\loccx_o$ and $\dynenv_o \supseteq \dynenv_i$, so that
    $\typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\rexpr'_0}{\rtyp{\tbool}{\expr}}{\loccx_0}{\dynenv}$
    and
    \statetyping[\varcx][\loccx_o][\dynenv_o]{\hp_o}{\sbstate_o}
    %
    By (2) and (3), weakened to $\dynenv_o$ using Lemma~\ref{lemma:weakening}, and rule \tif:
    $\typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\bif{\ee'_0}{\ee_1}{\ee_2}}{\typ}{\loccx}{\dynenv}$,
    which concludes the proof.
    \item \textbf{Rule \opifTrue: }
    $\eval{\hp}{\sbstate}{\bif{\ctrue}{\rexpr_1}{\rexpr_2}}
    {\hp}{\sbstate}{\rexpr_1}$,
    where $\hp = \hp_i = \hp_o$ and $\sbstate = \sbstate_i = \sbstate_o$.
    Trivial by (2) and with $\loccx_o = \loccx_i$ and $\dynenv_o = \dynenv_i$.
    \item \textbf{Rule \opifFalse: }
    $\eval{\hp}{\sbstate}{\bif{\cfalse}{\rexpr_1}{\rexpr_2}}
    {\hp}{\sbstate}{\rexpr_2}$,
    where $\hp = \hp_i = \hp_o$ and $\sbstate = \sbstate_i = \sbstate_o$.
    Trivial by (3) and with $\loccx_o = \loccx_i$ and $\dynenv_o = \dynenv_i$.
    \end{itemize}
    \item \textbf{Rule \tnew:}
    Let $\ee \equiv \blet{\xx}{\new{\lvar}}{\ee'}$. By inversion of the rule we get:
    $$
    (1)~\typing{\varcx,\lvar: \sloc}
           {\mapstoenv{\xx}{\tptr{\lvar}}}
           {\loccx_i,\mapstoowned{\lvar}{\uninit{1}}}
           {\dynenv_i}
           {\ee'}
           {\typ}{\loccx}
           {}
    $$
    By assumption we have
    $\eval{\hp_i}{\sbstate_i}
          {\blet{\xx}{\new{\lvar}}{\ee'}}
          {\hp_o}{\sbstate_o}{\ee_o}$, thus the rule \opnew{} must have been applied and we know
    $\ee_o \equiv \ee'[\cloc/\lvar][\vptr{\cloc}{\ptrtag}/\xx]$ and
    $\hp_o \equiv \hp_i\hbind{\cloc}{\poison}$.
    By Lemma~\ref{lemma:type-substitution} we get
    $$
    (2)~\typing{\varcx}
           {\mapstoenv{\xx}{\tptr{\cloc}}}
           {\loccx_i[\cloc/\lvar],\mapstoowned{\cloc}{\uninit{1}}}
           {\dynenv_i[\cloc/\lvar]}
           {\ee'[\cloc/\lvar]}
           {\typ[\cloc/\lvar]}{\loccx[\cloc/\lvar]}
           {}
    $$
    We know \wf{\typ} and \wf{\loccx} by inversion of \tnew,
    thereby, we know $\typ=\typ[\cloc/\lvar]$ and $\loccx = \loccx[\cloc/\lvar]$
    by lemmas~\ref{lemma:fv-subst} and \ref{lemma:wf-fv}.
    Then, applying Lemma~\ref{lemma:program-substitution} to (2) we get:
    $$
    (3)~\typing{\varcx}
           {\mapstoenv{\xx}{\tptr{\cloc}}}
           {\loccx_i[\cloc/\lvar],\mapstoowned{\cloc}{\uninit{1}}}
           {\dynenv_i[\cloc/\lvar],\mapstoowned{(\cloc, \ptrtag)}{\tptr{\cloc}}}
           {\ee'[\cloc/\lvar][\vptr{\cloc}{\ptrtag}/\xx]}
           {\typ}{\loccx}
           {}
    $$
    Picking $T_o=T_i[\cloc/\lvar]$ and $\dynenv_o=\dynenv_i,\mapstoowned{(\cloc, \ptrtag)}{\tptr{\cloc}}$ we
    get the first part of the conclusion.
    It remains to show $\statetyping[\varcx][\loccx_o][\dynenv_o]{\hp_o}{\sbstate_o}$ which is a direct application
    of Lemma~\ref{lemma:event:alloc}.

    % \item \textbf{Rule \tseq:}
    % Let $\ee \equiv \bseq{\stmt}{\rexpr'}$.
    % By inversion of the rule we get:
    % (1) \stmtyping{\varcx}{\env}{\loccx_i}{\dynenv_i}{\stmt}{\loccx_{\stmt}}{\dynenv}
    % and
    % (2) \typing{\varcx}{\env}{\loccx_{\stmt}}{\dynenv_i}{\rexpr'}{\typ}{\loccx}{\dynenv}.
    % %
    % By assumption we have $\eval{\hp_i}{\sbstate_i}{\bseq{\stmt}{\ee'}}
    % {\hp_o}{\sbstate_o}{\rexpr_o}$.
    % There are two cases:
    % \begin{itemize}
    %   \item \textbf{Rule \opskip} We have $\ee_o=\ee'$. We know the rule \tskip does not update
    %   the location context, thus $\loccx_s=\loccx_i$. We can satisfy the requirements in the conclusion
    %   by picking $\loccx_o=\loccx_i$ and $\dynenv_o=\dynenv_i$.
    %   \item \textbf{Rule \opseq:} We have (3) $\ee_o= \ee'$.
    % By inversion of \opseq, we have (4) \eval{\hp_i}{\sbstate_i}{\stmt}{\hp_o}{\sbstate_o}{\stmt_o}.
    % %
    % By assumption we also have (5) \statetyping[\varcx][\loccx_i][\dynenv]{\hp_i}{\sbstate_i}.
    % By (1), (4), (5), and Lemma~\ref{theorem:preservation:statement} we have (6)
    % \statetyping[\varcx][\loccx_{\stmt}][\dynenv']{\hp_o}{\sbstate_o} for some $\dynenv'\supseteq \dynenv_i$.
    % By weakening (Lemma~\ref{lemma:weakening}) and (2) we know
    % $$
    % \typing{\varcx}{\env}{\loccx_{\stmt}}{\dynenv'}{\rexpr'}{\typ}{\loccx}{\dynenv}.
    % $$
    % Thus, it suffices to pick $\loccx_o=\loccx_S$ and $\dynenv_o=\dynenv'$ to satisfy the conclusion.
    % \end{itemize}

  \item \textbf{Rule \tlet:}
  Let $\ee \equiv \blet{\xx}{\ee_{\xx}}{\ee'}$. By inversion of the rule we get:
  (1) \typing{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\ee_{\xx}}{\typ_{\xx}}{\loccx_0}{\dynenv} and
  (2) \typing{\varcx}{\mapstoenv{\xx}{\typ_\xx}}{\loccx_0}{\dynenv_i}{\ee}{\typ}{\loccx}{\dynenv_o}.
%
Since \ee steps, there are two cases:

\begin{itemize}

    \item \textbf{Rule \oplet:}
    {\eval{\hp_i}{\sbstate_i}{\blet{\xx}{\val}{\rexpr'}}
    {\hp_i}{\sbstate_i}{\rexpr'[\val/\xx]}}.
    Since $\ee_{\xx} = \val$, by (1), (2), and Lemma~\ref{lemma:program-substitution-2}:
  %
    \typing{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\rexpr'[\val/\xx]}{\typ}{\loccx}{\dynenv}
    which concludes the proof.
    \item \textbf{Rule \opprop:}
    {\eval{\hp_i}{\sbstate_i}{\blet{\xx}{\ee_x}{\rexpr'}}
    {\hp_o}{\sbstate_o}{\blet{\xx}{\ee'_x}{\rexpr'}}}.
    By inversion:
    {\eval{\hp_i}{\sbstate_i}{\ee_x}
    {\hp_o}{\sbstate_o}{\ee'_x}}.
    By (1) and inductive hypothesis:
    there exists $\loccx_o$ and $\dynenv_o \supseteq \dynenv_i$, so that
    $\typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\rexpr'_x}{\typ_x}{\loccx_0}{\dynenv}$
    and
    \statetyping[\varcx][\loccx_o][\dynenv_o]{\hp_o}{\sbstate_o}.
    %
    By (2), weakened to $\dynenv_o$ using Lemma~\ref{lemma:weakening}, and rule \tlet:
    $\typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\blet{\xx}{\ee'_{\xx}}{\ee'}}{\typ}{\loccx}{\dynenv}$,
    which concludes the proof.

  \end{itemize}


  \item \textbf{Rule \tcall:}
  Let $\ee \equiv \fcall{\ee'}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}$. By inversion of the rule we get:
  (0) \wf{\dynenv}
  (1) $\forall i. \typing{\varcx}{\emptyset}{\loccx}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx}{}$,
  (2) \typing{\varcx}{\emptyset}{\loccx}{\dynenv}{\ee'}
         {\polysig{\overline{\tvar}}
                  {\overline{\aa: \sort}}
                  {\expr}
                  {\loccx_{i}}
                  {\overline{\typ}}
                  {\typ_o}
                  {\loccx_{o}}}
        {\loccx_1 * \loccx_2 }{\dynenv},
  (3) $ \substvar = \subst{\overline{\aa}}{\overline{\expr}}$,
  (4) \loccxinc{\varcx}{}{}{\loccx_1}{\applysubst{\substvar}{\loccx_{i}}},
  (5) $\forall i.\sortck{\expr_i}{\sort_i}$, and
  (6) \lmodel{\varcx}{\applysubst{\substvar}{\expr}}.

  %
  Since \ee steps, we have the following cases:
  \begin{itemize}
    \item \textbf{Rule \opprop}:
      \eval{\hp_i}{\sbstate_i}{\fcall{\ee'}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
          {\hp_o}{\sbstate_o}{\fcall{\ee'_o}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}.
      By inversion of the rule
      \eval{\hp_i}{\sbstate_i}{\ee'}
          {\hp_o}{\sbstate_o}{\ee'_o}.
      By this, (2), and inductive hypothesis
      there exist $\loccx'_o$ and $\dynenv_o \supseteq \dynenv$, so that
      (7) $
          \typing{\varcx}{\emptyset}{\loccx'_o}{\dynenv_o}{\rexpr'_o}{\polysig{\overline{\tvar}}
          {\overline{\aa: \sort}}
          {\expr}
          {\loccx_{i}}
          {\overline{\typ}}
          {\typ_o}
          {\loccx_{o}}}
      {\loccx_1 * \loccx_2 }{\dynenv}
          $ and
      (8) \statetyping[\varcx][\loccx'_o][\dynenv_o]{\hp_o}{\sbstate_o}.
      By Lemmas~\ref{lemma:aval},~\ref{lemma:weakening}, and (1):
      %
      (9) $\forall i. \typing{\varcx}{\emptyset}{\loccx'_o}{\dynenv_o}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx'_o}{}$,
      %
      By rule \tcall on (9), (7), (3), (4), (5), (6), and (0):
      \typing{\varcx}{\emptyset}{\loccx'_o}{\dynenv_o}
                    {\fcall{\ee'}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
                    {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}} * \loccx_2}{}.
      Which, combined with (7), concludes the proof.

    \item \textbf{Rule \opcall:}
      $$
      \eval{\hp}{\sbstate}{\fcall{(\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr_\ff})}{\overline{\typ}}{\overline{\expr}}{\overline{\val}}}
                {\hp}{\sbstate}{\rexpr_\ff[\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr_\ff}/\ff,\overline{\val}/\overline{\xx},\overline{\aa}/\overline{\expr}]}
      $$

      %
      Since $\ee' \equiv \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr_\ff}$, by inversion of (2), we get:
      $$(7)\quad
      \typing{\varcx,\overline{\aa: \sort},\expr}
                    {\overline{\xx : \typ},
                      \ff: \polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                                  {{\expr}}{\loccx_{i}}
                                  {\overline{\typ}}
                                  {{\typ}}
                                  {\loccx_{o}}
                      }
                    {\loccx_i}{\dynenv}
                    {\rexpr_\ff}
                    {\typ_o}{\loccx_o}
                    {}$$
      %
      By Lemma~\ref{lemma:type-substitution} and (5):
      $$(8)\quad
      \typing{\varcx,\applysubst{\substvar}{\expr}}
                    {\overline{\xx : \applysubst{\substvar}{\typ}},
                      \ff: \applysubst{\substvar}{\polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                                  {{\expr}}{\loccx_{i}}
                                  {\overline{\typ}}
                                  {{\typ}}
                                  {\loccx_{o}}}
                      }
                    {\applysubst{\substvar}{\loccx_i}}{\applysubst{\substvar}{\dynenv}}
                    {\applysubst{\substvar}{\rexpr_\ff}}
                    {\applysubst{\substvar}{\typ_o}}
                    {\applysubst{\substvar}{\loccx_o}}
                    {}$$
      %
      The \substvar application is an identity in the type of the function (that is forall-quantified),
      and in $\dynenv$ (by (0) and lemma~\ref{lemma:wf-fv}).
      Further, by (6) and Lemma~\ref{lemma:condition} we remove logical condition $\applysubst{\substvar}{\expr}$:
      $$(9)\quad
      \typing{\varcx}
                    {\overline{\xx : \applysubst{\substvar}{\typ}},
                      \ff: {\polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                                  {{\expr}}{\loccx_{i}}
                                  {\overline{\typ}}
                                  {{\typ}}
                                  {\loccx_{o}}}
                      }
                    {\applysubst{\substvar}{\loccx_i}}
                    {{\dynenv}}
                    {\applysubst{\substvar}{\rexpr_\ff}}
                    {\applysubst{\substvar}{\typ_o}}
                    {\applysubst{\substvar}{\loccx_o}}
                    {}$$
      %
      By (1), (2), and Lemmata~\ref{lemma:program-substitution} and~\ref{lemma:aval}:
      $$(10)\quad
      \typing{\varcx}{\emptyset}
                    {\applysubst{\substvar}{\loccx_i}}
                    {{\dynenv}}
                    {\rexpr_\ff[\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr_\ff}/\ff,\overline{\val}/\overline{\xx},\overline{\aa}/\overline{\expr}]}
                    {\applysubst{\substvar}{\typ_o}}
                    {\applysubst{\substvar}{\loccx_o}}
                    {}$$
      %
      By (4) and Lemma~\ref{lemma:conctext-inclusion}
      $$(11)\quad
      \typing{\varcx}{\emptyset}
                    {\loccx_1}
                    {{\dynenv}}
                    {\rexpr_\ff[\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr_\ff}/\ff,\overline{\val}/\overline{\xx},\overline{\expr}/\overline{\aa}]}
                    {\applysubst{\substvar}{\typ_o}}
                    {\applysubst{\substvar}{\loccx_o}}
                    {}$$
      %

      Finally, by Lemma~\ref{lemma:framing}
      $$(12)\quad
      \typing{\varcx}{\emptyset}
                    {\loccx_1 * \loccx_2}
                    {{\dynenv}}
                    {\rexpr_\ff[\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{\rexpr_\ff}/\ff,\overline{\val}/\overline{\xx},\overline{\expr}/\overline{\aa}]}
                    {\applysubst{\substvar}{\typ_o}}
                    {\applysubst{\substvar}{\loccx_o}* \loccx_2}
                    {}$$
      %
      Which concludes the proof, because $\ee'$ is a value,
      thus $\loccx_1 * \loccx_2 = \loccx$ and by assumption
      \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate}.

       \item \textbf{Rule \opvecnew:}
        We have
        $$
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecnew[\typ_v]}{}{}{}}
          {\hp_i}{\sbstate_i}
          {\vvec{0}{\poison}}
        $$
        Because the output state does not change we know it is still well-typed.
        By inversion of (2) we know $\subtyping{\rtyp{\tvec[\typ_v]}{0}}{\typ_o}$.
        We conclude by applying \tvecvec and \tsub to prove the result is also well-typed.

        \item \textbf{Rule \opvecpush:}
        We have
        $$
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecpush[\typ_v]}{}{\cloc}{\vptr{\cloc}{\ptrtag}, \val}}
          {\hp_o}{\sbstate_o}
          {\poison}
        $$

        By inversion of (1) we get $\dynenv_i(\cloc, \ptrtag) = \tptr{\cloc}$ and
        \typing{\varcx}{\emptyset}{\loccx}{\dynenv_i}{\val}{\typ_v}{\loccx}{}.
        Then, by Lemma~\ref{lemma:vec:push} we get
        \statetyping[\varcx][(\cloc \mapsto \rtyp{\tvec[\typ_v]}{n + 1}), \loccx_2][\dynenv_o]{\hp_o}{\sbstate_o}.
        Finally, by inversion of (2) we get \subtyping{\uninit{1}}{\typ_o} and consequently
        by applying \tumem and \tsub the result is well-typed.

        \item \textbf{Rule \opvecpushempty:}
        We have
        $$
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecpush[\typ_v]}{}{\cloc}{\vptr{\cloc}{\ptrtag}, \val}}
          {\hp_o}{\sbstate_o}
          {\poison}
        $$
        and by inversion of the rule we also have $\hp(\cloc) = \vptr{0}{\val'}$.
        By inversion of (1) we also have
        \typing{\varcx}{\emptyset}{\loccx}{\dynenv_i}{\val}{\typ_v}{\loccx}{},
        $\dynenv_i(\cloc, \ptrtag) = \tptr{\cloc}$ and
        \subtyping{\uninit{1}}{\typ_o}.
        We pick $\dynenv_o = \dynenv_i, (\cloc', \ptrtag')\mapsto \tref{\mut}{\typ_v}$.
        By Lemma~\ref{lemma:vec:push-empty} we get
        \statetyping[\varcx][\cloc\mapsto \rtyp{\tvec[\typ_v]}{1}, \loccx_2][\dynenv_o]{\hp_o}{\sbstate_o}.
        We conclude by applying \tumem and \tsub to prove the result is well-typed.

        \item \textbf{Rule \opvecindexmut:}
        We have
        $$
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecindexmut[\typ_v]}{}{}{\vptr{\cloc}{\ptrtag}, i}}
          {\hp_i}{\sbstate_o}
          {\vptr{\cloc' + i}{\ptrtag''}}
        $$
        By inversion of (1) we have $\dynenv_i(\cloc, \ptrtag) = \tref{\mut}{\rtyp{\tvec[\typ_v]}{n}}$.
        Therefore, by well-typedness of the input state and Lemma~\ref{lemma:event:read} we have
        (6) \typing{\varcx}{\emptyset}{\emptyset}{\dynenv}{\hp(\cloc)}{\rtyp{\tvec[\typ_v]}{n}}{\emptyset}{}.
        Then, by lemmas~\ref{lemma:canonical:vec} and \ref{lemma:value-refinement} we have $\hp(\cloc)=\vvec{n}{\val}$.
        There are two cases:
        \begin{itemize}
            \item $n=0$. This case is impossible because by (6) $\entailment{\varcx}{0\leq i < 0}$ would need to hold
            which is impossible.
            \item $n > 0$.
            By inversion of \tvecvec we have $\val=\vptr{\cloc'}{\ptrtag'}$.
            We conclude by picking $\dynenv_o=\dynenv,(\cloc', \ptrtag')\mapsto \tref{\mut}{\typ_v}$ and
            applying Lemma~\ref{lemma:vec:indexmut}.
        \end{itemize}
    \end{itemize}

      \item \textbf{Rule \ttvar:} Impossible because the typing environment \env is empty.
    \item \textbf{Rule \tunpack:} Impossible because the typing environment \env is empty.
    \item \textbf{Rules \ttrue, \tfalse, \tconstint, \tfun, \ttptr, \tumem:}
          These cases are trivial, since the expressions do not step.

    % \item \textbf{Case \tskip:} Impossible because \sskip cannot take a step.

    \item \textbf{Case \tassign:} Let $\ee=\sassign{\place}{\ee_0}$.
    Since $\ee$ steps we have two options
    By inversion of the rule we have
    \begin{enumerate}
      \item \rvaltyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\ee_0}{\typ_v}{\loccx},
      \item \pltyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\place}{\tref{\mut}{\typ}}{\loccx_i}
      \item \subtyping{\typ_v}{\typ}.
    \end{enumerate}
    Since $\ee$ takes a step there are two options:
    \begin{itemize}
        \item \textbf{Case \opprop:}
        By inversion of the rule we have \eval{\hp_i}{\sbstate_i}{\ee_0}{\hp_o}{\sbstate_o}{\ee_1}
        and $\ee_o=\sassign{\place}{\ee_2}$.
        By inductive hypothesis on (1) there exists $\dynenv_o$ and $\loccx_o$ such that
        \begin{enumerate}
          \item \valtyping{\varcx}{\emptyset}{\loccx_o}{\dynenv'}{\ee_1}{\typ_v}
          \item \statetyping[\varcx][\loccx_o][\dynenv']{\hp_o}{\sbstate_o}
        \end{enumerate}
        We conclude by applying \tassign to prove
        \typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\sassign{\place}{\ee_o}}{\uninit{1}}{\loccx}{}.

        \item \textbf{Case \opass:} Let $\ee=\sassign{\vptr{\cloc}{\ptrtag}}{\val}$,
        $\ee_o=\poison$ and $\hp_o=\hp_i\hbind{\cloc}{\val}$.
        Replacing $\vptr{\cloc}{\ptrtag}$ for $\place$ in (2) we also get
        $\dynenv(\cloc,\ptrtag)=\tref{\mut}{\typ}$.
        By using (1), (3) and subsumption we get
        \valtyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\val}{\typ}.
        Let us pick $\loccx_o=\loccx$ and $\dynenv_o=\dynenv_i$.
        We get the first part of the conclusion by applying \tumem.
        We conclude by applying Lemma~\ref{lemma:event:weak-write}.
    \end{itemize}
    \item \textbf{Case \tassignstrg:} Let $\ee=\sassign{\place}{\ee_0}$.
    By inversion of the rule we have
    \begin{enumerate}
      \item \rvaltyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\ee_0}{\typ}{\loccx'} and
      \item $\loccx=\loccx'[\cloc\mapsto\typ]$.
    \end{enumerate}
    Since $\ee$ takes a step there are two options:
    \begin{itemize}
        \item \textbf{Case \opprop:} The proof is similar to the \opprop case
        for the \tassign case by applying the inductive hypothesis.

        \item \textbf{Case \opass:} Let $\ee=\sassign{\vptr{\cloc}{\ptrtag}}{\val}$,
        $\ee_o=\poison$ and $\hp_o=\hp_i\hbind{\cloc}{\val}$.
        Replacing $\vptr{\cloc}{\ptrtag}$ for $\place$ in (2) we also get
        $\dynenv(\cloc,\ptrtag)=\tptr{\cloc}$.
        Let us pick $\loccx_o=\loccx'$ and $\dynenv_o=\dynenv_i$.
        We conclude by applying Lemma~\ref{lemma:event:strg-write}
    \end{itemize}

    \item \textbf{Case \tstrgrebor:} Let $\ee=\rvstrgref{\place}$ and $T_o = T_i$.
    Since $\ee$ takes a step then the \opstrgrebor{} must have been applied and thus we know
    $\place = \vptr{\cloc}{\ptrtag}$ and $\ee_o=\vptr{\cloc}{\ptrtag'}$.
    By inversion of the typing rule we know that
    \pltyping{\varcx}{\emptyset}{\loccx_o}{\dynenv_i}{\vptr{\cloc}{\ptrtag}}{\tptr{\cloc}}{\loccx_o}
    and consequently $\dynenv_i(\cloc,\ptrtag)=\tptr{\cloc}$.
    Picking $\dynenv_o=\dynenv_i,\mapstoowned{(\cloc,\ptrtag')}{\tptr{\cloc}}$ we directly
    \pltyping{\varcx}{\emptyset}{\loccx_o}{\dynenv_i}{\vptr{\cloc}{\ptrtag'}}{\tptr{\cloc}}{\loccx_o}.
    We conclude by Lemma~\ref{lemma:event:strg-rebor} to prove the output state is well-typed.

    \item \textbf{Case \tstrgmutrebor:} Since $\ee$ takes a step then \opmutrebor{} must have been
    applied and we know $\ee=\rvmutref{\vptr{\cloc}{\ptrtag}}$ and $\ee_o=\vptr{\cloc}{\ptrtag'}$.
    We also know $\loccx_o=\loccx_i[\cloc\mapsto\typ]$.
    By inversion of the typing rule we have that
    (1) \pltyping{\varcx}{\emptyset}{\loccx_o}{\dynenv_i}{\vptr{\cloc}{\ptrtag}}{\tptr{\cloc}}{\loccx_o}
    and \subtyping{\loccx_i(\cloc)}{\typ}.
    By (1) we also know $\dynenv_i(\cloc, \ptrtag) = \tptr{\cloc}$.
    If we pick $\dynenv_o=\dynenv_i,\mapstoowned{(\cloc, \ptrtag')}{\tref{\mut}{\typ}}$
    we get directly
    \pltyping{\varcx}{\emptyset}{\loccx_o}{\dynenv_i}{\vptr{\cloc}{\ptrtag'}}{\tref{\mut}{\typ}}{\loccx_o}.
    We conclude by applying Lemma~\ref{lemma:event:weaken-rebor} to prove the output state is well-typed.

    \item \textbf{Case \tmutmutrebor:} Since $\ee$ takes a step then \opmutrebor{} must have been applied,
    thus we know $\ee=\rvmutref{\vptr{\cloc}{\ptrtag}}$ and $\ee_o=\vptr{\cloc}{\ptrtag'}$.
    We also know $T=T_i$.
    By inversion of the typing rule we know that
    \pltyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\vptr{\cloc}{\ptrtag}}{\tref{\mut}{\typ}}{\loccx_i}
    and consequently $\dynenv_i(\cloc, \ptrtag)=\tref{\mut}{\typ}$.
    By definition of \statetyping[\varcx][\loccx_i][\dynenv_i]{\hp_i}{\sbstate_i} we know
    \subtyping{\typ}{\loccx_i(\cloc)}{\typ} and \valtyping{\varcx}{\emptyset}{\emptyset}{\dynenv_i}{\hp(\cloc)}{\typ}.
    We conclude picking $\dynenv_o=\dynenv_i,\mapstoowned{(\cloc, \ptrtag')}{\tref{\mut}{\typ}}$ and applying
    Lemma~\ref{lemma:event:mut-rebor}.

    \item \textbf{Case \tshrrebor:}
    Since \ee takes a step then \opshrrebor must have been applied.
    Therefore, $\ee=\rvshrref{\vptr{\cloc}{\ptrtag}}$ and $\ee_o=\vptr{\cloc}{\ptrtag'}$.
    We also know $\loccx=\loccx_i$ and by inversion of the typing rule we have
    (1) \pltyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\vptr{\cloc}{\ptrtag}}{\tref{\bormode}{\typ'}}{\loccx_i} and (2)
    \subtyping{\typ'}{\typ}.
    By (1) we also have $\dynenv_i(\cloc, \ptrtag)=\tref{\bormode}{\typ'}$.
    Since the input stack is well-typed we know \subtyping{\loccx_i(\cloc)}{\typ'} and
    and transitivity of subtyping we have \subtyping{\loccx_i(\cloc)}{\typ}.
    We pick $\dynenv_o=\dynenv_i(\cloc,\ptrtag')\mapsto \tref{\shr}{\typ}$ and conclude
    applying Lemma~\ref{lemma:event:shr-rebor}.

    \item \textbf{Case \tderef:} Since $\ee$ takes a step then \opderef must have been applied,
    therefore $\ee=\deref{\vptr{\cloc}{\ptrtag}}$ and $\ee_o=\hp(\cloc)$.
    By inversion of the typing rule we know
    $\pltyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\vptr{\cloc}{\ptrtag}}{\tref{\bormode}{\typ}}{\loccx_i}$
    and consequently $\dynenv_i(\cloc, \ptrtag)=\tref{\bormode}{\typ}$.
    We pick $\dynenv_o=\dynenv_i$ and conclude by applying Lemma~\ref{lemma:event:read} to pove
    the output state is well-typed.

    \item \textbf{Case \tderefstrg:}
    Since $\ee$ takes a step then \opderef must have been applied, therefore
    $\ee=\deref{\vptr{\cloc}{\ptrtag}}$ and $\ee_o=\hp(\cloc)$.
    By inversion of the typing rule we know
    $\pltyping{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\vptr{\cloc}{\ptrtag}}{\tptr{\cloc}}{\loccx_i}$
    and $\loccx(\cloc)=\typ$.
    Consequently, we know $\dynenv_i(\cloc,\ptrtag)=\tptr{\cloc}$.
    We pick $\dynenv_o=\dynenv_i$ and conclude by applying Lemma~\ref{lemma:event:strg-read}.
\end{itemize}
\end{proof}





==> metatheory/proofs/progress.tex <==
\progress*
\begin{proof}
By induction on the type derivation tree \typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\rexpr}{\typ}{\loccx_o}{\dynenv_o}.
\begin{itemize}
    \item \textbf{Rule \tsub:}
    By inversion of the rule we get
    \typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\rexpr}{\typ_1}{\loccx_o}{\dynenv_o}
    at which we apply the inductive hypothesis.

    \item \textbf{Rule \tlet:}
    Let $\ee \equiv  \blet{\xx}{\ee_\xx}{\ee'}$.
    By inversion of the rule,
    \typing{\emptyset}{\env}{\loccx_i}{\dynenv_i}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv}.
    By inductive hypothesis, there are three cases:
    (1) If $\ee_{\xx}$ is a value, the \oplet rule applies with $\hp_i$ and  $\sbstate_i$;
    (2) If $\evalerr{\hp_i}{\sbstate_i}{\rexpr_\xx}$, then, by rule \opproperr,
    $\evalerr{\hp_i}{\sbstate_i}{\rexpr}$; and
    (3) If $\eval{\hp_i}{\sbstate_i}{\rexpr_\xx}{\hp_o}{\sbstate_o}{\ee'_\xx}$,
    then, by rule \opprop,
    $\eval{\hp_i}{\sbstate_i}{\blet{\xx}{\ee_\xx}{\ee'}}{\hp_o}{\sbstate_o}{\blet{\xx}{\ee'_\xx}{\ee'}}$.
    \item \textbf{Rule \tnew:}
    Let $\ee \equiv \blet{\xx}{\new{\lvar}}{\rexpr'}$.
    One of the rules \opnew or \opnewerr applies.
    \item \textbf{Rule \tif:}
    Let $\ee \equiv  \bif{\ee'}{\ee_1}{\ee_2}$.
    By inversion of the rule,
    \typing{\emptyset}{\env}{\loccx_i}{\dynenv_i}{\ee'}{\rtyp{\tbool}{\expr}}{\loccx_o}{\dynenv_o}.
    By inductive hypothesis, there are three cases:
    (1) If $\ee'$ is a value, then, by Lemma~\ref{lemma:canonical:bool},
    it is either \ctrue or \cfalse and one of the  \opifTrue or \opifFalse rules applies with $\hp_i$ and  $\sbstate_i$;
    (2) If $\evalerr{\hp_i}{\sbstate_i}{\rexpr'}$, then, by rule \opproperr,
    $\evalerr{\hp_i}{\sbstate_i}{\rexpr}$; and
    (3) If $\eval{\hp_i}{\sbstate_i}{\rexpr'}{\hp_o}{\sbstate_o}{\ee''}$,
    then, by rule \opprop,
    $\eval{\hp_i}{\sbstate_i}{\ee}{\hp_o}{\sbstate_o}{\bif{\ee''}{\ee_1}{\ee_2}}$.
    \item \textbf{Rule \tseq:}
    Let $\ee \equiv \bseq{\stmt}{\rexpr'}$.
    By inversion of the rule we get:
    \stmtyping{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\stmt}{\loccx_{\stmt}}{\dynenv_{\stmt}}.
    By assumption we have \statetyping[\emptyset][\loccx_i][\dynenv_i]{\hp_i}{\sbstate_i}.
    By Lemma~\ref{lemma:progress-stmt}, we have that
    either (1)
there exists $\hp_o, \sbstate_o$ such that \evalstm{\hp_i}{\sbstate_i}{\stmt}{\hp_o}{\sbstate_o},
(2) \evalstmerr{\hp_i}{\sbstate_i}{\stmt} or (3) $\stmt_i=\sskip$.
In case (1) and by rule \opseq,
there exists $\hp_o, \sbstate_o$ such that
\eval{\hp_i}{\sbstate_i}{\bseq{\stmt}{\rexpr'}}
          {\hp_o}{\sbstate_o}{\rexpr'}.
In case (2) and by rule \opseqerr,
\evalerr{\hp_i}{\sbstate_i}{\bseq{\stmt}{\rexpr'}}.
Finally, in case (3) \opskip applies.

    \item \textbf{Rule \tcall:}
    Let $\ee \equiv \fcall{\ee'}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}$.
    By inversion of the rule,
    \typing{\emptyset}{\env}{\loccx_i}{\dynenv_i}{\ee'}{\polysig{\overline{\tvar}}{\overline{\aa: \sort}}
    {\expr}
    {\elftcx}{\overline{\xx : \typ}}{\overline{\loc}}{\loccx_{fi}}
    {\typ}{\loccx_{fo}}}{\loccx}{\dynenv}.
    By inductive hypothesis, there are three cases:
    (1) If $\evalerr{\hp_i}{\sbstate_i}{\rexpr'}$, then, by rule \opproperr,
    $\evalerr{\hp_i}{\sbstate_i}{\rexpr}$; and
    (2) If $\eval{\hp_i}{\sbstate_i}{\rexpr'}{\hp_o}{\sbstate_o}{\ee''}$,
    then, by rule \opprop,
    $\eval{\hp_i}{\sbstate_i}{\ee}{\hp_o}{\sbstate_o}{\fcall{\ee''}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}$.
    (3) If $\ee'$ is a value, then, by Lemma~\ref{lemma:canonical:fun} we have the following cases
    \begin{itemize}
        \item $e' = \vrec{f}{\overline{\expr'}}{\overline{\yy}}{\expr_b}$.
        Arguments are a-values and by inversion of typing under the empty environment,
        they must be values, thus rule \opcall applies.
        \item $e' = \vecnew[\typ_v]$. In this case \opvecnew applies.
        \item $e' = \vecpush[\typ_v]$. Let $\val_1$ and $\val_2$ be the two arguments of the function call.
        By inversion of \tcall we have:
        \begin{enumerate}
            \item \typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\val_1}{\tptr{\cloc}}{\loccx_i}{}
            \item \typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\val_2}{\typ_v}{\loccx_i}{}
            \item \loccxinc{\emptyset}{}{}{\loccx_1}{\cloc \mapsto \rtyp{\tvec[\typ_v]}{n}}.
        \end{enumerate}
        By lemmas \ref{lemma:canonical:ptr} and \ref{lemma:canonical:int} we know $\val_1 = \vptr{\cloc}{\ptrtag}$.
        Since the input state is well-typedness we have by (3) that $\cloc \in \dom{\hp}$ and
        \typing{\emptyset}{\emptyset}{\emptyset}{\dynenv_i}{\hp(\cloc)}{\rtyp{\tvec[\typ_v]}{n}}{\emptyset}{}.
        By lemmas~\ref{lemma:canonical:vec} and \ref{lemma:value-refinement} we know $\hp(\cloc) = \vptr{n}{\val'}$.
        If $n=0$ then \opvecpushempty applies.
        If $n > 0$ then $\val' = \vptr{\cloc'}{\ptrtag'}$ and $\forall j \in [0, n). \cloc' + j \in \dom{\hp}$
        and \opvecpush applies.
        \item $e' = \vecindexmut[\typ_v]$. Let $\val_1$ and $\val_2$ be the two arguments of the function call.
        By inversion of \tcall we have:
        \begin{enumerate}
            \item \typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\val_1}{\tref{\mut}{\rtyp{\tvec[\typ_v]}{n}}}{\loccx_i}{}
            \item \typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\val_2}{\rtyp{\tint}{m}}{\loccx_i}{}
            \item \entailment{\emptyset}{0 \leq m < n}
        \end{enumerate}
        By lemmas \ref{lemma:canonical:ptr} and \ref{lemma:canonical:int} we have
        $\val_1 = \vptr{\cloc}{\ptrtag}$ and $\val_2 = z$.
        By Lemma~\ref{lemma:value-refinement} and (2) we have $z = m$, and by (3) we have (4) $0\leq z < n$.
        By well-formedness of the input state and (1) we have
        \typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\hp(\cloc)}{\rtyp{\tvec[\typ_v]}{n}}{\loccx_i}{}
        and by lemmas~\ref{lemma:canonical:vec} and \ref{lemma:value-refinement} we have $\hp(\cloc) = \vvec{n}{\val'}$.
        The case $n=0$ is impossible because (4) must hold.
        Since $n>0$, by inversion of \tvecvec we have $\val'= \vptr{\cloc'}{\ptrtag'}$ and $\cloc' + i \in \dom{\dynenv_i}$
        for all $0 \leq i < n$.
        By well-typeness of the input state we have $\dom{\dynenv_i} = \dom{\hp}$ and consequently $\cloc' + z \in \dom{\hp}$.
        Therefore, the rule \opvecindexmut applies, and we conclude the proof.
    \end{itemize}


    \item \textbf{Rule \ttvar:} Impossible because the typing environment \env is empty.

    \item \textbf{Rule \tunpack:} Impossible because the typing environment \env is empty.

    \item \textbf{Rules \ttrue, \tfalse, \tconstint, \tfun, \ttptr, and \tumem:} \ee is a value.

    \item \textbf{Case \tassign,\tassignstrg:} We have $\ee=\sassign{\place}{\ee'}$.
    Since the statement must be close since we are in an empty environment we have $\place=\vptr{\cloc}{\ptrtag}$.
    If $\ee'=\val$ then either stacked borrow transition in the premise of \opass holds and we take a step, or
    it does not hold and we step to an error by rule \opproperr.
    If $\ee'$ is not a value then by inductive hypothesis either takes a step or goes to an error
    in either case we make progress by rule \opassrval{} or \opasserr.

    \item \textbf{Case \tstrgrebor:} $\ee=\rvstrgref{\place}$. We know $p$ must be equal to $\vptr{\cloc}{\ptrtag}$
    because we are in an empty environment, thus either \opstrgrebor applies or we step to an error
    if the stacked borrow transition does not hold.

    \item \textbf{Case \tstrgmutrebor,\tmutmutrebor:} $\ee=\rvmutref{\place}$.
    We know $p$ must be equal to $\vptr{\cloc}{\ptrtag}$ because we are in an empty environment,
    thus either \opmutrebor applies or we step to an error if the stacked borrow transition does not hold.

    \item \textbf{Case \tshrrebor:} $\ee=\rvshrref{\place}$. We know $p$ must be equal to
    $\vptr{\cloc}{\ptrtag}$ because we are in an empty environment,
    thus either \opshrrebor applies or we step to an error if the stacked borrow transition does not hold.

    \item \textbf{Case \tderef,\tderefstrg:} $\ee=\deref{\place}$. We know $p$ must be equal to
    $\vptr{\cloc}{\ptrtag}$ because we are in an empty environment.
    If the stacked borrow transition in the premise of \opderef holds then \cloc must be in $\dom{\sbstate\dotstacks}$.
    Then, by well-typedness of the input state we have that $\cloc \in \dom{\hp}$ and the rule \opderef applies.
    If the stacked borrow transition does not hold then we step to an error.
    \end{itemize}
\end{proof}



==> metatheory/proofs/rvalue-preservation.tex <==



==> metatheory/proofs/soundness.tex <==
\soundness*
\begin{proof}
By induction on the length of the evaluation path.
For path of length 0, the theorem is a direct implication of Progress (Theorem~\ref{theorem:progress}).
For path of length $n+1$:
$\goesto
      {\hp_i}{\sbstate_i}{\rexpr_i}
      {\hp_n}{\sbstate_n}{\rexpr_n} \rightsquigarrow
      \langle \hp,\sbstate, \rexpr \rangle
$.
By the induction hypothesis and determinism of our operational semantics,
there exists $\loccx_o$ and $\dynenv_o \supseteq \dynenv_i$ such that
     $\statetyping[\varcx][\loccx_o][\dynenv_o]{\hp_o}{\sbstate_o}$ and
    \typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\rexpr}{\typ}{\loccx}{\_}.
    The proof concludes by
    applying progress (Theorem~\ref{theorem:progress}) and then
    preservation (Theorem~\ref{theorem:preservation}).
\end{proof}


==> metatheory/runtime-typing.tex <==
\subsection{Well-typed States}
Intuitively, a state is well-typed if the following conditions
hold:
(1) for each location \cloc the stack $\sbstate\dotstacks(\cloc)$
must be split into a section composed of only unique permissions
followed by a section composed of only shared permissions,
(2) pointers \vptr{\cloc}{\ptrtag} in the shared section
must be associated to shared references in \dynenv
(\ie $\dynenv(\cloc,\ptrtag) = \tref{\shr}{\typ}$),
(3) the unique section must further be split
into a section associated to strong pointers
($\dynenv(\cloc,\ptrtag) = \tptr{\cloc}$) and a section
associated with mutable references
($\dynenv(\cloc, \ptrtag) = \tref{\mut}{\typ}$),
and (4) for every pointer \vptr{\cloc}{\ptrtag} it must
be safe to read from it at type $\dynenv(\cloc, \ptrtag)$.
%
This implies, for example, that for every mutable reference
\tref{\mut}{\typ} associated to a location \cloc the type \typ
must be a subtype of $\loccx(\cloc)$.

\begin{judgment}{Well-typed state}{
  \statetyping[\varcx][\loccx][\dynenv]{\hp}{\sbstate}\quad
}
  \inferrule
  {
    \dom{\hp} = \dom{\sbstate\dotstacks} \\\\
    \forall \cloc\in \dom{\hp}.~\heaplettyping{\cloc}{\hp(\cloc)}{\sbstate\dotstacks(\cloc)}
  }
  {
    \statetyping{\hp}{\sbstate}
  }
\end{judgment}

\begin{judgment}{Well-typed heaplet}{\heaplettyping[\varcx][\loccx][\dynenv]{\cloc}{\val}{\stack}}

  \inferrule[\hptracked]
    {
    \cloc \in \dom{\loccx} \\
    \stacktyping{\shr}{\cloc}{\stack}{\loccx(\cloc)} \\\\
    \typing{\varcx}{\emptyset}{\loccx}{\dynenv}{\val}{\loccx(\cloc)}{\loccx}{}
    }
    {
      \heaplettyping{\cloc}{\val}{\stack}
    }

  \inferrule[\hpuntracked]
    {
    \cloc \notin \dom{\loccx} \\
    \stacktyping{\shr}{\cloc}{\stack}{\typ} \\\\
    \typing{\varcx}{\emptyset}{\loccx}{\dynenv}{\val}{\typ}{\loccx}{}
    }
    {
      \heaplettyping{\cloc}{\val}{\stack}
    }
\end{judgment}


\begin{judgment}{Well-typed stacks}{
    \stacktyping[\varcx][\dynenv]{\shr}{\cloc}{S,(\sharedro, \ptrtag, \_)}{\typ}
}

  \inferrule[\hpshr]
  {
    \dynenv(\cloc, \ptrtag) = \tref{\shr}{\typ'} \\
    \stacktyping{\shr}{\cloc}{S}{\typ} \\\\
    \subtyping{\typ}{\typ'}
  }
  {
    \stacktyping{\shr}{\cloc}{S,(\sharedro, \ptrtag, \_)}{\typ}
  }

  \inferrule[\hpshrmut]
  {
    \stacktyping{\mut}{\cloc}{S}{\typ}
  }
  {
    \stacktyping{\shr}{\cloc}{S}{\typ}
  }

  \inferrule[\hpmut]
  {
    \dynenv(\cloc, \ptrtag) = \tref{\mut}{\typ'} \\
    \stacktyping{\mut}{\cloc}{S}{\typ} \\\\
    \subtyping{\typ}{\typ'} \\
    \subtyping{\typ'}{\typ}
  }
  {
    \stacktyping{\mut}{\cloc}{S,(\unique, \ptrtag, \_)}{\typ}
  }

  \inferrule[\hpmutstrg]
  {
    \stacktyping{\strg}{\cloc}{S}{\typ}
  }
  {
    \stacktyping{\mut}{\cloc}{S}{\typ}
  }

  \inferrule[\hpstrg]
  {
    \dynenv(\cloc, \ptrtag) = \tptr{\cloc} \\
    % \valtyping{\varcx}{\emptyset}{\loccx}{\dynenv}{\val}{\loccx(\cloc)} \\\\
    \stacktyping{\strg}{\cloc}{S}{\typ}
  }
  {
    \stacktyping{\strg}{\cloc}{S,(\unique, \ptrtag, \_)}{\typ}
  }

  \inferrule[\hpempty]
  {}
  {
    \stacktyping{\strg}{\cloc}{\emptyset}{\typ}
  }

  \inferrule[\hpdisabled]
  {
    \stacktyping{\ast}{\cloc}{S}{\typ}
  }
  {
    \stacktyping{\ast}{\cloc}{S,(\disabled, \_, \_)}{\typ}
  }
\end{judgment}


==> metatheory/syntax.tex <==
\bpara{Syntax of Expressions}
{
\small
$$
\begin{array}{rrcll}
    \multicolumn{5}{c}{
        \aa,\lvar \in \mathit{RefineVar} \qquad \cloc \in \mathit{Loc} \qquad \xx, \ff \in \mathit{Var} \qquad t \in \mathit{Tag}
    }
    \\
    \syntaxcat{Expressions} &
    e & ::=
              & \blet{\xx}{e}{e}                                          & \textit{let-bind}       \\
      && \mid & \blet{\xx}{\new{\lvar}}{e}                                & \textit{let-alloc}       \\
      && \mid & \bif{\ee}{e}{e}                                           & \textit{if-then-else} \\
      && \mid & \eunpack{\xx}{\aa}{e}                                     & \textit{unpacking} \\
      && \mid & \fcall{e}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}  & \textit{function call} \\
      && \mid & \sassign{\place}{\ee}                                     & \textit{assignment} \\
      && \mid & \rvstrgref{\place} \mid \rvmutref{\place} \mid \rvshrref{\place} & \textit{(re)borrows} \\
      && \mid & \deref{\place}                                            & \textit{potinter dereference} \\
      && \mid & \xx                                                       & \textit{variables} \\
      && \mid & \val                                                      & \textit{values} \\

    \syntaxcat{Values} &
    \val & ::=
                    & \vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}   & \textit{(recursive) functions} \\
            && \mid & \ctrue \mid \cfalse               & \textit{booleans}  \\
            && \mid & 0, \pm 1, \dots                   & \textit{integers}  \\
            && \mid & \poison                           & \textit{uninitialized memory} \\
            && \mid & \vptr{\cloc}{\ptrtag}             & \textit{tagged pointers} \\
            && \mid & \vvec{n}{\val'}                   & \textit{vector values} \\
            && \mid & \vecnew                           & \textit{vector new}  \\
            && \mid & \vecpush                          & \textit{vector push} \\
            && \mid & \vecindexmut                      & \textit{vector mutable indexing} \\

      \syntaxcat{Logic} &
      \expr & ::= & \ctrue \mid \cfalse \mid 0, \pm 1, \dots & \textit{constants} \\
      && \mid & \aa \mid \expr = \expr & \textit{variables and equality} \\
      && \mid & \lnot \expr \mid \expr [\land,\vee] \expr \mid \expr [+, - , *] \expr  & \textit{bool and  arithmetic} \\
      && \mid & \cloc                                                             & \textit{locations} \\


    \syntaxcat{A-values} &
        \aval & ::=  & \val \mid \xx  \\

         \syntaxcat{Place} &
        \place & ::= & \xx \mid \vptr{\cloc}{\ptrtag} \\

    % \syntaxcat{Pointer Tag} &
    %     \ptrtag &  &
    \end{array}
$$
}

\bpara{Syntax of Types}
%%
{
\small
\[
\begin{array}{rrcll}
    \syntaxcat{Types} &
        \typ & :=   & \rtyp{\tcon}{\expr}                      & \textit{indexed type} \\
            && \mid & \texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}  & \textit{existential type} \\
            && \mid & \tptr{\loc}                              & \textit{pointer to location $\loc$}\\
            && \mid & \tbor{\lft}{\bormode}{\typ}              & \textit{borrowed reference (mutable or shared)}  \\
            && \mid & \uninit{n}                               & \textit{uninitialized memory of size $n$} \\
            && \mid & \polysig{\overline{\tvar}}
                              {\overline{\aa: \sort}}
                              {\expr}
                              {\loccx}
                              {\overline{\typ}}
                              {\typ}
                              {\loccx} \\
    \syntaxcat{Base Types} &
        \tcon & ::= & \tint  \mid \tbool \mid \tvec     & \textit{integers, booleans, and vectors} \\
    \syntaxcat{Modifier} &
        \bormode & ::=   & \mut \mid \shr  & \textit{mutable or shared} \\
    \syntaxcat{Locations} &
        \loc & := & \lvar \mid \cloc  & \textit{a concrete or abstract location}\\
    \syntaxcat{Sorts} &
        \sort  & := &  \sint \mid \sbool \mid \sloc \lftonly{\mid  \slft}\\

    \syntaxcat{Refinement contexts} &
        \varcx & :=   & \emptyset
                    \mid \varcx, \aa: \sort
                    \mid \varcx, \expr \\
    \syntaxcat{Location contexts} &
        \loccx & :=   & \emptyset \mid \loccx, \mapstoowned{\loc}{\typ} \\
    \syntaxcat{Value contexts} &
        \env & :=   & \emptyset \mid \env, \mapstoenv{\xx}{\typ} \\
    \syntaxcat{Dynamic Location contexts} &
        \dynenv & :=   & \emptyset \mid \dynenv, \mapstoowned{(\cloc,\ptrtag)}{\typ}
        %& \textit{Only references or pointer types.}\\
\end{array}
\]
}


==> metatheory/theorems/preservation.tex <==
\begin{restatable}[Preservation]{theorem}{preservation}
\label{theorem:preservation}
If
\begin{itemize}
\item $
\typing{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\rexpr}{\typ}{\loccx}{\dynenv}
$,
\item \eval{\hp_i}{\sbstate_i}{\rexpr}{\hp_o}{\sbstate_o}{\rexpr_o}, and
\item \statetyping[\varcx][\loccx_i][\dynenv_i]{\hp_i}{\sbstate_i},
\end{itemize}
then there exist $\loccx_o$ and $\dynenv_o \supseteq \dynenv_i$, such that
\begin{itemize}
    \item $
    \typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\rexpr_o}{\typ}{\loccx}{\dynenv}
    $ and
    \item \statetyping[\varcx][\loccx_o][\dynenv_o]{\hp_o}{\sbstate_o}
\end{itemize}
\end{restatable}


==> metatheory/theorems/progress.tex <==
\begin{restatable}[Progress]{theorem}{progress}
\label{theorem:progress}
If
\typing{\emptyset}{\emptyset}{\loccx_i}{\dynenv_i}{\rexpr}{\typ}{\loccx_o}{\dynenv_o}
and
\statetyping[\emptyset][\loccx_i][\dynenv_i]{\hp_i}{\sbstate_i},
then
\begin{itemize}
\item \rexpr is a value,
\item \evalerr{\hp_i}{\sbstate_i}{\rexpr}, or
\item there exists
     $\hp_o$, $\sbstate_o$,
     and $\rexpr_o$ so that
    \eval{\hp_i}{\sbstate_i}{\rexpr}{\hp_o}{\sbstate_o}{\rexpr_o}.
\end{itemize}
\end{restatable}


==> metatheory/theorems/soundness.tex <==
\begin{restatable}[Soundness]{theorem}{soundness}
\label{them:soundness}
If
\begin{itemize}
\item $
\typing{\varcx}{\emptyset}{\loccx_i}{\dynenv_i}{\rexpr_i}{\typ}{\loccx}{\_}
$,
\item \statetyping[\varcx][\loccx_i][\dynenv_i]{\hp_i}{\sbstate_i}, and
\item \goesto
      {\hp_i}{\sbstate_i}{\rexpr_i}
      {\hp}{\sbstate}{\rexpr}.
\end{itemize}
then
\begin{itemize}
    \item $\rexpr$ is a value and there exist $\loccx_o $ and $\dynenv_o \supseteq \dynenv_i$ so that
    \typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\rexpr}{\typ}{\loccx}{\_}, or
    \item
     $\evalerr{\hp_o}{\sbstate_o}{\rexpr}$, or
     \item there exists $\loccx_o$, $\dynenv_o \supseteq \dynenv_i$, $\hp_o, \sbstate_o$, and $\rexpr_o$ such that
     $\eval{\hp}{\sbstate}{\rexpr}{\hp_o}{\sbstate_o}{\rexpr_o}$,
     \statetyping[\varcx][\loccx_o][\dynenv_o]{\hp_o}{\sbstate_o}, and
    \typing{\varcx}{\emptyset}{\loccx_o}{\dynenv_o}{\rexpr_o}{\typ}{\loccx}{\_}.
\end{itemize}
\end{restatable}


==> metatheory/type-substitution.tex <==
\begin{lemma}[Type substitution]\label{lemma:type-substitution}
Given \sortck[\varcx_1]{\expr}{\sort} and
          \typing{\varcx_1,\aa:\sort,\varcx_2}
              {\env}
              {\loccx_i}
              {\dynenv}
              {\ee}
              {\typ}
              {\loccx_o}
              {}
          then

          \typing{\varcx_1,\varcx_2[\expr/\aa]}
              {\env[\expr/\aa]}
              {\loccx_i[\expr/\aa]}
              {\dynenv[\expr/\aa]}
              {\ee[\expr/\aa]}
              {\typ[\expr/\aa]}
              {\loccx_o[\expr/\aa]}
              {}
\end{lemma}
\begin{proof}
\begingroup
    \newcommand\indelta{\ensuremath{\varcx_1,\aa:\sort, \varcx_2}}
    \newcommand\outdelta{\ensuremath{\varcx_1,\varcx_2[\expr/\aa]}}
    \newcommand\s{[\expr/\aa]}

    By induction on the typing derivation.

    \begin{itemize}
        \item \textbf{Case \tsub:} Inverting the rules we have:
        \begin{enumerate}
            \item \typing{\indelta}{\env}{\loccx_i}{\dynenv}{\ee}{\typ_1}{\loccx}{}
            \item \subtyping[\indelta]{\typ_1}{\typ}
            \item \loccxinc{\indelta}{}{}{\loccx}{\loccx_o}
        \end{enumerate}
        We apply the inductive hypothesis to (1) and Lemma~\ref{lemma:subtyping-substitution} to (2) and (3) to get
        \begin{enumerate}
            \item \typing{\outdelta}{\env\s}{\loccx_i\s}{\dynenv\s}{\ee\s}{\typ_1\s}{\loccx\s}{}
            \item \subtyping[\outdelta]{\typ_1\s}{\typ\s}
            \item \loccxinc{\outdelta}{}{}{\loccx\s}{\loccx_o\s}
        \end{enumerate}

        \item \textbf{Case \tlet:} By inversion of the rule:
        \begin{enumerate}
            \item \typing{\indelta}{\env}{\loccx_i}{\dynenv}{\ee_x}{\typ_x}{\loccx}{}
            \item \typing{\indelta}{\env,x:\typ_x}{\loccx}{\dynenv}{\ee_x}{\typ}{\loccx_o}{}
            \item $\xx\notin \dom{\env}$
        \end{enumerate}
        Applying inductive hypothesis we get
        \begin{enumerate}
            \item \typing{\outdelta}{\env\s}{\loccx_i\s}{\dynenv\s}{\ee_x\s}{\typ_x\s}{\loccx\s}{}
            \item \typing{\outdelta}{(\env,x:\typ_x)\s}{\loccx\s}{\dynenv\s}{\ee_x\s}{\typ\s}{\loccx_o\s}{}
        \end{enumerate}
        By definition we have $(\env,x:\typ_x)\s = \env\s,x: \typ_x\s$ and $\dom{\env} = \dom{\env\s}$,
        thus we conclude by applying \tlet.

        \item \textbf{Case \tnew:} By inversion of the rule:
        \begin{enumerate}
            \item \typing{\indelta,\lvar:\sloc}{\env, \xx:\tptr{\lvar}}{\loccx_i,\lvar\mapsto\uninit{1}}{\dynenv}{\ee}{\typ}{\loccx_o}{}
            \item \wf[\indelta]{\typ}
            \item \wf[\indelta]{\loccx_o}
            \item $\xx \notin \dom{\env}$
            \item $\lvar \notin \dom{\indelta}$
        \end{enumerate}
        Applying the inductive hypothesis and Lemma~\ref{lemma:wf-substitution} we have
        \begin{enumerate}
            \item \typing{\varcx_1,(\varcx_2,\lvar:\sloc)\s}{(\env, \xx:\tptr{\lvar})\s}{(\loccx_i,\lvar\mapsto\uninit{1})\s}{\dynenv\s}{\ee\s}{\typ\s}{\loccx_o\s}{}
            \item \wf[\outdelta]{\typ\s}
            \item \wf[\outdelta]{\loccx_o\s}
        \end{enumerate}
        By (5) we have $\lvar \neq \aa$, then by definition of substitution we have
        $$
          \typing{\outdelta,\lvar:\sloc}{\env\s, \xx:\tptr{\lvar}}{\loccx_i\s,\lvar\mapsto\uninit{1}}{\dynenv\s}{\ee\s}{\typ\s}{\loccx_o\s}{}
        $$
        We conclude by applying \tnew.

        \item \textbf{Case \tif:}
        Similarly, follows by applying the inductive hypothesis and definition of substitution.

        % \item \textbf{Case \tseq} By inductive hypotheses \ref{case:type-substitution:expr} and \ref{case:type-substitution:stmt}.

        \item \textbf{Case \tunpack} By inversion of the rule:
        \begin{enumerate}
            \item \typing{\indelta}{\env_1,x:\bty[\bb],\env_2}{\loccx_i}{\dynenv}{\ee}{\typ}{\loccx_o}{}
            \item \wf[\indelta]{\typ}
            \item \wf[\indelta]{\loccx_o}
            \item $\bb \notin \dom{\indelta}$
        \end{enumerate}
        Applying the inductive hypothesis and Lemma~\ref{lemma:wf-substitution} we hve
        \begin{enumerate}
            \item \typing{\varcx_1,(\varcx_2, \bb:\sort)\s}{(\env_1,x:\bty[\bb],\env_2)\s}{\loccx_i\s}{\dynenv\s}{\ee\s}{\typ\s}{\loccx_o\s}{}
            \item \wf[\outdelta]{\typ\s}
            \item \wf[\outdelta]{\loccx_o\s}
        \end{enumerate}
        Because of (4) then $\aa\neq\bb$ and consequently we have
        \typing{\outdelta, \bb:\sort}{(\env_1,x:\bty[\bb],\env_2)\s}{\loccx_i\s}{\dynenv\s}{\ee\s}{\typ\s}{\loccx_o\s}{}.
        We conclude by applying \tunpack.

        \item \textbf{Case \tcall} By inversion of the rule:
        By induction hypothesis, Assumption~\ref{assumption:model:substitution} and
        and lemmas~\ref{lemma:subtyping-substitution}, \ref{lemma:wf-substitution} and \ref{lemma:well-sortedness-substitution}.

        \item \textbf{Case \tfun} By inversion of the rule:
        \begin{enumerate}
           \item $\ff \not \in \dom{\env}$
           \item $\forall i. \xx_i \notin \dom{\env}$
           \item $\forall i. \bb_i \notin \dom{\indelta}$
           \item \typing{\indelta,\overline{\bb: \sort},\expr'}
                        {\env,
                            \overline{\xx : \typ},
                            \ff: \polysig{\overline{\tvar}}{{\overline{\bb: \sort}}}
                                        {{\expr'}}{\loccx_{i}}
                                        {\overline{\typ}}
                                        {{\typ}}
                                        {\loccx_{o}}
                            }
                        {\loccx_i}{\dynenv}
                        {\ee}
                        {\typ}{\loccx_o}
                        {}
        \end{enumerate}
        By applying the inductive hypothesis:

        \begin{enumerate}
            \setcounter{enumi}{3}
           \item \typing{\varcx_1,(\varcx_2,\overline{\bb: \sort},\expr')\s}
                        {(\env,
                            \overline{\xx : \typ},
                            \ff: \polysig{\overline{\tvar}}{{\overline{\bb: \sort}}}
                                        {{\expr'}}{\loccx_{i}}
                                        {\overline{\typ}}
                                        {{\typ}}
                                        {\loccx_{o}}
                        )\s}
                        {\loccx_i\s}{\dynenv\s}
                        {\ee\s}
                        {\typ\s}{\loccx_o\s}
                        {}
        \end{enumerate}
        By (3) we have $b_i \neq \aa$ for all $i$ and by definition of substitution we have:
        \begin{enumerate}
            \setcounter{enumi}{3}
           \item \typing{\varcx_1,\varcx_2\s,\bb: \sort,\expr'}
                        {\env\s,
                            \overline{\xx : \typ},
                            \ff: \polysig{}{{\overline{\bb: \sort}}}
                                        {{\expr'\s}}{\loccx_{i}\s}
                                        {\overline{\typ\s}}
                                        {{\typ\s}}
                                        {\loccx_{o}\s}
                        }
                        {\loccx_i\s}{\dynenv\s}
                        {\ee\s}
                        {\typ\s}{\loccx_o\s}
                        {}
        \end{enumerate}
        We conclude by applying \tfun.

        \item \textbf{Case \ttvar,\ttrue,\tfalse,\tconstint,\tumem,\ttptr:} Direct since they apply to expressions
            closed under \varcx.
        % \item \textbf{Case \tskip:} By applying rule \tskip.

        \item \textbf{Cases \tassignstrg, \tassign, \tstrgmutrebor, \tmutmutrebor, \tstrgrebor, \tderef and \tderefstrg}
            All cases follow directly by inductive hypothesis and Lemma~\ref{lemma:subtyping-substitution}
    \end{itemize}
\endgroup
\end{proof}

\begin{lemma}[Subtyping Substitution]\label{lemma:subtyping-substitution}
Given \sortck[\varcx_1]{\expr}{\sort}, then

\begin{enumerate}[label=\roman*]
    \item\label{case:subtyping-substitution:subtyping} If \subtyping[\varcx_1,\aa:\sort,\varcx_2]{\typ_1}{\typ_2} then
          \subtyping[\varcx_1,\varcx_2[\expr/\aa]]{\typ_1[\expr/\aa]}{\typ_2[\expr/\aa]}.
    \item\label{case:subtyping-substitution:loccxinc} If \loccxinc{\varcx_1,\aa:\sort,\varcx_2}{}{}{\loccx_1}{\loccx_2} then
          \loccxinc{\varcx_1,\varcx_2[\expr/\aa]}{}{}{\loccx_1[\expr/\aa]}{\loccx2[\expr/\aa]}.
\end{enumerate}
\end{lemma}
\begin{proof}
\begingroup
\newcommand\indelta{\varcx_1,\aa:\sort,\varcx_2}
\newcommand\outdelta{\varcx_1,\varcx_2[\expr/\aa]}
\newcommand\s{[\expr/\aa]}
    By mutual induction on the derivation trees:

    \textbf{Case \ref{case:subtyping-substitution:subtyping})}

    \begin{itemize}
        \item \textbf{Case \subptr and \submem:} By applying the rule since they apply to arbitrary context.
        \item \textbf{Case \subrtyp:} By inversion of the rule we have \entailment{\indelta}{\expr_1 = \expr_2}.
        Thus, by assumption~\ref{assumption:model:substitution} we know \entailment{\outdelta}{(\expr_1 = \expr_2)\s}.
        Therefore, by definition of substitution, \entailment{\outdelta}{\expr\s = \expr_\s}.
        Applying rule \subrtyp we have \subtyping[\outdelta]{\rtyp{\bty\s}{\expr_1\s}}{\rtyp{\bty\s}{\expr_2\s}}.
        By definition of substitution
        $$
        \subtyping[\outdelta]{\bty[\expr_1]\s}{\bty[\expr_2]\s}
        $$
        which concludes this part of the proof.

        \item \textbf{Case \subunpack:} By inversion of the rule we have
        $$
        \subtyping[\indelta,\bb:\getsort{\bty},\expr']{\bty[\bb]}{\typ}
        $$
        Applying, the inductive hypothesis we get
        $$
        \subtyping[\varcx_1,(\varcx_2, \bb:\getsort{\bty},\expr')\s]{\bty[\bb]\s}{\typ\s}
        $$
        By definition of substitution and since $\bb$ must be fresh:
        $$
        \subtyping[\varcx_1,\varcx_2\s, \bb:\getsort{\bty},\expr'\s]{\bty[\bb]\s}{\typ\s}
        $$
        Now we apply rule \subunpack to get
        $$
        \subtyping[\varcx_1,\varcx_2\s]{\texists{\bb}{\bty[\bb]}{\expr'\s}}{\typ\s}
        $$
        And by definition of substitution we have
        $$
        \subtyping[\varcx_1,\varcx_2\s]{(\texists{\bb}{\bty[\bb]}{\expr'})\s}{\typ\s}
        $$
        which is the desired goal.

        \item \textbf{Case \subexists:} By inversion of the rule we have \entailment{\indelta}{\expr_2[\expr_1/\bb]}
        Thus, by Assumption~\ref{assumption:model:substitution}, \entailment{\outdelta}{\expr_2[\expr_1/\bb]\s}.
        Since $\bb$ must be fresh then $\bb \notin \fv{\expr}$ and by Lemma~\ref{lemma:substitution-composition}
        we have \entailment{\outdelta}{\expr\s[\expr_1\s/\bb]}.
        Now, applying \subexists we get:
        $$
        \subtyping[\outdelta]{\bty[\expr_1\s]}{\texists{\bb}{\bty[\bb]}{\expr_2\s}}
        $$
        Finally, by definition of substitution we get
        $$
        \subtyping[\outdelta]{\bty[\expr_1]\s}{\texists{\bb}{\bty[\bb]}{\expr_2}\s}
        $$
        which concludes this part of the proof.

        \item \textbf{\subbormut and \subborshr:} By the inductive hypothesis

        \item \textbf{\subfun:} By inversion of the rule
        \begin{enumerate}
            \item \entailment{\indelta, \overline{\bb: \sort_\bb}}{\expr_2 \Rightarrow \expr_1}
            \item \loccxinc
                    {\indelta, \overline{\bb: \sort_\bb}}
                    {\elftcx}{\llftcx}
                    {\loccx_{2i}}
                    {\loccx_{1i}}
            \item $\forall i. \subtyping[\indelta, \overline{\bb: \sort_\bb}]{\typ_{2i}}{\typ_{1i}}$
            \item \loccxinc
                    {\indelta, \overline{\bb: \sort_\bb}}
                    {}{}
                    {\loccx_{1o}}
                    {\loccx_{2o}}
            \item \subtyping[\indelta, \overline{\bb: \sort_\bb}]{\typ_{1o}}{\typ_{2o}}
        \end{enumerate}
        Applying the inductive hypotheses and Assumption~\ref{assumption:model:substitution} get get:
        \begin{enumerate}
            \item \entailment{\varcx_1,(\varcx_2, \overline{\bb: \sort_\bb})\s}{(\expr_2 \Rightarrow \expr_1)\s}
            \item \loccxinc
                    {\varcx_1,(\varcx_2, \overline{\bb: \sort_\bb})\s}
                    {}{}
                    {\loccx_{2i}\s}
                    {\loccx_{1i}\s}
            \item $\forall i. \subtyping[\varcx_1,(\varcx_2, \overline{\bb: \sort_\bb})\s]{\typ_{2i}\s}{\typ_{1i}\s}$
            \item \loccxinc
                    {\varcx_1,(\varcx_2, \overline{\bb: \sort_\bb})\s}
                    {}{}
                    {\loccx_{1o}\s}
                    {\loccx_{2o}\s}
            \item \subtyping[\varcx_1, (\varcx_2, \overline{\bb: \sort_\bb})\s]{\typ_{1o}\s}{\typ_{2o}\s}
        \end{enumerate}
        Since $\overline{\bb}$ need to be fresh we get
        \begin{enumerate}
            \item \entailment{\varcx_1,\varcx_2\s, \overline{\bb: \sort_\bb}}{(\expr_2 \Rightarrow \expr_1)\s}
            \item \loccxinc
                    {\varcx_1,\varcx_2\s, \overline{\bb: \sort_\bb}}
                    {}{}
                    {\loccx_{2i}\s}
                    {\loccx_{1i}\s}
            \item $\forall i. \subtyping[\varcx_1,\varcx_2\s, \overline{\bb: \sort_\bb}]{\typ_{2i}\s}{\typ_{1i}\s}$
            \item \loccxinc
                    {\varcx_1,\varcx_2\s, \overline{\bb: \sort_\bb}}
                    {}{}
                    {\loccx_{1o}\s}
                    {\loccx_{2o}\s}
            \item \subtyping[\varcx_1, \varcx_2\s, \overline{\bb: \sort_\bb}]{\typ_{1o}\s}{\typ_{2o}\s}
        \end{enumerate}
        We conclude by applying \subfun.
    \end{itemize}

    \textbf{Case \ref{case:subtyping-substitution:loccxinc})}

    \begin{itemize}
        \item \textbf{Case \loccxinctrans:} By inductive hypothesis \ref{case:subtyping-substitution:loccxinc}.
        \item \textbf{Case \loccxincperm:} Direct since if $\loccx'$ is a permutation of $\loccx$ then
        $\loccx'\s$  is also a permutation of $\loccx\s$.
        \item \textbf{Case \loccxincweaken:} By Lemma~\ref{lemma:substitution-concat}.
        \item \textbf{Case \loccxincframe:} By the inductive hypothesis \ref{case:subtyping-substitution:loccxinc}.
        and Lemma~\ref{lemma:substitution-concat}.
        \item \textbf{Case \loccxincsub:} By the inductive hypothesis \ref{case:subtyping-substitution:subtyping}.
    \end{itemize}
\endgroup
\end{proof}

\begingroup
\newcommand\indelta{\varcx_1,\aa:\sort,\varcx_2}
\newcommand\outdelta{\varcx_1,\varcx_2[\expr/\aa]}
\newcommand\s{[\expr/\aa]}

\begin{lemma}[Well-formedness Substitution]\label{lemma:wf-substitution}
Given \sortck[\varcx_1]{\expr}{\sort}, then

\begin{enumerate}[label=\roman*]
    \item If \wf[\indelta]{\typ} then \wf[\outdelta]{\typ\s}
    \item If \wf[\indelta]{\loccx} then \wf[\outdelta]{\loccx\s}
    \item If \wf[\indelta]{\dynenv} then \wf[\outdelta]{\dynenv\s}
\end{enumerate}
\end{lemma}
\begin{proof}
    Each one by induction on the derivation tree.
\end{proof}


\begin{lemma}[Well-sortedness Substitution]\label{lemma:well-sortedness-substitution}
If \sortck[\varcx_1]{\expr}{\sort}, \sortck[\indelta]{\expr'}{\sort'} and \wfvarcx{\varcx_1,\varcx_2}
then \sortck[\outdelta]{\expr'\s}{\sort'}
\end{lemma}
\begin{proof}
    By induction on the derivation tree applying Lemma~\ref{lemma:well-sortedness:weakening} and
    the assumption \sortck[\varcx_1]{\expr}{\sort} on the variable case.
\end{proof}

\endgroup

\begin{lemma}[Well-sortedness Weakening]\label{lemma:well-sortedness:weakening}
If \sortck[\varcx_1]{\expr}{\sort} and \wfvarcx{\varcx_1, \varcx_2} then \sortck[\varcx_2]{\expr}{\sort}.
\end{lemma}
\begin{proof}
    By induction on the derivation tree noting that if $\aa:\sort \in \varcx_1$ and $\wfvarcx{\varcx_1, \varcx_2}$ then
    $\aa:\sort \in \varcx_1, \varcx_2$.
\end{proof}

\begin{lemma}[Substitution composition]\label{lemma:substitution-composition}
    If $\aa \notin \fv{\expr_\bb}$ then $(\expr[\expr_a/\aa])[\expr_\bb/\bb] = (\expr[\expr_b/\bb])[\expr_a[\expr_\bb/\bb]/\aa]$
\end{lemma}
\begin{proof}
    By induction on the structure of $\expr$.
    The interesting case is the variable case.
    Let $\expr = c$ for some variable $c$.
    We have three cases
    \begin{itemize}
        \item $c \neq \aa \wedge c \neq \bb$: By applying the definition of substitution we get $c$ in both sides of the equality.
        \item $c = \aa$: By applying the definition of substitution on the left side of the equality we get
        $\expr_a[\expr_\bb/\bb]$.
        Applying, the definition of substitution on the right side once we get $\aa[\expr_a[\expr_\bb/\bb]/\aa]$.
        Applying it a second time we get $\expr_\aa[\expr_\bb/\bb]$.
        \item $c = \bb$: On the left side we have
        $$
        (\bb[\expr_a/\aa])[\expr_\bb/\bb] = \bb[\expr_\bb/\bb] = \expr_\bb
        $$
        On the right side we have
        $$
        (\bb[\expr_\bb/\bb])[\expr_a[\expr_\bb/\bb]/\aa] = \expr_\bb[\expr_a[\expr_\bb]/\aa]
        $$
        By the assumption $\aa \notin \fv{\expr_\bb}$ we get
        $$
        \expr_\bb[\expr_a[\expr_\bb]/\aa] = \expr_\bb
        $$
        which concludes the proof.
    \end{itemize}
\end{proof}

\begin{lemma}[Substitution Concatenation]\label{lemma:substitution-concat}
    $(\loccx_1,\loccx_2)[\expr/\aa] = \loccx_1[\expr/\aa], \loccx_2[\expr/\aa]$
\end{lemma}
\begin{proof}
    By induction on the structure of $\loccx_2$ applying the definition of substitution.
\end{proof}


==> metatheory/typing.tex <==
\subsection{Well-typed Expressions}
\begin{judgment}{Well-typed Expressions}{\typing{\varcx}{\env}{\loccx}{\dynenv}{\rexpr}{\typ}{\loccx}{\dynenv}}


    \inferrule[\tlet]
    {
        \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\ee_{\xx}}{\typ_{\xx}}{\loccx}{\dynenv}\\\\
        \typing{\varcx}{\env,\mapstoenv{\xx}{\typ_\xx}}{\loccx}{\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv_o}
    }
    {\typing{\varcx}{\env}{\loccx_i}{\dynenv}{\blet{\xx}{\ee_{\xx}}{\ee}}{\typ}{\loccx_o}{\dynenv_o}}

    \inferrule[\tnew]
    {
     \wf{\typ} \\
     \wf{\loccx_o}\\\\
     \typing{\varcx, \lvar:\sloc}
            {\env, \mapstoenv{\xx}{\tptr{\lvar}}}
            {\loccx_i, \mapstoowned{\lvar}{\uninit{1}}}
            {\dynenv}{\ee}{\typ}{\loccx_o}{\dynenv} \\
    }
    {\typing{\varcx}
            {\env}{\loccx_i}{\dynenv}{\blet{\xx}{\new{\lvar}}{e}}{\typ}{\loccx_o}{\dynenv}
    }

    \inferrule[\tsub]
    {
        \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\ee}
            {\typ_1}
            {\loccx}
            {\dynenv} \\\\
        \subtyping{\typ_1}{\typ} \\
        \loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx}{\loccx_o}\\
    }
    {
        \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\ee}
            {\typ}
            {\loccx_o}
            {\dynenv}
    }

    \inferrule[\tif]
    {
        \typing{\varcx}{\env}{\loccx_i}{\dynenv}{\ee}{\rtyp{\tbool}{\expr}}{\loccx_o}{\dynenv_o} \\\\
        \typing{\varcx, \expr}{\env}{\loccx_o}{\dynenv}{\ee_1}{\typ}{\loccx}{\dynenv} \\\\
        \typing{\varcx, \lnot \expr}{\env}{\loccx_o}{\dynenv}{\ee_2}{\typ}{\loccx}{\dynenv} \\
    }
    {\typing{\varcx}{\env}{\loccx_i}{\dynenv_i}{\bif{\ee}{\ee_1}{\ee_2}}{\typ}{\loccx}{\dynenv}}

    \inferrule[\tunpack]
    {
        \typing{\varcx, \aa : \getsort{\tcon}, \expr}{\env_1,\mapstoenv{\xx}{\rtyp{\tcon}{\aa}}, \env_2}
               {\loccx_i}{\dynenv}
               {\ee}{\typ}
               {\loccx_o}{\dynenv}
    }
    {
        \typing{\varcx}{\env_1,\mapstoenv{\xx}{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}, \env_2}
               {\loccx_i}{\dynenv}
               {\eunpack{\xx}{\aa}{e}}{\typ}
               {\loccx_o}{\dynenv}
    }

    \inferrule[\tcall]
    {
        \forall i. \typing{\varcx}{\env}{\loccx}{\dynenv}{\aval_i}{\applysubst{\substvar}{\typ_{i}}}{\loccx}{} \\
        \typing{\varcx}{\env}{\loccx}{\dynenv}{e}
               {\polysig{\overline{\tvar}}
                        {\overline{\aa: \sort}}
                        {\expr}
                        {\loccx_{i}}
                        {\overline{\typ}}
                        {\typ_o}
                        {\loccx_{o}}}
              {\loccx_1, \loccx_2 }{\dynenv} \\
        \substvar = \subst{\overline{\aa}}{\overline{\expr}} \\
        \loccxinc{\varcx}{}{}{\loccx_1}{\applysubst{\substvar}{\loccx_{i}}}\\
        \forall i.\sortck{\expr_i}{\sort_i} \\
        \lmodel{\varcx}{\applysubst{\substvar}{\expr}} \\
        \wf{\dynenv}\\
    }
    {
        \typing{\varcx}{\env}{\loccx}{\dynenv}
               {\fcall{\ee}{\overline{\typ}}{\overline{\expr}}{\overline{\aval}}}
               {\applysubst{\substvar}{\typ_o}}{\applysubst{\substvar}{\loccx_{o}}, \loccx_2}{}
    }
\end{judgment}

\begin{judgment}{Well-typed Expressions (assignment)}{\typing{\varcx}{\env}{\loccx}{\dynenv}{\rexpr}{\typ}{\loccx}{\dynenv}}
    \inferrule[\tassign]
    {
        \rvaltyping{\varcx}{\env}{\loccx_i}{\dynenv}{\ee}{\typ_v}{\loccx_o} \\\\
        \pltyping{\varcx}{\env}{\loccx_o}{\dynenv}{\place}{\tref{\mut}{\typ}}{\loccx_o} \\
        \subtyping{\typ_v}{\typ}
    }
    {\typing{\varcx}{\env}{\loccx_i}{\dynenv}{\sassign{\place}{\ee}}{\uninit{1}}{\loccx_o}{}}

    \inferrule[\tassignstrg]
    {
        \rvaltyping{\varcx}{\env}{\loccx_i}{\dynenv}{\ee}{\typ}{\loccx_o} \\\\
        \pltyping{\varcx}{\env}{\loccx_o}{\dynenv}{\place}{\tptr{\loc}}{\loccx_o}
    }
    {\typing{\varcx}{\env}{\loccx_i}{\dynenv}{\sassign{\place}{\ee}}{\uninit{1}}{\loccx_o[\loc \mapsto \typ]}{}}
\end{judgment}


\begin{judgment}{Well-typed Expressions (values)}{\typing{\varcx}{\env}{\loccx}{\dynenv}{\ee}{\typ}{\loccx}{}}

    \inferrule[\ttvar]
    {\mapstoenv{\xx}{\typ} \in \env}
    {\typing{\varcx}{\env}{\loccx}{\dynenv}{\xx}{\selfty{\typ}{\xx}}{\loccx}{}}

    \inferrule[\ttrue]
    {}
    {\typing{\varcx}{\env}{\loccx}{\dynenv}{\ctrue}{\rtyp{\tbool}{\ctrue}}{\loccx}{}}

    \inferrule[\tfalse]
    {}
    {\typing{\varcx}{\env}{\loccx}{\dynenv}{\cfalse}{\rtyp{\tbool}{\cfalse}}{\loccx}{}}

    \inferrule[\tconstint]
    {}
    {\typing{\varcx}{\env}{\loccx}{\dynenv}{i}{\rtyp{\tint}{i}}{\loccx}{}}


    \inferrule[\tfun]
    {   \typing{\varcx,\overline{\aa: \sort},\expr}
               {\env,
                \overline{\xx : \typ},
                \ff: \polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                             {{\expr}}{\loccx_{i}}
                             {\overline{\typ}}
                             {{\typ}}
                             {\loccx_{o}}
                }
               {\loccx_i}{\dynenv}
               {\ee}
               {\typ}{\loccx_o}
               {}
    }
    {
        \typing{\varcx}{\env}{\loccx}{\dynenv}
               {\vrec{\ff}{\overline{\aa}}{\overline{\xx}}{{e}}}
               {\polysig{\overline{\tvar}}{{\overline{\aa: \sort}}}
                          {\expr}{\loccx_{i}}{\overline{\typ}}
                          {\typ}{\loccx_{o}}
               }
               {\loccx}{\dynenv}
    }

    \inferrule[\ttptr]
    {}
    {\typing{\varcx}{\env}{\loccx}{\dynenv}{\vptr{\cloc}{\ptrtag}}{\dynenv(\cloc, \ptrtag)}{\loccx}{\dynenv}}

    \inferrule[\tumem]
    {}
    {\typing{\varcx}{\env}{\loccx}{\dynenv}{\poison}{\uninit{1}}{\loccx}{\dynenv}}

    \inferrule[\tvecnew]
    {}
    {
        \typing{\varcx}{\env}{\loccx}{\dynenv}{\vecnew}{\loccx}
        {\kw{fn}() \rightarrow \tvec<0>}
        {}
    }

    \inferrule[\tvecpush]
    {}
    {
        \typing
        {\varcx}{\env}{\loccx}{\dynenv}{\vecpush}
        {\polysig{}
            {\lvar:\sloc}{\ctrue}
            {[\mapstoowned{\lvar}{\rtyp{\tvec}{n}}]}
            {\tptr{\lvar}}
            {\uninit{1}}{[\mapstoowned{\lvar}{\rtyp{\tvec}{n + 1}}]}
        }
        {\loccx}
        {}
    }

    \inferrule[\tvecindexmut]
    {}
    {
        \typing
        {\varcx}{\env}{\loccx}{\dynenv}{\vecindexmut}
        {
            \polysig
            {}
            {\aa:\sint,\bb:\sint}
            {0 \leq \bb < \aa}
            {\emptyset}
            {\tref{\mut}{\rtyp{\tvec}{\aa}}, \rtyp{\tint}{\bb}}
            {\tref{\mut}{\typ}}
            {\emptyset}
        }
        {\loccx}
        {}
    }

    \inferrule[\tvecvec]
    {
        n \geq 0 \\
        n > 0 \implies \val = \vptr{\cloc}{\ptrtag} \wedge \forall i \in [0, n).~\dynenv(\cloc + i, \ptrtag) = \tref{\mut}{\typ}
    }
    {
        \typing
        {\varcx}{\env}{\loccx}{\dynenv}{\vvec{n}{\val}}
        {
            \rtyp{\tvec}{n}
        }
        {\loccx}
        {}
    }

\end{judgment}

\begin{judgment}{Well-typed Expressions (borrows)}{\typing{\varcx}{\env}{\loccx}{\dynenv}{\ee}{\typ}{\loccx}{}}

\inferrule[\tstrgrebor]
{\pltyping{\varcx}{\env}{\loccx}{\dynenv}{\place}{\tptr{\loc}}{\loccx}}
{\rvaltyping{\varcx}{\env}{\loccx}{\dynenv}{\rvstrgref{\place}}{\tptr{\loc}}{\loccx}}


\inferrule[\tstrgmutrebor]
{
    \pltyping{\varcx}{\env}{\loccx}{\dynenv}{\place}{\tptr{\loc}}{\loccx} \\
    \subtyping{\loccx(\loc)}{\typ}
}
{\rvaltyping{\varcx}{\env}{\loccx}{\dynenv}{\rvmutref{\place}}{\tref{\mut}{\typ}}{\loccx[\loc\mapsto \typ]}}


\inferrule[\tmutmutrebor]
{\pltyping{\varcx}{\env}{\loccx}{\dynenv}{\place}{\tref{\mut}{\typ}}{\loccx}}
{\rvaltyping{\varcx}{\env}{\loccx}{\dynenv}{\rvmutref{\place}}{\tref{\mut}{\typ}}{\loccx}}



\inferrule[\tshrrebor]
{
    \pltyping{\varcx}{\env}{\loccx}{\dynenv}{\place}{\tref{\bormode}{\typ'}}{\loccx} \\
    \subtyping{\typ'}{\typ}
}
{\rvaltyping{\varcx}{\env}{\loccx}{\dynenv}{\rvshrref{\place}}{\tref{\shr}{\typ}}{\loccx}}

\end{judgment}

\begin{judgment}{Well-typed Expressions (dereference)}{\typing{\varcx}{\env}{\loccx}{\dynenv}{\ee}{\typ}{\loccx}{}}

\inferrule[\tderef]
{\pltyping{\varcx}{\env}{\loccx}{\dynenv}{\place}{\tref{\bormode}{\typ}}{\loccx}}
{\rvaltyping{\varcx}{\env}{\loccx}{\dynenv}{\deref{\place}}{\typ}{\loccx}}


\inferrule[\tderefstrg]
{\typing{\varcx}{\env}{\loccx}{\dynenv}{\place}{\tptr{\loc}}{\loccx}{}}
{\rvaltyping{\varcx}{\env}{\loccx}{\dynenv}{\deref{\place}}{\loccx(\loc)}{\loccx}}
\end{judgment}

\subsection{Location Context Inclusion and Subtyping}

\begin{judgment}{Context inclusion}{\loccxinc{\varcx}{\elftcx}{\llftcx}{\loccx}{\loccx}}
    \inferrule[\loccxinctrans]
        {\loccxinc
        {\varcx}
        {\elftcx}{\llftcx}
        {\loccx_1}
        {\loccx_2}\and
        \loccxinc
                {\varcx}
                {\elftcx}{\llftcx}
                {\loccx_2}
                {\loccx_3}}
        {
            \loccxinc
                {\varcx}
                {\elftcx}{\llftcx}
                {\loccx_1}
                {\loccx_3}
        }

    \inferrule[\loccxincperm]
        {\loccx' \text{ is a permutation of } \loccx}
        {
            \loccxinc
                {\varcx}
                {\elftcx}{\llftcx}
                {\loccx}
                {\loccx'}
        }

    \inferrule[\loccxincweaken]
        {}
        {
            \loccxinc
                {\varcx}
                {\elftcx}{\llftcx}
                {\loccx,\loccx'}
                {\loccx}
        }

    \inferrule[\loccxincframe]
        {
            \loccxinc
                {\varcx}
                {\elftcx}{\llftcx}
                {\loccx_1}{\loccx_2}
        }{
            \loccxinc
                {\varcx}
                {\elftcx}{\llftcx}
                {\loccx,\loccx_1}
                {\loccx, \loccx_2}
        }

    \inferrule[\loccxincsub]
        {
            \subtyping{\typ_1}{\typ_2}
        }
        {
            \loccxinc
                {\varcx}
                {\elftcx}{\llftcx}
                {\mapstoowned{\loc}{\typ_1}}
                {\mapstoowned{\loc}{\typ_2}}
        }
\end{judgment}


\begin{judgment}{Subtyping}{\subtyping[\varcx][\elftcx][\llftcx]{\typ}{\typ}}
    \inferrule[\subptr]
        {}
        {
            \subtyping{\tptr{\loc}}{\tptr{\loc}}
        }

\inferrule[\submem]
        {}
        {
            \subtyping{\uninit{n}}{\uninit{n}}
        }

\inferrule[\subfun]
        {
            \entailment{\varcx, \overline{\aa: \sort}}{\expr_2 \Rightarrow \expr_1} \and
            \loccxinc
                {\varcx, \overline{\aa: \sort}}
                {\elftcx}{\llftcx}
                {\loccx_{2i}}
                {\loccx_{1i}} \and
            \forall i. \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{2i}}{\typ_{1i}} \\
        \loccxinc
            {\varcx, \overline{\aa: \sort}}
            {\elftcx}{\llftcx}
            {\loccx_{1o}}
            {\loccx_{2o}} \and
        \subtyping[\varcx, \overline{\aa: \sort}]{\typ_{1o}}{\typ_{2o}}
        }
        {
            \subtyping{
            \polysig{\overline{\tvar}}
            {\overline{\aa: \sort}}
            {\expr_1}
            {\loccx_{1i}}
            {\overline{\typ_1}}
            {\typ_{1o}}
            {\loccx_{1o}}
            }{
            \polysig{\overline{\tvar}}
            {\overline{\aa: \sort}}
            {\expr_2}
            {\loccx_{2i}}
            {\overline{\typ_2}}
            {\typ_{2o}}
            {\loccx_{2o}}
            }
        }

    \inferrule[\subrtyp]
        {
            \entailment{\varcx}{\expr_1 = \expr_2}
        }{
            \subtyping
                {\rtyp{\tcon}{\expr_1}}
                {\rtyp{\tcon}{\expr_2}}
        }

    \inferrule[\subunpack]
        {
          % \fresh{\aa}{\varcx} \and
           \subtyping
                [\varcx, \aa: \getsort{\tcon}, \expr]
                {\rtyp{\tcon}{\aa}}
                {\typ}
        }{
            \subtyping
                {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}
                {\typ}
        }

    \inferrule[\subexists]
        {
            \entailment{\varcx}{\expr_2[\expr_1/\aa]}
        }{
            \subtyping
                {\rtyp{\tcon}{\expr_1}}
                {\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr_2}}
        }

    \inferrule[\subborshr]
        {
            \subtyping{\typ_1}{\typ_2}
        }{
            \subtyping
                {\tbor{\lft}{\shr}{\typ_1}}
                {\tbor{\lft}{\shr}{\typ_2}}
        }

    \inferrule[\subbormut]
        {
            \subtyping{\typ_1}{\typ_2}
            \and
            \subtyping{\typ_2}{\typ_1}
        }{
            \subtyping
                {\tbor{\lft}{\mut}{\typ_1}}
                {\tbor{\lft}{\mut}{\typ_2}}
        }
\end{judgment}




==> metatheory/vectors.tex <==

\subsection{Operational semantics}

\begin{judgment}{Operational Semantics}{\eval{\hp}{\sbstate}{\ee}{\hp}{\sbstate}{\rexpr}}
    \inferrule[\opvecnew]
    {
    }
    {
        \eval
          {\hp}{\sbstate}
          {\fcall{\vecnew}{}{}{}}
          {\hp}{\sbstate}
          {\vvec{0}{\poison}}
    }

    \inferrule[\opvecpush]
    {
        \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate} \\\\
        \transdealloc{\sbstate}{\cloc'}{\ptrtag'}{n}{\sbstate'} \\\\
        \transalloc{\sbstate'}{\cloc''}{\ptrtag''}{n+1}{\sbstate_o} \\\\
        [\cloc'', \cloc'' + n] \mathrel{\#} \dom{\hp} \\\\
        \hp_i = \hp\hbind{\cloc}{\vvec{n}{\vptr{\cloc'}{\ptrtag'}}}\hbindn{n}{\cloc'}{\overline{\val}} \\\\
        \hp_o = \hp\hbind{\cloc}{\vvec{n+1}{\vptr{\cloc''}{\ptrtag''}}}\hbindn{n+1}{\cloc''}{\overline{\val} \append [\val]}
    }
    {
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecpush}{}{\cloc}{\vptr{\cloc}{\ptrtag}, \val}}
          {\hp_o}{\sbstate_o}
          {\poison}
    }

    \inferrule[\opvecpushempty]
    {
        \transwrite{\sbstate_i}{\cloc}{\ptrtag}{\sbstate} \\\\
        \transalloc{\sbstate}{\cloc'}{\ptrtag'}{1}{\sbstate_o} \\\\
        \cloc' \notin \dom{\hp} \\\\
        \hp_i = \hp\hbind{\cloc}{\vvec{0}{\val'}} \\\\
        \hp_o = \hp\hbind{\cloc}{\vvec{1}{\vptr{\cloc'}{\ptrtag'}}}\hbind{\cloc'}{\val}
    }
    {
        \eval
          {\hp_i}{\sbstate_i}
          {\fcall{\vecpush}{}{\cloc}{\vptr{\cloc}{\ptrtag}, \val}}
          {\hp_o}{\sbstate_o}
          {\poison}
    }

    \inferrule[\opvecindexmut]
    {
        \cloc + i \in \dom{\hp} \\\\
        \transread{\sbstate_i}{\cloc}{\ptrtag}{\sbstate} \\\\
        \transreborrow{\sbstate}{\cloc' + i}{\ptrtag'}{\ptrtag''}{\mut}{\sbstate_o} \\\\
        \hp = \hp'\hbind{\cloc}{\vvec{n}{\vptr{\cloc'}{\ptrtag'}}}
    }
    {
        \eval
          {\hp}{\sbstate_i}
          {\fcall{\vecindexmut}{}{}{\vptr{\cloc}{\ptrtag}, i}}
          {\hp}{\sbstate_o}
          {\vptr{\cloc' + i}{\ptrtag''}}
    }
\end{judgment}




% \begin{judgment}{Subtyping}{\subtyping{\typ}{\typ}}
%     \inferrule
%         {}
%         {
%             \subtyping{}\tvec
%         }
% \end{judgment}

\subsection{Preservation}

\preservation*
\begin{proof}
    We add the following cases to the proof of \textbf{Rule \tcall}.

\end{proof}

\progress*
\begin{proof}
    We need to modify the proof of case \tfun by applying the extended cannonical forms lemma for
    functions (\ref{lemma:canonical:fun}) adding the following cases:
\end{proof}



==> metatheory/vectors/syntax.tex <==
\begin{figure}
\[
\begin{array}{rrcll}

    \syntaxcat{Values} &
        \val & ::=  & \dots \\
            && \mid & \vvec{n}{\val} \\
            && \mid & \vecpush \\
            && \mid & \vecnew  \\
            && \mid & \vecindexmut \\

    \syntaxcat{Base Types} &
        \tcon & ::= & \dots \mid \tvec     & \textit{integers, booleans, or user-defined} \\

\end{array}
\]
\caption{Extension of Syntax for Vectors}
\end{figure}


==> metatheory/vectors/typing.tex <==
\begin{figure}
\begin{judgment}{Value typing}{\valtyping{\varcx}{\env}{\emptyset}{\dynenv}{\val}{\typ}}

    \inferrule[\tvecnew]
    {}
    {
        \valtyping{\varcx}{\env}{\emptyset}{\dynenv}{\vecnew}
        {\kw{fn}() \rightarrow \tvec}
    }

    \inferrule[\tvecpush]
    {}
    {
        \valtyping
        {\varcx}{\env}{\emptyset}{\dynenv}{\vecpush}
        {\polysig{}
            {\lvar:\sloc}{\ctrue}
            {[\mapstoowned{\lvar}{\rtyp{\tvec}{n}}]}
            {\tptr{\lvar}}
            {\uninit{1}}{[\mapstoowned{\lvar}{\rtyp{\tvec}{n + 1}}]}
        }
    }

    \inferrule[\tvecindexmut]
    {}
    {
        \valtyping
        {\varcx}{\env}{\emptyset}{\dynenv}{\vecindexmut}
        {
            \polysig
            {}
            {\aa:\sint,\bb:\sint}
            {0 \leq \bb < \aa}
            {\emptyset}
            {\tref{\mut}{\rtyp{\tvec}{\aa}}, \rtyp{\tint}{\bb}}
            {\tref{\mut}{\typ}}
            {\emptyset}
        }
    }

    \inferrule[\tvecvec]
    {
        n \geq 0 \\
        n > 0 \implies \val = \vptr{\cloc}{\ptrtag} \wedge \forall i \in [0, n).~\dynenv(\cloc + i, \ptrtag) = \tref{\mut}{\typ}
    }
    {
        \valtyping
        {\varcx}{\env}{\emptyset}{\dynenv}{\vvec{n}{\val}}
        {
            \rtyp{\tvec}{n}
        }
    }
\end{judgment}
\caption{Typing for Vectors}
\end{figure}

==> metatheory/wellformed.tex <==
\subsection{Well-formedness}
%
The well-formedness judgments (\wfvdash) document the binding struct
of the grammar as well as well-sortedness of refinements.
%
In what follows, we assume well-formed implicitly in other judgments.
%

\begin{judgment}{Well-formed Types}{\wf[\varcx]{\typ}}
    \inferrule[\twfidx]
    {\sortck[\varcx]{\expr}{\getsort{\tcon}}}
    {\wf[\varcx]{\rtyp{\tcon}{\expr}}}

    \inferrule[\twfex]
    {\sortck[\varcx,\aa :\getsort{\tcon} ]{\expr}{\tbool{}}}
    {\wf[\varcx]{\texists{\aa}{\rtyp{\tcon}{\aa}}{\expr}}
    }

    \inferrule[\twfptr]
    {
        \sortck{\loc}{\sloc}
    }
    {
        \wf[\varcx]{\tptr{\loc}}
    }

    \inferrule[\twfref]
    {\wf[\varcx]{\typ}}
    {\wf[\varcx]{\tbor{\lft}{\bormode}{\typ}}
    }

    \inferrule[\twfmem]
    {}
    {\wf[\varcx]{\uninit{n}}
    }

    \inferrule[\twffun]
    {
        \sortck[\varcx,\overline{\aa: \sort}]{\expr}{\sbool}\\
        \dom{\loccx_o} \subseteq \dom{\loccx_i} \\
        % \varcx' = \varcx\setminus\{(\lvar:\sloc) \mid  (\lvar:\sloc) \in \varcx\}\\
        \wf[\varcx',\overline{\aa: \sort}]{\loccx_i}\\
        \forall i. \wf[\varcx',\overline{\aa: \sort}]{\typ_i}\\
        \wf[\varcx',\overline{\aa: \sort}]{\typ_o}\\
        \wf[\varcx',\overline{\aa: \sort}]{\loccx_o}
    }
    {\wf[\varcx]{\polysig{\overline{\tvar}}
    {{\overline{\aa: \sort}}}
    {{\expr}}
    {\loccx_i}
    {\overline{\typ}}
    {\typ_o}
    {\loccx_o}}
    }
\end{judgment}

\begin{judgment}{Well-formed Value Contexts}{\wf[\varcx]{\env}}

    \inferrule[\twfbind]
        {\wf[\varcx]{\typ}\\
        \wf[\varcx]{\env}
        }
        {\wf[\varcx]{\env, \mapstoenv{\xx}{\typ}}}

    \inferrule[\twfemp]{}{\wf[\varcx]{\emptyset}}
\end{judgment}

\begin{judgment}{Well-formed Dynamic Contexts}{\wf[\varcx]{\dynenv}}
    \inferrule[\twfbind]
        {\wf[\varcx]{\typ}\\
        \wf[\varcx]{\dynenv}
        }
        {\wf[\varcx]{\dynenv, \mapstoowned{(\cloc,\ptrtag)}{\typ}}}

    \inferrule[\twfemp]{}{\wf[\varcx]{\emptyset}}
\end{judgment}
\begin{judgment}{Well-formed Location contexts}{\wf[\varcx]{\loccx}}
    \inferrule[\twfbind]
        {
        \wf[\varcx]{\typ} \\
        \wf[\varcx]{\loccx} \\
        \sortck{\loc}{\sloc} \\
        \loc \notin \dom{\loccx}
        }
        {\wf[\varcx]{\loccx, \mapstoowned{\loc}{\typ}}}

    \inferrule[\twfemp]{}{\wf[\varcx]{\emptyset}}
\end{judgment}

\begin{judgment}{Well-formed Refinements Contexts}{\wfvarcx{\varcx}}
    \inferrule
        {}
        { \wfvarcx{\emptyset}}

    \inferrule
        { \wfvarcx{\varcx} \\ \sortck{\expr}{\sbool}}
        { \wfvarcx{\varcx,\expr} }

    \inferrule
        { \wfvarcx{\varcx} \\ \aa \notin \dom{\varcx}}
        { \wfvarcx{\varcx,\aa:\sort} }
\end{judgment}

\begin{judgment}{Well-sorted Refinements}{\sortck[\varcx]{\expr}{\sort}}
    \inferrule{\aa:\sort \in \varcx}{\sortck{\aa}{\sort}}

    \inferrule{\sortck{\expr_1}{\sort}\\\sortck{\expr_2}{\sort}}{\sortck{\expr_1=\expr_2}{\sbool}}

    \inferrule{}{\sortck{\cloc}{\sloc}}

    \inferrule
        {
            \oplus \in \{+, -, *\} \\\\
            \sortck{\expr}{\sint} \\ \sortck{\expr_2}{\sint}
        }
        {\sortck{\expr_1 \oplus \expr_2}{\sint}}

    \inferrule
        {
            \oplus \in \{\wedge, \vee\} \\\\
            \sortck{\expr}{\sbool} \\ \sortck{\expr_2}{\sbool}
        }
        {\sortck{\expr_1 \oplus \expr_2}{\sbool}}

    \inferrule
        {
            \sortck{\expr}{\sbool}
        }
        {\sortck{\neg\expr}{\sbool}}

    \inferrule
        {
            n \in \mathbb{Z}
        }
        {\sortck{n}{\sint}}
\end{judgment}


==> overview-old.tex <==
\lstMakeShortInline[language=lr,basicstyle=\ttfamily]`

\section{A Tour of \sys}
\label{sec:overview}

Let us begin with a high-level overview of \sys's
key features that illustrates how liquid refinements
work hand in glove with \rust's types to yield
a compact way to \emph{specify} correctness requirements
and an automatic way to \emph{verify} them with minimal
programmer overhead.
%
First, we show how \sys decorates types with logical
\emph{refinements} that capture invariants
(\S~\ref{sec:overview:ref}).
%
Next, we demonstrate how \rust's type system allows
us to precisely track refinements in the presence of
imperative mutation and \emph{updates} (\S~\ref{sec:overview:mut}).
%
Finally, we show how \sys lets the programmer compose
types to write refined \emph{interfaces}
that can then be used to verify clients in a modular
fashion (\S~\ref{sec:overview:api}).

% \Cref{fig:kmeans} shows \sys in action.
% The functions `init_zeros` and `normalize_centers` are taken from an
% implementation of the \kmeans clustering algorithm and exemplify many of the key features of \sys.
% Without getting into the details, the goal of \kmeans is to compute $k$ sets of
% $n$-dimensional vectors.
% Thus, the algorithm has to maintain the critical invariant that all these vectors
% have the same dimension.
% We specify this invariant by annotating functions with a refined signature using
% the `#[lr::sig]` attribute, which \sys automatically verifies against the implementation.

% In the rest of this section we explain the features of \sys that enables
% the specification and verification of the code in \Cref{fig:kmeans}.
% As we will see, the critical piece is `RVec`, a \emph{refined} version
% of \rust's standard `Vec` that keep tracks of its length statically.
% We begin in \Cref{sec:overview:ref} describing how \sys extends \rust type system
% with refinement types.
% Then, in \Cref{sec:overview:mut}, we briefly explain \rust' unique ownership
% mechanism and how it enables the power of refinement types in the presence of mutation.
% We continue in \Cref{sec:rvec} by looking at the API of `RVec`, which
% illustrates how the combination of refinement types, ownership and polymorphism
% enables the specification of rich invariants.
% Lastly, in \Cref{sec:rmat}, we look at how refinement types can be used to build
% abstractions over data structures that must satisfy some invariant.

% % to naturally express and maintain this invariant.
% The API of `RVec` is shown in \Cref{fig:rvec-api}.
% Throughout the rest of this section,
% we explain all the necessary details to understand the signatures of `RVec`'s methods and how they are
% used to specify the code in \Cref{fig:kmeans}.

\subsection{Refinements}
\label{sec:overview:ref}

% #[lr::sig(fn(usize<@n>) -> usize<n+`\n1`>)]
% fn inc(n: usize) -> usize {
    % n + `\n1`
% }

\begin{figure}
\coderule
\begin{minipage}{0.40\textwidth}
\begin{lr}[xleftmargin=-2.7em,numbersep=3pt,numbers=none]
#[lr::sig(fn(i32<@n>) -> bool<`\n0` < n>)]
fn is_pos(n: i32) -> bool {
  if `\n0` < n { true } else { false }
}
\end{lr}
\end{minipage}
\hspace{0em}
\begin{minipage}{0.46\textwidth}
\begin{lr}[firstnumber=5,numbersep=3pt,numbers=none]
#[lr::sig(fn(i32<@x>) -> i32{v:x<=v && `\n0`<=v})]
fn abs(x: i32) -> i32 {
  if x < `\n0` { -x } else { x }
}
\end{lr}
\end{minipage}
\coderule

\caption{Examples illustrating the three fundamental refinement
type extensions in \sys: indexed types, refinement parameters and
existential types.}

\label{fig:functional}
\end{figure}

Refinement types allow expressions in some underlying,
typically decidable, logic to be used to \emph{constrain}
the set of values inhabited by a type, thereby
tracking additional information about the values of the type
they refine \cite{sprite}.

% By restricting the logic to an SMT-decidable theory, \sys allows the specifications of
% rich invariants while providing a decidable type system.
% Moreover, by using the \emph{liquid types} inference framework~\citep{LiquidTypes, LocalRefinement},
% \sys is able to infer refinements avoiding the burden of excessive annotations.
% \nl{Should we say more about liquid inference? I wouldn't know where to put it though.}
% The three fundamental extensions in \sys are \emph{indexed types},
% \emph{refinement parameters} and \emph{existential types}.

\bpara{Indexed Types}
%
% There was a confusion if you talk about indexed types in general
% (citation was at the end) or in \sys concretely
An indexed type~\cite{XiPfenning99} in \sys refines a \rust base type
by indexing it with a refinement value.
%
Each indexed type is associated with a
refinement \emph{sort} and it must be
indexed by values of that sort.
%
The exact meaning of the index varies depending on the type.
%
For example, \rust primitive integers can be indexed
by integers in the logic (of sort \sint) describing
the exact integer they are equal to.
%
Hence, indexed integers correspond to singleton types,
for instance, the type `i32<n>` describes 32-bit%
\footnote{\rust has primitive types for signed
and unsigned integers of 8, 16, 32, 64 and 128 bits,
plus the pointer-sized integers \inlinelr{usize}
and \inlinelr{isize}.}
signed
integers equal to  `n` and the type `usize<n+$\n1$>` describes
a pointer-sized unsigned integer equal to `n + $\n1$`.
%
Consequently, \sys can verify that the \rust expression $\n1 + \n2 + \n3$
has the type `i32<$\n6$>`.
%
Similarly, the boolean type `bool<b>` is indexed
by the boolean value `b` (of sort \sbool) it is equal to.
%
For example, \sys can type the \rust expression `$\n1 + \n2 + \n3$ <= $\n{10}$` as
`bool<true>`.
%
As a final example, we also consider the type `RVec<T, n>` of
\emph{growable} vectors indexed by their length (of sort \sint),
as detailed later in~\S~\ref{sec:overview:api}.
%
For simplicity, our examples have a single index.
However, as discussed in~\S~\ref{sec:overview:api},
types can have multiple indices, for example, we
can index a type for 2-D matrices by the number
of rows and columns.

\bpara{Refinement Parameters}
%
\sys's function signatures can be
parameterized by variables in the
refinement logic.
%
Informally, such \emph{refinement parameters}
behave like ghost variables that exist
solely for verification, but do not exist
at runtime.
%
\sys automatically instantiates the
refinement parameters using the actual
arguments passed in at the respective sites.

% \bpara{Example: \texttt{is\_pos}}
%
The first two features---indices and refinement parameters---%
are illustrated by the signature for the function `is_pos`
specified with the \rust attribute `#[lr::sig(...)]` on
the left in~\cref{fig:functional}.
%
The function `is_pos` tests whether a 32-bit signed integer
% \footnote{\rust has primitive types for signed
% and unsigned integers of 8, 16, 32, 64 and 128 bits,
% plus the pointer-sized integers \inlinelr{usize}
% and \inlinelr{isize}.}
is (strictly) positive.
%
The signature uses a refinement parameter `n`
to specify that the function takes as input
an integer equal to `n` and returns a boolean
equal to `$\n0$ < n`.
%
The syntax `@n` is used to bind and quantify
over `n` for the entire scope of the function.
% \ag{Quantification is scary and what we're trying to avoid! I assume this is a different sort of quantification since our logic is quantifier-free. What type of different quantification then?}
% Type theoretically it is a quantification, you are quantifying over all possible refinements.

%\footnote{For simplicity, we elide the issue of overflow, which can be
% addressed via standard mechanisms \cite{overflow-blog-lh}.}
%
% The code purposely avoids mutation to center
% the discussion in the refinement type extensions.
% In the next section, we discuss how \rust's unique ownership mechanism unlocks the power of
% refinement types in the presence of mutation.
%
% The attribute `#[lr::sig]` on top of function
% definitions is used to annotate them
% with a refined signature.
% The signature for `inc` specifies
% that the returned value is exactly one more than
% the input.
%
% \nl{inc is actually not sound unless n+1 fits
% in a usize, extremely subtle an unimportant,
% but maybe there's an example as simple as this
% one that doesn't raise suspicions.}

\bpara{Existential Types}
%
Indexed types suffice when we know
the exact value of the underlying term, \ie can
represent it with a \emph{singleton} expression
in the refinement logic.
%
However, often we want to specify that the underlying
value is from a \emph{set} denoted by a refinement
constraint \cite{ConstableS87,Rushby98}.
%
\sys accomodates such specifications via \emph{existential types}
of the form `{v. B<v> | p}` where:
%
(1)~`v` is a variable in the refinement logic,
(2)~`B<v>` is a base type indexed by `v` and
(3)~`p` a predicate constraining `v`.
%
For example, we can use the existential
type `{v. i32<v> | $\n0$ < v}` to specify
the set of \emph{positive} 32-bit integers.
%
Similarly, we can describe the set of
\emph{non-empty} vectors with the type
`{v. RVec<T, v> | $\n0$ < v}`.
%
For types with only one index, we define
the syntax `B{v : p}` to mean `{v. B<v> | p}`.
%
Hence, we can write the two types above
as `i32{v : v > $\n0$}` and `RVec<T>{v : $\n0$ < v}`.
%
Further, we write `B` to abbreviate `B{v : true}`.

% \bpara{Example: \texttt{abs}}
%
Existential types are illustrated by the signature for
the function `abs` shown on the right in~\cref{fig:functional}
which computes the absolute value of the `i32` input `x`.
%
The function's output type is an existential
that specifies that the returned value is a
non-negative `i32` whose values is at least
as much that of the input `x`.

\subsection{Updates}
\label{sec:overview:mut}


\begin{figure}
\coderule
\begin{minipage}{0.93\textwidth}
\begin{lr}
#[lr::sig(fn(usize<@n>) -> RVec<f32, n>)]
fn init_zeros(n: usize) -> RVec<f32> {
    let mut vec = RVec::new();  `\label{line:init_zeros:init-v}`
    let mut i = `\n0`;          `\label{line:init_zeros:init-i}`
    while i < n {
        vec.push(`\n{0.0}`);    `\label{line:init_zeros:push-v}`
        i += `\n1`;             `\label{line:init_zeros:inc-i}`
    }
    vec
}

#[lr::sig(fn(&mut RVec<f32, @n>, &RVec<f32, n>))]
fn add(x: &mut RVec<f32>, y: &RVec<f32>) {
    let mut i = `\n0`;
    while i < x.len() {
        *x.get_mut(i) = *x.get(i) + *y.get(i);  `\label{line:add:get}`
        i += `\n1`;
    }
}

#[lr::sig(fn(usize<@n>, &mut RVec<RVec<f32, n>, @k>, &RVec<f32, k>))]
fn normalize_centers(n: usize, xs: &mut RVec<RVec<f32>>, ws: &RVec<usize>) -> i32 {
    let mut i = `\n0`;
    while i < xs.len() {
        normal(xs.get_mut(i), *ws.get(i)); `\label{line:normalize_centers:normal}`
        i += `\n1`;
    }
}
\end{lr}
\end{minipage}
\coderule
\caption{Code taken from an implementation of the \kmeans clustering algorithm illustrating
the interaction between ownership and refinement types.
The code uses \inlinelr{RVec}, a refined version of \rust's \inlinelr{Vec}, to ensure the algorithm works
over vectors of the same dimension.}
\label{fig:kmeans}
\end{figure}

The whole point of \rust, of course, is to
allow for efficient imperative \emph{sharing}
and \emph{updates}, without sacrificing
thread- or memory-safety.
%
This is achieved via an \emph{ownership type system}
that ensures that aliasing and mutation cannot happen
at the same time \cite{Noble98,ownership-survey,RustBelt}.
%
Next, let's see how \sys lets logical constraints
ride shotgun with \rust's ownership types to scale
refinement types to an imperative setting using
(parts of) an implementation of the \kmeans clustering
algorithm shown in \cref{fig:kmeans}.
%
In this code, each $n$-dimensional point is represented as
a vector of size $n$, and we wish to verify the
safety of vector accesses, \ie that each
read and write occurs within the bounds
of the vector.

This goal is challenging for two reasons.
%
First, the vector sizes can \emph{grow} or \emph{shrink}
via `push` or `pop` operations.
%
Second, the code maintains several \emph{collections}
of points (\eg clusters or candidate centers)
where each point must have the same
dimensions.
%
This combination of mutation and collections
complicates verification using program-logic \cite{Prusti}
by necessitating the use of complex, user-specified,
universally quantified invariants (\S~\ref{sec:eval:compare}).
%
In contrast, let us see how \sys entirely automates
verification by fusing refinements with \rust's
syntactic discipline for controlling sharing
and updates.


\bpara{Exclusive Ownership}
%
\rust's most basic form of ownership
is \emph{exclusive ownership}, in
which only one function has the
right to mutate a memory location.
%
In \sys, exclusive ownership plays
crucial role: by ruling out aliasing, we can
safely perform \emph{strong updates}~\citep{L3,AliasTypes},
\ie we can change the refinements on a type when updating data,
and thereby, use different types to denote the different values
at that location at different points in time.

% \bpara{Example: \texttt{init\_zeros}}
%
For example, consider the function `init_zeros` which
takes as input a `usize` value `n`
and returns as output an `n`-dimensional
vector of 32-bit floats (`f32`), specified
as `RVec<f32, n>`.
%
The integer counter `i` is initialized with $\n0$
on line \ref{line:init_zeros:init-i} of~\cref{fig:kmeans}.
%
After the definition, the memory location
pointed to by `i` is exclusively owned by
the function `init_zeros`, meaning it cannot
be updated by any other code or thread.
%
Thus, if at line \ref{line:init_zeros:inc-i}
in~\cref{fig:kmeans} we know `i` has type `i32<j>`
for some `j`, then, after executing the statement `i += $\n1$`,
we can update its type to be `i32<j + $\n1$>`.
%
As detailed later in \S~\ref{sec:implementation}
\sys's liquid typing exploits these strong updates
to automatically infer that `i` is equal to the length
of `vec`
%when the loop exits,
%`i` has the type `i32<n>`
(and since the loop exists with `i = n`, the returned
value `vec` has type `RVec<f32, n>`).


\bpara{Shared and Mutable References}
%
Exclusive ownership suffices for local updates
(\eg `i` in `init_zeros`) but for more complex
data, ultimately, functions must % eventually NV: ultimately is enought
reliquish ownership to other functions that
update the data in some fashion.
%
\rust's unique approach to allow this
is called \emph{borrowing}, via two kinds
of references.
%
First, a value of type `&T` is a \emph{shared}
reference, that can be used to access the `T` value
in a read-only fashion.
%
Second, a value of type `&mut T` is considered
to be a \emph{mutable reference} that can be used
to write or update the contents of a `T` value.
%
For safety, \rust allows multiple aliasing
(read-only) shared references but only a
single mutable reference to a value at a time.

% Shared references play an important role as a mechanism that allows \rust
% to provide primitives for shared mutable state~\cite{RustBelt}, but their
% direct interaction with refinement types is less surprising.
% As a quick example, consider the second argument to the function `add` which is a
% shared reference to a vector.

For example, consider the function `add`
in \cref{fig:kmeans}, which adds two vectors
point-wise, mutating the first vector in-place.
%
This means that clients of `add` must grant
access to mutate the vector. \rust's key idea
is that when calling `add` the vector is only
temporarily borrowed, granting write access
to the callee for the duration of the
function call.
%
In plain \rust, this protocol is specified
by saying that `add` takes a mutable reference
`&mut RVec<f32>` to the first vector and a shared
reference `&RVec<f32>` to the second (which is not
modified by `add`).
%
\sys refines the \rust signature to say that the
first argument has type `&mut RVec<f32, @n>`, \ie
is a vector of size `n`, and that the second vector
also has the same size.
%
Crucially, unlike updates to an owned location,
updates through a mutable reference `&mut T`
\emph{do not change} the type `T`.
%
In other words, mutating through a mutable
reference can only perform \emph{weak updates}.
%
This may sound like a restriction, but it
is actually a powerful notion, as the caller
can rely upon the fact that recipients of a
mutable reference `&mut T` will respect the
invariants of `T`.
%
For instance, clients of `add` can be sure
that the first vector will continue to have
the same length after the function returns.

% Consider again the implementation of `init_zeros`.
% Initially, `vec` is exclusively owned by the function after its definition
% in line \ref{line:init_zeros:init-v}.
% Later, in line \ref{line:init_zeros:push-v}, we call the `push` method on `vec`.
% This requires granting `push` temporary access to mutate `vec`.
% \rust's unique approach to allow this is \emph{borrowing}, which is the mechanism used to handle
% references.
% The idea is that when calling `push`, `vec` is only borrowed, granting
% access to mutate `vec` for the duration of the function call.

% The syntax `vec.push($\n{0.0}$)` roughly desugars to `RVec::push(&mut vec, $\n{0.0}$)`,
% where `&mut vec` creates a mutable reference to `vec`.
% A mutable reference `&mut T` grants \emph{temporary exclusive access} to a value
% of type `T`.
% A recipient of a mutable reference not only gains access to mutate the value,
% it also upholds the responsibility to ensure the value continuous to have type `T`.
% This has an interesting interaction with refinement.
% For example, a recipient of a mutable reference `&mut i32{v : v > $\n0$}` can mutate
% the value, but it must also uphold the constraint `v > $\n0$`.

\bpara{Whither Strong Updates?}
%
\rust's existing mechanisms to control aliasing and mutation---%
%
(1) exclusive ownership, which provide strong updates
    but preclude any aliasing,
%
(2) shared references (borrows), which allow aliasing, but
    preclude any form of updates, and
%
(3) mutable references (borrows), which allow weak updates,
    but preclude any form of aliasing---%
%
are insufficient for refinement typing.
%
To verify idiomatic \rust code we require
references that permit \emph{strong updates}.

Consider again the function `init_zeros`
from \cref{fig:kmeans}.
%
Initially, `vec` is exclusively owned by
the function after its definition in line
\ref{line:init_zeros:init-v}.
%
Later, in line \ref{line:init_zeros:push-v},
we call the `push` method on `vec`.
%
The syntax `vec.push($\n{0.0}$)` desugars
to `RVec::push(&mut vec, $\n{0.0}$)`, where
`&mut vec` creates a mutable reference to `vec`.
%
Thus, the traditional way to handle this
call would be for `push` to take a mutable
reference.
%
However, as mutable references only allow
weak updates, we would not be able to change
the type of `vec` after the call, thereby
leaving the verifier clueless that the
size increased by one.

\bpara{Strong References}
%
To this end, \sys extends \rust with
\emph{strong references}, written `&strg T`,
which refine \rust's `&mut T` and,
like regular mutable references, also
grant temporary exclusive access but allow
strong updates.
%
\sys accommodates strong references by extending
function signatures to specify the \emph{updated type}
of each strong references after the function returns.

For example, consider the signature for `RVec::push` shown
in \cref{fig:rvec-api}. The plain \rust signature for this
function is `fn(&mut self, T) -> ()`, where `self` refers
to the receiver `RVec<T>`.
%
However, the \sys signature for `RVec::push` refines the
above to specify that:
%
(1)~the receiver is an `RVec<T, n>`, \ie a vector of size `n`,
%
(2)~`self` is a \emph{strong} mutable reference, and
%
(3)~the \emph{updated} type of the receiver is `RVec<T, n+$\n1$>`,
    as denoted by the method's `ensures` clause.
%
Crucially, as `n` is a refinement parameter denoting the input
size of the receiver, the above updated type precisely tracks
how `push` increases the size of the underlying vector.
\nv{This forward reference that you refer to push signature before you introduce the
Vec API is confusing.}


\subsection{Interfaces}
\label{sec:overview:api}

\begin{figure}
\begin{framedlr}
impl RVec<T, @n> {
    fn new() -> RVec<T, `\n0`>;
    fn len(&self) -> usize<n>;
    fn is_empty(&self) -> bool<n == `\n0`>;
    fn get(&self, idx: usize{v : v < n}) -> &T;
    fn get_mut(&mut self, idx: usize{v : v < n}) -> &mut T;
    fn push(&strg self, value: T) -> ()
       ensures *self: RVec<T, n + `\n1`>;
    fn pop(&strg self) -> T
       requires n > `\n0` ensures *self: RVec<T, n - `\n1`>;
}
\end{framedlr}
% alternative syntax without impl
% \begin{lr}
% fn new() -> RVec<T, `\n0`>;
% fn len(&RVec<T, @n>) -> usize<n>;
% fn is_empty(&RVec<T, @n>) -> bool<n == `\n0`>;
% fn get(&RVec<T, @n>, usize{v : v < n}) -> &T;
% fn get_mut(&mut RVec<T, @n>, usize{v : v < n}) -> &mut T;
% fn push(vec: &strg RVec<T, @n>, T) ensures *vec: RVec<T, n + `\n1`>;
% fn pop(vec &strg RVec<T, @n>) -> T
%   where n > `\n0`
%   ensures *vec: RVec<T, n - `\n1`>;
% \end{lr}
\caption{
Signatures of \inlinelr{RVec} methods.
The \inlinelr{impl} syntax mirrors \inlinelr{impl} blocks in \rust.
The type variable \inlinelr{T} and the refinement variable \inlinelr{n}
are in scope for the entire block.
The syntax \inlinelr{&self}, \inlinelr{&mut self}, and \inlinelr{&strg self} are used
as in \rust as shorthand for reference of the block's type (\inlinelr{RVec<T, n>} in this case).
}
\label{fig:rvec-api}
\end{figure}

Our design for \sys crucially allows
us to use standard type constructors
as building blocks to \emph{compose}
complex structures from simple ones,
in a way that, dually, lets standard
syntax directed typing rules \emph{decompose}
complex reasoning about those structures
into efficiently decidable (quantifier free)
validity queries over the constituents.
%
Next, we illustrate this composition
by showing a refined API for operating
on \emph{vectors}, and demonstrating how the
API can be used to implement a refined
API for reasoning about \emph{matrices},
all while guaranteeing that well-typed programs
access the underlying containers within their
prescribed bounds.

\bpara{A Refined Vector API}
%
\Cref{fig:rvec-api} summarizes the signatures
for `RVec`---vectors refined by size.
%
\sys uses the syntax `impl RVec<T, @n>`,
inspired by \rust `impl` blocks, to bind the type
variable `T` and the refinement variable `n` for
the entire block.
%
In the signature for each method, the syntax
`&self`, `&mut self`, and `&strg self`
denote references to the receiver's type,
`RVec<T, n>` in this case.

\begin{itemize}

\item `new` is used to construct empty
vectors: the return type `RVec<T, $\n0$>` guarantees
the returned vector has size zero.

\item `len` can be used to determine the
size of the vector. The method takes a shared reference,
which implicitly specifies the vector will have the same
length after the function returns. Moreover, the returned
`usize<n>` stipulates the result equals the receiver's size.

\item `is_empty` also takes a shared reference and
checks if the vector is empty, returning a boolean
which is true exactly when the length is zero.

\item `get` and `get_mut` are used to access the elements
of the vector: `get` returns a shared (read-only) reference
while `get_mut` returns a mutable one that can be used to
update the vector (as in line \ref{line:add:get} in
`add` of \cref{fig:kmeans}). The type for the index `idx`
specifies that only valid indices (less than size `n`)
%\nv{this is confusing: either only say less than n or clarify that the greater or
%equal to 0 comes from Rust. (I prefer the first)}
%\nv{Shall I edit?}
can be used to access the receiving vector.
%
Crucially, by taking a mutable reference, `get_mut`
guarantees that the length of the vector and the type
of the elements it contains remain the same after the
function returns.
%
Furthermore, by returning a mutable reference, users
of `get_mut` must respect the invariants in `T` when
mutating the reference, ensuring the vector will continue
to hold elements of type `T`.
\nv{For a non refinement type expert to understnad what you mean here
we need to give an example where T is refined.
Or just say here, for example a vector of integers geater than 42}

\item `push` and `pop` are used to grow and shrink
the vector by one element at a time.
%
As discussed in \S~\ref{sec:overview:mut}, `push`
takes a strong reference and specifies that the length
of the vector has increased by one after the function
returns, via the `ensures` clause `*self: RVec<T, n + $\n1$>`
which denotes the updated type of the location pointed
to by the `self` parameter after the function call.
%
Similarly, `pop` ensures the length has decreased
by one, but stipulates the precondition that the vectors
must be non-empty before popping via the `requires` clause
that constrains the refinement parameter `n` to be positive.
%
\end{itemize}

\bpara{Quantified Invariants via Polymorphism}
\nv{I believe this should go to 2.1}
%
`RVec` is polymorphic over `T`: the type of elements
it contains.
%
For a classical type systems, polymorphism facilitates
code \emph{reuse}: we can use the datatype to hold
collections of integers or strings or booleans \etc.
%
\sys exploits polymorphism to enable specification
and verification: we can instantiate `T` with arbitrary
refined types to compactly specify that \emph{all}
elements of the vector satisfy some invariant.
%
For instance, the function `normalize_centers`
in \cref{fig:kmeans} uses `RVec<RVec<f32, n>, k>`
to concisely specify a collection of `k`-centers,
\emph{each of which} is an `n`-dimensional point.
%
Program logic based methods must use universally quantified
formulas to express such properties, which increases the
specification burden on programmers (who must now write
tricky quantified invariants), and the verification burden
on the solver (which must now reason about those quantified
invariants!).
%
In contrast, \sys's type-directed method automatically
verifies, that despite working over mutable references,
we can be sure all the inner vectors still
have the same length after the function
returns even though we are passing references
to these vectors to the function `normal`
in line~\ref{line:normalize_centers:normal}.


\bpara{A Refined Matrix API}
%
Suppose now that we want to work
with 2-dimensional matrices.
%
As we have seen in the `kmeans` code
we could implement this as a vector
of vectors, but spelling out the type
every time gets tedious.
%
By extending \rust's built-in mechanism
for custom data structure with refinement
types, \sys lets us easily define refined
abstractions that avoid working directly
over the vector of vectors.
%
\ag{The next few sentences are kinda repititive, 4x ``the x does y''}
The code in \cref{fig:rmat} uses `RVec`
to build a verified refined API for matrices.
%
The type `RMat<m, n>` corresponds
to a 2-dimensional matrix of size `m $\times$ n`
that is implemented using a vector of vectors.
%
The attribute `#[lr::refined_by]`
on the `struct` definition specifies
the type is indexed by two integers
`m` and `n`.
%
The attribute `#[lr::field]` is used
to annotate the field `vec` with a
refinement type.
%
\sys will track and ensure that `vec`
always has this type over the different
`RMat` methods:
%
\begin{itemize}
    \item `new` initializes a matrix
           of size `m $\times$ n` with
           all elements set to `$\n{0.0}$`,
           using `init_zeros` from \cref{fig:kmeans}
           to initialize each inner vector with zeros.
    \item `get` and `get_mut` are used to access
           the elements of the matrix using valid
           indices as arguments.
\end{itemize}

\rj{need some outro for this section}
\sys can be used to ensure that the clients of such
refined interfaces satisfy the specified invariants.
In~\S~\ref{sec:eval} we use the `RVec` and `RMat` refined
APIs to verify seven clients and conclude that verification
requires less annotations and it is two times faster than
program-logic based verifiers that use quantifiers.


% \nl{new and initzeros are fundamentally the same function, but to implement it polymorphically
% we would need support for Clone. Maybe we can mention it.}

\begin{figure}
\begin{framedlr}
#[lr::refined_by(m: int, n: int)]
pub struct RMat {
    #[lr::field(RVec<RVec<f32, n>, m>)]
    vec: RVec<RVec<f32>>
}

impl RMat {
    #[lr::sig(usize<@m>, usize<@n>) -> RMat<m, n>]
    pub fn new(m: usize, n: usize) -> RMat {
        let mut vec = RVec::new();   `\label{line:rmat:new}`
        let mut i = `\n0`;
        while i < m {
            vec.push(init_zeros(n));
            i += `\n1`;
        }
        RMat { vec }
    }

    #[lr::sig(&RMat<@m, @n>, usize{v : v < m}, usize{v : v < n}) -> &f32]
    pub fn get(&self, i: usize, j: usize) -> &f32 {
        self.vec.get(i).get(j)
    }

    #[lr::sig(&mut RMat<@m, @n>, usize{v : v < m}, usize{v : v < n}) -> &mut f32]
    pub fn get_mut(&mut self, i: usize, j: usize) -> &mut f32 {
        self.vec.get_mut(i).get_mut(j)
    }
}
\end{framedlr}
\caption{Implementation of a 2-dimensional matrix as a vector of vectors of the same length.
The attribute \inlinelr{lr::refined_by} is used to declare the struct's indices \inlinelr{m} and \inlinelr{n}.
The attribute \inlinelr{lr::field} is used to annotate the struct field with a refinement type.
}
\label{fig:rmat}
\end{figure}

\lstDeleteShortInline`

